Testing Symmetric Markov Chains from a Single Trajectory

Classical distribution testing assumes access to i.i.d. samples from the distribution that is being tested. We initiate the study of Markov chain testing, assuming access to a single trajectory of a Markov Chain. In particular, we observe a single trajectory X0,...,Xt,... of an unknown, symmetric, and finite state Markov Chain M. We do not control the starting state X0, and we cannot restart the chain. Given our single trajectory, the goal is to test whether M is identical to a model Markov Chain M0 , or far from it under an appropriate notion of difference. We propose a measure of difference between two Markov chains, motivated by the early work of Kazakos [Kaz78], which captures the scaling behavior of the total variation distance between trajectories sampled from the Markov chains as the length of these trajectories grows. We provide efficient testers and information-theoretic lower bounds for testing identity of symmetric Markov chains under our proposed measure of difference, which are tight up to logarithmic factors if the hitting times of the model chain M0 is O(n) in the size of the state space n.

==> MC_to_adversarial.tex <==
Summary of our approach.


==> adversarial.tex <==
\section{The Adversarial Testing Problem}

	
	\begin{definition}
	\textbf{Input:} $\eps$, Distributions $q_1,\ldots,q_n$ and $p_1,p_2,\ldots,p_n$ each with a support of size $n$. For $t=1$ to $m$, adversary picks a $j(t) \in \{1,\ldots,n\}$ and draws $\Poi(1)$ samples from $p_j(t)$ and gives the samples to the tester.
	Promised that either Case 1: $p_j = q_j$ for all $j \in \{1,\ldots,n\}$ or Case 2: $\sum_{t=1}^{m} \dtv(p_j(t),q_j(t)) \ge m\eps$ for all $j \in \{1,\ldots,n\}$ happens.
	\\
	\noindent \textbf{Output:} With probability $\ge 2/3$, correctly distinguish between case 1 and case 2.
	\end{definition}
	
\subsection{Bucketing Approach to Solve the Adversarial Testing Problem}
	For each $j \in \{1,\ldots,n\}$ let $\mathcal{A}_j$ be the set of $i$ such that $q_{ij} \ge \eps/50n$.
	Each time step the adversary chooses a distribution and draws $\Poi(1)$ samples, we define a new term in our statistic for those samples. 
	Suppose the adversary chooses distribution $j(t)$ at time step $t$ and let $X_{j(t)} \sim \Poi(1)$ denote the number of samples drawn. Let $X_{ij(t)}$ denote the number of occurences of element $i$ within these $X_{j(t)}$ samples. Then define
	\begin{align}
	Z_t = \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{\left(X_{ij(l)} - q_{ij(l)}\right)^2 - X_{ij(l)}}{q_{ij(l)}}
	\end{align}
	with $Z_0 = 0$ and our final statistic $Z = Z_m$ where $m$ is the number of time steps the adversary runs for.
	In case 1, $\E[Z] = \E[Z_m] = 0$. In case 2, $\E[Z] = \E[Z_m] = \sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)}}, q_{\mathcal{A}_{j(t)}} \right) \ge \sum_{t=0}^m \eps^2/5 = m\eps^2/5$.
	We will now study the tail behavior of the random variable $Z_m$ by using tools from martingale theory.\\
	
	
	
	
	$Z_t$ can be expressed as a sum of three terms, the first two of which each form a martingale sequence and the third term is a constant.
	\begin{align}
	Z_t &= \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{\left(X_{ij(l)} - q_{ij(l)}\right)^2 - X_{ij(l)}}{q_{ij(l)}} \\
	&= \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{\left(X_{ij(l)} - p_{ij(l)}\right)^2 - X_{ij(l)} + (p_{ij(l)} - q_{ij(l)})^2 -2(X_{ij(l)}-p_{ij(l)})(p_{ij(l)} - q_{ij(l)} ) }{q_{ij(l)}} \\
	&= A_t - 2B_t + C_t
	\end{align}
	where
	\begin{align*}
	A_t = \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{\left(X_{ij(l)} - p_{ij(l)}\right)^2 - X_{ij(l)}}{q_{ij(l)}}\\
	B_t = \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{\left(X_{ij(l)} - p_{ij(l)}\right)\left(p_{ij(l)} - q_{ij(l)}\right)}{q_{ij(l)}}\\
	C_t = \sum_{l=0}^t \sum_{i \in \mathcal{A}_{j(l)}} \frac{(p_{ij(l)} - q_{ij(l)})^2}{q_{ij(l)}} = \E[Z_t]
	\end{align*}
	
	\begin{lemma}
	The sequences $\{A_t\}_{t \ge 0}$ and $\{B_t\}_{t \ge 0}$ are martingales.
	\end{lemma}
	\begin{proof}
		\begin{align}
		\E\left[A_{t+1} | A_t\right] &= A_t + \E\left[\sum_{i \in \mathcal{A}_{j(t+1)}} \frac{\left(X_{ij(t+1)} - p_{ij(t+1)}\right)^2 - X_{ij(t+1)}}{q_{ij(t+1)}}\right] \\
		&= A_t + \sum_{i \in \mathcal{A}_{j(t+1)}} \frac{\E\left[\left(X_{ij(t+1)} - p_{ij(t+1)}\right)^2\right] - \E\left[X_{ij(t+1)}\right]}{q_{ij(t+1)}} \\
		&= A_t + \sum_{i \in \mathcal{A}_{j(t+1)}} \frac{p_{ij(t+1)} - p_{ij(t+1)}}{q_{ij(t+1)}} = A_t, \label{eq:a3}
		\end{align}
		where (\ref{eq:a3}) holds because $X_{ij(t+1)} \sim \Poi(p_{ij(t+1)})$ and for a Poisson random variable with parameter $\l$, we have that the second central moment is the same as the mean and both are equal to $\l$. Hence $\{A_t\}_{t \ge 0}$ is a martingale sequence.
		Similarly,
		\begin{align}
		\E\left[B_{t+1} | B_t\right] &= B_t + \E\left[\sum_{i \in \mathcal{A}_{j(t+1)}} \frac{\left(X_{ij(t+1)} - p_{ij(t+1)}\right)(p_{ij(t+1)} - q_{ij(t+1)})}{q_{ij(t+1)}}\right] \\
		&= B_t + \sum_{i \in \mathcal{A}_{j(t+1)}} \frac{\E\left[\left(X_{ij(t+1)} - q_{ij(t+1)}\right)\right](p_{ij(t+1)} - q_{ij(t+1)})}{q_{ij(t+1)}} \\
		&= B_t. \label{eq:b3}
		\end{align}
		Hence $\{B_t\}_{t \ge 0}$ is a martingale sequence.
	\end{proof}
	
	\begin{corollary}
		$$\E[C_t] = \E[Z_t].$$
	\end{corollary}
	\begin{proof}
		Since $A_t$ and $B_t$ form martingale sequences we have $\E[A_t] = \E[B_t] = 0$ for all $t$.
	\end{proof}
	
	
\noindent The next step is to employ martingale tail inequalities on $\{A_t\}_{t \ge 0}$ and $\{B_t\}_{t \ge 0}$. Let us focus on $\{A_t\}_{t \ge 0}$ for the purpose of this discussion. To employ Freedman's inequality (\ref{eq:freedman}) on this martingale sequence, we first need to bound the sum of the conditional variances of the martingale increments i.e. $\sum_{t=0}^{m-1} \Var{A_{t+1}-A_t | A_t}$. This quantity, however, depends on the choices made by the adversary. And it is important to incorporate a choice-dependent bound to solve the problem efficiently because any uniform bound we can show across all possible choices of the adversary leads to suboptimal sample complexity. This is because the sum of the variances can potentially vary over a wide range of values forcing the tester to pay a high penalty in the worst case. However, the key insight is that the adversary cannot win by playing with the sum of the variances because the variances are intricately coupled with the expected value of our statistic and in particular, when we are in case 2, if the adversary made choices so that the sum of the variances is large the expected value of the statistic is also sufficiently large which allows us to distinguish the two cases. \\

\noindent Martingale inequalities are not equipped to work under such adaptive settings. They typically require a a bound on the increments or variances which are fixed constants. To tackle the adaptivity, we take the following approach. We first observe that an upper bound on $\sum_{t=0}^{m-1} \Var{A_{t+1}-A_t | A_t}$ is $f(n,1/\eps)\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right)$ for an appropriate function $f$ which is choice independent. We have thus seperated the choice dependent and the choice independent parts from the bound. Next, we observe that we can show a gap of $\Omega(\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right))$ between the values of $\E[Z_m]$ under the two cases. \\

\noindent Given the above observations, we proceed as follows. $\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right)$ can range from $m\eps^2/5$ to $200mn/\eps$. The lower bound comes from \ref{} and the upper bound follows from \ref{}. Define
\begin{align}
\left[ \left\lfloor \frac{m\eps^2}{5} \right\rfloor = \gamma_0, \gamma_1, \ldots, \gamma_{\lceil \log_2 \frac{1000n}{\eps^3} \rceil} \ge \frac{200mn}{\eps}  \right]
\end{align}
such that $\gamma_{i+1} = 2\gamma_i$. Also let $\lceil \log_2 \frac{1000n}{\eps^3} \rceil = w$. The interval $[\gamma_0, \gamma_w]$ covers the whole range of possible values of the quantity $\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right)$.
The next crucial observation is that although analyzing our adversary $H$ directly is difficult, he is no more powerful than the union of a group of $w$ adversaries $\{H_l\}_{1 \le l \le w}$ who operate on the same input in the following manner. Each  $H_l$ runs for $m$ steps and is allowed to pick any sequence of $m$ distributions, denoted by $\{j(t)^{(l)}\}$, which satisfies $\sum_{t=0}^m \dtv(p_{j(t)^{(l)}},q_{j(t)^{(l)}}) \ge m\eps$ with the additional restriction that $\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right) \in [\gamma_{l-1}, 2\gamma_l]$. 
This observation shown formally in Lemma~\ref{lem:adversary-breakdown} enables us to split the analysis of the original adaptive adversary into the analysis for each of these restricted adversaries for whom we can employ martingale tail inequalities. 


To make the above observation formal, we define some notation. First, we will draw $m$ i.i.d $\Poi(1)$ random variables (denote their values by $r_1,r_2,\ldots,r_m$) apriori to use as the sample sizes from each $\{ p_{j(t)}\}$. Let $s_t = \sum_{l=1}^t r_l$. Given $r_1,\ldots,r_m$, let $\pi^t : [n]^t \times [n]^{s_t} \rightarrow [n] $ denote a policy function followed by the adversary $H$ at step $t$ to choose $j(t+1)$. The input to $\pi^t$ is the past history of choices made and samples observed until time $t$. The output is the value of $j(t+1)$. Clearly, the adversary has access to all samples seen so far to make future decisions and hence, he is adaptive. We let $\pi$ denote the overall policy followed by the adversary throughout the process. The goal of the adversary is to maximize the probability of failure of our test. If on a particular sequence of observations (and choices made by the adversary) $[n]^m \times [n]^{s_m}$ our tester outputs a wrong answer we will give a reward of 1 and 0 otherwise. The reward obtained by an adversary following a policy $\pi$ on a sequence of observations $o \in [n]^m \times [n]^{s_m}$ is denoted by $\pi(o)$.
Then we have the following Lemma.
\begin{lemma}[Relating the Power of Adversary $H$ to the joint power of $\bigcup_l \{H_l\}$]
\label{lem:adversary-breakdown}
Let $\pi_*$ denote the optimal policy that can be followed by $H$. There exists a set of policies $\{ \pi_l \}$ such that $\pi_l$ is a valid policy for the adversary $H_l$ and 
\begin{align}
\left\{ o : \pi_*(o) = 1 \right\} \subseteq \bigcup_{l=1}^w \left\{ o : \pi_l(o) = 1 \right\}
\end{align}
\end{lemma}	
\begin{proof}
We will view the sequence of choices a policy can make as a directed graph with $2m+1$ levels indexed from 0 to $2m$,  where each node in level $2t$ uniquely corresponds to a possible state of the world $(o \in [n]^t \times [n]^{s_t})$ after the adversary has made $t$ moves and a total of $s_t$ samples have been drawn ($r_i$ at step $i$), and level $2t+1$ corresponds to the state of the world after the adversary has made $t+1$ moves but the samples from $p_{j(t+1)}$ are yet to be drawn. We connect states in adjacent levels by directed arrows if we can go from one state to the other. An alternate view of this graph is as the strategy space of a two-player game being played by nature and the adversary. Adversary makes moves from even levels to odd levels. Nature makes moves from odd levels to even levels.\\
\noindent Given this representation, let us focus on constructing $\pi_l$ for some $l$. Denote the constraint $\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right) \in [\gamma_{l-1}, 2\gamma_l]$ by $C_l$. First we go to level $2m$ and color all the states which correspond to a sequence of adversary choices which don't violate $C_l$. Then, working backwards we color nodes in previous levels if there exists a path leading to a colored node at the last level. \\
\noindent Once we have done this coloring, we construct $\pi_l$ as follows: starting from the initial state we follow along the path $\pi_*$ takes as long as we are in a colored state at every even level. If $\pi_*$ makes a step to a state which is uncolored we deviate and follow the path of colored nodes which is guaranteed to exist from our current state. Now a crucial observation is that colored nodes in odd levels only have colored neighbors in the next level. That is, no matter how many samples we see and what samples we see, if after choosing a certain $p_{j(t)}$ we are in colored state we can still transition to a colored state for the next time step. This is because the samples observed (which aren't under the adversary's control) do not affect the adversary's ability to satisfy or violate $C_l$. Hence, this construction ensures we end up in a state which satisfies $C_l$ thereby implying that $\pi_l$ is a valid policy for adversary $H_l$. \\
\noindent We construct all $\pi_l$s in the manner above and the final observation is that since the interval $[\gamma_0, \gamma_w]$ contains the whole range of values $\sum_{t=0}^m \chi^2\left(p_{\mathcal{A}_{j(t)^{(l)}}}, q_{\mathcal{A}_{j(t)^{(l)}}} \right)$ can take, no matter which path $\pi_*$ takes, there exists an $l$ such that the path is also taken by $\pi_l$. Finally, since policy $\pi_*$ has to satisfy the constraint that $\sum_{t=0}^m \dtv(p_{j(t)^{(l)}},q_{j(t)^{(l)}}) \ge m\eps$, and we have constructed $\pi_l$ such that the set of paths it takes is a subset of the paths $\pi_*$ could have taken, the above constraint is still satisfied for every potential path $\pi_l$ could take.
\end{proof}	


Due to Lemma~\ref{lem:adversary-breakdown}, we immediately get the following Corollary via a union bound. 
\begin{corollary}
\label{cor:adversary-union-bound}
If under adversary $H_l$ our tester fails with a probability $\le 1/n^2$, then under adversary $H$ it fails with probability at most $w/n^2$.
\end{corollary}	
	
	
Now, we focus on adversaries of the type $H_l$ for each $l$ and show that our tester succeeds under each of them with a high probability. Let us consider our statistic under an adversary of the type $H_l$ for some $l \in \{1,2,\ldots,w\}$. It can be easily verified that $\{A_t\}_{t \ge 0}$ and $\{B_t\}_{t \ge 0}$ and still martingales with $A_0 = 0$ and $B_0 = 0$.
We will argue that both these martingale sequences concentrate around 0. We begin by defining a common stopping time for the two martingale sequences. Intuitively, the stopping time is used to exclude events with a very low probability for hurting our bounds. 
	
	
	\begin{definition}[Stopping Time for the Martingale sequences]
		\label{def:stoppingtime}
		Let $\tau_K$ be a stopping time for the martingale sequence $\{Z_t\}_{t \ge 0}$ defined as follows:
		\begin{align*}
		\tau_K = \min_{t \ge 0} \left\{t  \middle| X_{j(t)} > K\log n \right\}.
		\end{align*}
	\end{definition}
	
	\begin{lemma}[Stopping Time Large]
		\label{lem:largestoppingtime}
		\begin{align}
		\Pr\left[\tau_K \le m \right] \le m\exp\left(-\frac{K^2\log^2 n}{2(1+K\log n)} \right).
		\end{align}
	\end{lemma}
	\begin{proof}
		Prove using Tail bound on Poisson random variables from Canonne's note and union bound.
	\end{proof}
	
	\begin{lemma}[Martingale Increment Bound]
		\label{lem:incrementbounds}
		If $X_{j(t+1)} \le K\log n$, then 
		\begin{align}
		&\abss{A_{t+1} - A_t} \le \frac{51n\log^3 n}{\eps} \text{ for all } 0\le t < m, \label{eq:incrementbound1}\\
		&\abss{B_{t+1}-B_t} \le \frac{51n\log^2 n}{\eps}\text{ for all } 0\le t < m. \label{eq:incrementbound2}
		\end{align}
	\end{lemma}
	\begin{proof}
		We begin with the proof of (\ref{eq:incrementbound1}).
		\begin{align}
		\abss{A_{t+1}-A_t} &= \abss{\sum_{i \in \mathcal{A}_{j(t+1)} } \frac{(X_{ij(t+1)} -p_{ij(t+1)})^2 - X_{ij(t+1)}}{q_{ij(t+1)}} } \\
		&\le \abss{ \sum_{i \in \mathcal{A}_{j(t+1)}, X_{ij(t+1)} = 0 } \frac{p_{ij(t+1)}^2}{q_{ij(t+1)}}} + \abss{\sum_{i \in \mathcal{A}_{j(t+1)}, X_{ij(t+1)} > 0 } \frac{\log^2 n}{q_{ij(t+1)}} } \label{eq:incr1e1} \\
		&\le \abss{ \sum_{i \in \mathcal{A}_{j(t+1)}} \frac{p_{ij(t+1)}^2}{q_{ij(t+1)}}} + \frac{50Kn\log^3 n}{\eps} \label{eq:incr1e2} \\
		&\le \frac{50n}{\eps}\sum_{i \in \mathcal{A}_{j(t+1)}} p_{ij(t+1)}^2 + \frac{50Kn\log^3 n}{\eps} \label{eq:incr1e3} \\
		&\le \frac{51Kn\log^3 n}{\eps},  \label{eq:incr1e4}
		\end{align}
		where TODO.
		Next, we proceed to show (\ref{eq:incrementbound2}). 
		\begin{align}
		\abss{B_{t+1}-B_t} &= \abss{\sum_{i \in \mathcal{A}_{j(t+1)} } \frac{(X_{ij(t+1)} -p_{ij(t+1)})( p_{ij(t+1)} - q_{ij(t+1)}  )}{q_{ij(t+1)}} } \\
		&\le \abss{ \sum_{i \in \mathcal{A}_{j(t+1)}, X_{ij(t+1)} = 0 } \frac{p_{ij(t+1)}^2}{q_{ij(t+1)}}} + 2\abss{\sum_{i \in \mathcal{A}_{j(t+1)}, X_{ij(t+1)} > 0} \frac{\log n}{q_{ij(t+1)}}} \\
		&\le \frac{50n}{\eps}\sum_{i \in \mathcal{A}_{j(t+1)}} p_{ij(t+1)}^2 + \frac{50Kn\log^2 n}{\eps} \\
		&\le \frac{51Kn\log^2 n}{\eps},
		\end{align}
		where TODO.
	\end{proof}


	\begin{lemma}[Bound on Conditional Variance of Increments]
		\label{lem:varbounds}
		\begin{align}
		&\Var{A_{t+1}-A_t | A_t} \le \frac{300n}{\eps}\left(\chi^2\left(p_{\mathcal{A}_{j(t+1)}},q_{\mathcal{A}_{j(t+1)}}\right) + 2\right), \label{eq:variancebound1} \\
		&\Var{B_{t+1}-B_t | B_t} \le \frac{50n}{\eps}\chi^2\left(p_{\mathcal{A}_{j(t+1)}},q_{\mathcal{A}_{j(t+1)}}\right). \label{eq:variancebound2}
		\end{align}
	\end{lemma}
	\begin{proof}
		We begin with the proof of (\ref{eq:variancebound1}).
		\begin{align}
		\Var{A_{t+1} - A_t | A_t} &= \sum_{i \in \mathcal{A}_{j(t+1)} } \Var{\frac{(X_{ij(t+1)} -p_{ij(t+1)})^2 - X_{ij(t+1)}}{q_{ij(t+1)}}} \label{eq:var1e1} \\
		&= \sum_{i \in \mathcal{A}_{j(t+1)} } \frac{\E\left[(X_{ij(t+1)} -p_{ij(t+1)})^4 + X_{ij(t+1)}^2 -2(X_{ij(t+1)} -p_{ij(t+1)})^2 X_{ij(t+1)}  \right]}{q_{ij(t+1)}^2} \\
		&= \sum_{i \in \mathcal{A}_{j(t+1)} } \frac{p_{ij(t+1)}(1+3p_{ij(t+1)}) + p_{ij(t+1)}^2 + p_{ij(t+1)} - 2p_{ij(t+1)} + 2p_{ij(t+1)}^2}{q_{ij(t+1)}^2} \label{eq:var1e3} \\
		&= 6 \sum_{i \in \mathcal{A}_{j(t+1)} } \frac{p_{ij(t+1)}^2}{q_{ij(t+1)}^2} \le \frac{300n}{\eps}\sum_{i \in \mathcal{A}_{j(t+1)} } \frac{p_{ij(t+1)}^2}{q_{ij(t+1)}} \\
		&\le \frac{300n}{\eps}\left(2 + \chi^2\left(p_{\mathcal{A}_{j(t+1)}},q_{\mathcal{A}_{j(t+1)}}\right)\right),
		\end{align}
		where (\ref{eq:var1e1}) holds because the random variables $\{X_{ij(t+1)}\}$ are independent due to Poissonization, TODO.
		Next we prove (\ref{eq:variancebound2}).
		\begin{align}
		\Var{B_{t+1} - B_t | B_t} &= \sum_{i \in \mathcal{A}_{j(t+1)} } \Var{\frac{(X_{ij(t+1)} -p_{ij(t+1)})\left(p_{ij(t+1)} - q_{ij(t+1)}\right)}{q_{ij(t+1)}}} \label{eq:var2e1} \\
		&= \sum_{i \in \mathcal{A}_{j(t+1)}} \frac{p_{ij(t+1)} (p_{ij(t+1)} - q_{ij(t+1)})^2}{q_{ij(t+1)}^2} \le \frac{50n}{\eps}\sum_{i \in \mathcal{A}_{j(t+1)}} \frac{(p_{ij(t+1)} - q_{ij(t+1)})^2}{q_{ij(t+1)}} \\
		&= \frac{50n}{\eps}\chi^2\left(p_{\mathcal{A}_{j(t+1)}},q_{\mathcal{A}_{j(t+1)}}\right),
		\end{align}
		TODO.
	\end{proof}
	
	
	\begin{lemma}[Applying Freedman's Inequality]
		In the equal case,
		$$\Pr\left[\abss{Z_m} > \frac{m\eps^2}{10}\right] \le TBF.$$
		In the far case,
		$$\Pr\left[\abss{Z_m - \E[Z_m]} > \frac{\E[Z_m]}{2}\right] \le TBF.$$
	\end{lemma}
	\begin{proof}
		First let us consider the equal case. In this case the sequence $\{B_t\}_{t \ge 0}$ is the zero martingale and the sequence $\{C_t\}_{t \ge 0}$ is also always 0 for all $t$. Hence, $\{Z_t\}_{t \ge 0}$ itself is a martingale. Let 
		\begin{align}
		V_t = \sum_{l=0}^{t-1} \Var{Z_{l+1} - Z_{l} | Z_l}.
		\end{align}
		From (\ref{eq:variancebound1}) of Lemma~\ref{lem:varbounds}, we get that
		\begin{align}
		V_m &\le \frac{300n}{\eps}\left(\sum_{l=0}^{m-1}\chi^2\left(p_{\mathcal{A}_{j(l+1)}},q_{\mathcal{A}_{j(l+1)}}\right) + 2m\right) = \frac{600nm}{\eps} = S.
		\end{align}
		with probability 1 because $p_{j(l+1)} = q_{j(l+1)}$ for all $l$. Also from (\ref{eq:incrementbound1}) and (\ref{eq:incrementbound2}) of Lemma~\ref{lem:incrementbounds} we have,
		\begin{align}
		\abss{Z_{t+1}-Z_t} \le \frac{102n\log^3 n}{\eps} = D.
		\end{align}
		Also let $\rad = m\epsilon^2/10$.
		Hence, we have
		\begin{align}
		\Pr\left[\abss{Z_m - Z_0} > \rad\right] &\le \Pr\left[\abss{Z_m - Z_0} > \rad \land V_m \le S \right] \\
		&\le \Pr\left[\abss{Z_m - Z_0} > \rad \land V_m \le S \land \tau_K \le m \right] + \Pr\left[\tau_k > m\right] \\
		&\le \Pr\left[\left(\exists \: t \le m \text{ s.t. } \abss{Z_t - Z_0} > \rad \land V_t \le S\right) \land \tau_K \le m \right] + \Pr\left[\tau_k > m\right] \\
		&\le \Pr\left[\exists \: t \le \tau_K \text{ s.t. } \abss{Z_t - Z_0} > \rad \land V_t \le S \right] + \Pr\left[\tau_k > m\right] \\
		&\le 2\exp\left(-\frac{\rad^2}{2(\rad D + S)}\right) + m\exp\left(-\frac{K^2\log^2 n}{2(1+K\log n)} \right),
		\end{align}
		TODO.
		For $m = C\frac{n\log^3 n}{\epsilon^2}$ for a big enough constant $C$, we have that
		\begin{align}
		\Pr\left[\abss{Z_m} > \rad\right] \le \frac{1}{n^2}.
		\end{align}
		
		Now, we consider the far case. We will get the desired statement by using tail inequalities for the random variables $A_m$ and $B_m$ that we obtain via Freedman's inequality. 
		
		
		
		
	\end{proof}

==> call-notes.tex <==
Markov chain testing notes:
Plan is to get rid of dependence on cover time for symmetric MC testing -> Intuition is that to distinguish between two chains, cover time not really necessary and a word of length 1/eps suffices. 

Approaches:
1. Get a word of length c*n*polylog(n)/eps and construct a subgraph over which a sub-MC can be defined. Argue that w.h.p this subgraph still has enough signal left to allow efficient testing.


Ideas: Expander graphs, Cheeger constant, Generalized problem with sub-stochastic symmetric matrices and per-vertex large mass guarantee.


One issue is what happens to the mapping we had earlier. i.e. can we really get i.i.d. samples from the subgraph's sub-stochastic matrix?

Q. Why is 1/eps sufficient to distinguish?


==> outline.tex <==
\begin{itemize}
 \item Intro
 \item Preliminaries
 \item Distance (part of preliminaries)
 \item Symmetric MC Upper bound
 \item Symmetric MC Lower bound
 \item Card Shuffling
\end{itemize}


\nick{For Costis, regarding different dependency on $\eps$ between results for (i) symmetric and (ii) sparse (card shuffling) Markov chains.}
We have $\frac{1}{\eps}$ dependency on $\eps$ in our upper and lower bound results for symmetric Markov chains, and $\frac{1}{\eps^2}$ dependency for the
identity testing of sparse Markov chains. One may think that the cause of this is the difference between Hellinger and total variation distances, but I think 
it is not the case. In fact, in both settings we can avoid using Hellinger distance in our definition of $\eps$.
I believe that the real cause is different definitions of the parameter $\eps$ in two settings. More specifically, $\eps$ is related in different ways
to the total variation distance between word distributions in two settings. In the symmetric setting, we have both $\dtv{\word{P}{\ell}}{\word{Q}{\ell}},
\hellinger{\word{P}{\ell}}{\word{Q}{\ell}} \ge 0.1$ for $\ell=\wTheta{\frac{1}{\eps}}$; while in the second setting $\eps=\dtv{\word{P}{n}}{\word{Q}{n}}$, 
where $n>>\ell\approx\frac{1}{\eps}$ (note that there is explicit polynomial inequality relation between $\eps$ and $n$ 
in our lower bounds, see Theorems~\ref{thm:symm-lower-bound} and Theorem~\ref{thm:sparse-lower-bound}). Because of this relation between $n$ and 
$\eps$, technically speaking, one cannot fix $n$ and study asymptotic dependency on $\eps$. On the other note, the different dependency on $\eps$ might be just 
a difference between more special setting of symmetric Markov chains versus general case. Indeed, we might expect better dependency on 
$\eps$ in a more specialized setting. 

\begin{itemize}
 \item General conventions
 \begin{itemize}
  \item vectors $\vect{v}$ (macro \verb|\vect{v}|)
  \item matrices $A$,$B$,$C$,$D$,$P$,$Q$,$M$.
  \item square root product of matrices and vectors $\srprod{P_t}{Q_t}$, $\srprod{\vect{p}}{\vect{q}}$ (macro \verb|\srprod{P}{Q}|) 
  \item $\onenorm{A}$ ``entrywise'' norm ($L_1$) of a matrix $A$ (macro \verb|\onenorm{A}|) 
  \item $\twonorm{A}$ ``entrywise'' norm ($L_2$) of a matrix $A$ (macro \verb|\twonorm{A}|) 
  \item $\onev$ - vector of all ones (macro \verb|\onev|)
  \item $\srprodt{\vect{p}}{\vect{q}}$  (macro \verb|\srprodt{\vect{p}}{\vect{q}}|)
  \item $\trans{\onev}\circ\srprod{P_t}{Q_t}\circ\onev$ (macro \verb|\trans{\onev}\circ\srprod{P_t}{Q_t}\circ\onev|)
  \item spectral radius $\specr{A}$ of a matrix $A$ (macro \verb|\specr{A}|)
  \item eigenvalues: $\eigi[1]\ge\dots\ge\eigi\ge\dots\ge\eigi[n]$ (macro \verb|\eigi[1],\eigi|)
	\item eigenvectors: $\eigvi[1],\dots,\eigvi,\dots\eigvi[n]$ (macro \verb|\eigvi[1],\eigvi|)
  \item $\dtv{\distr_1}{\distr_2}$ TV distance between $\distr_1$ and $\distr_2$ (macro \verb|\dtv{\distr_1}{\distr_2}|)
  \item $\hellinger{\distr_1}{\distr_2}$ Hellinger distance between $\distr_1$ and $\distr_2$ (macro \verb|\hellinger{\distr_1}{\distr_2}|)
 \end{itemize}
 \item Markov Chain
 \begin{itemize}
 \item number of states $n$
 \item number of steps $T$
 \item transition probabilities, $n\times n$ matrix $P,Q$ or $M$
 \item stationary distributions $\stationp$ and $\stationq$ of $P$ and $Q$ (macro \verb|\stationp , \staionq|)
 \item cover time $\covert{M}$ (macro \verb|\covert{M}|)
 \item hitting time $\hitt{M}$ (macro \verb|\hitt{M}|) 
 \item indexes of states $i,j$, index of time $t$
 \item word distributions $\word{P}{T}$ of length $T$ (macro \verb|\word{P}{T}|) 
 \item word distribution $\word{P}{\infty}$
 \item family of Marcov Chains $\MCfamily$ (macro \verb|\MCfamily|)
 \end{itemize}
 \item number of samples $m$
 \item Card Shuffling
 \begin{itemize}
 \item MC $\MCseqP$, each $P_t$ is a sparse matrix, $p_0$ is initial distribution. (macro \verb|\MCseqP, \MCseqQ|)
 \item $P\eqdef\MCseqP$, $Q\eqdef\MCseqQ$
 \item distance  $\dist{P}{Q}$ between words of length $n$ in $\MCseqP$ and $\MCseqQ$ models. 
 \item generic edge $e$
 \item set of all edges $E(t)$ from states at time $t$ to states at time $t+1$.
 \end{itemize}
 
\end{itemize}


==> pre-stoc18-version/distance.tex <==
%\label{sec:distance}
%As a first preliminary, we will define a distance between long-time evolving Markov chains $P$ and $Q$. 
We begin by considering the following simple question: how close is the behavior of two given Markov chains $P$ and $Q$?
A natural notion of distance would tell us how easy it is to distinguish which Markov chain $P$ or $Q$ a word $w=s_0\to s_1\cdots\to s_\ell$ of certain length $\ell$ was generated from. 
%In other words, our notion of distance is guided by the following question: 
%\begin{quote}
%Given a word $w=s_0\to s_1\cdots\to s_\ell$ generated from either Markov chain $P$ or Markov chain $Q$, how well can be distinguish which Markov chain $P$ or $Q$, the word $w$ came from?
%\end{quote}
The answer to this question is precisely captured by the total variation distance $\dtv{\word{P}{\ell}}{\word{Q}{\ell}}$ between {\em word distributions} 
$\word{P}{\ell}$, $\word{Q}{\ell}$ for words of length $\ell$ generated by Markov chains $P$, and respectively $Q$ (see Lemma \ref{lem:tv_lemma}). As a proxy for the total variation distance 
$\dtv{\word{P}{\ell}}{\word{Q}{\ell}}$, it is more convenient to use square of the Hellinger distance $\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}}$
or the closely related Bhattacharya coefficient\footnote{Hellinger distance is tightly related to the Bhattacharya coefficient between two distributions which is defined as
$BC(p,q) = \sum_{i \in [k]} \sqrt{p_i\cdot q_i}$. It captures similarity of two distributions and lies in $[0,1]$.}, which is useful for studying 
divergence of non-stationary and continuous Markov chains as was observed in~\cite{Kazakos78}. Similar to \cite{Kazakos78}, we can establish
nice recurrence relations for the Bhattacharya coefficient of two word distributions, which is captured by the matrix 
$\srprod{P}{Q}\eqdef\left[\sqrt{P_{ij}\cdot Q_{ij}}~ \right]_{i,j\in[n\times n]}$. %(see Appendix~\ref{app:sec_dist} for derivation of \eqref{eq:hellinger_square_algebraic} and missing proofs of the claims in this section)
%Precise calculation of $1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}}$. 
\be
\label{eq:hellinger_square_algebraic}
1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}}=\srprodt{\vect{p}}{\vect{q}}\circ \left(\srprod{P}{Q}\right)^{\ell} \circ \onev,
\ee
\begin{multline*}
1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}}=\sum_{w=s_0\ldots s_\ell}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}
=\trans{\left[\sum_{\substack{w=s_0\ldots s_{\ell}\\s_\ell=s}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{s\in[n]}\circ\onev\\
=\trans{\left[\sum_{r\in[n]}\sqrt{\Prlong[P]{r\to s}\Prlong[Q]{r\to s}}\sum_{\substack{w=s_0\ldots s_{\ell-1}\\s_{\ell-1}=r}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{s\in[n]}\circ\onev\\
=\trans{\left[\sum_{\substack{w=s_0\ldots s_{\ell-1}\\s_{\ell-1}=r}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{r\in[n]}\circ
\begin{bmatrix}
&\vdots&\\
\cdots&\sqrt{P_{rs}\cdot Q_{rs}}&\cdots\\
&\vdots&
\end{bmatrix}_{r,s\in[n\times n]}
\circ\onev
\\
=\trans{\left[\sum_{\substack{w=s_0\ldots s_{\ell-1}\\s_{\ell-1}=r}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{r\in[n]}\circ\srprod{P}{Q}\circ\onev
=\srprodt{\vect{p}}{\vect{q}}\circ \left(\srprod{P}{Q}\right)^{\ell} \circ \onev,
%\label{eq:hellinger_square_algebraic}
\end{multline*}
where $\vect{p}$ and $\vect{q}$ are vectors of initial distributions of $s_0$ over $[n]$, and 
$\srprod{\vect{p}}{\vect{q}}\eqdef\left[\sqrt{p_s\cdot q_s}\right]_{s\in[n]}$.
An important observation is that the distance between $\word{P}{\ell}$ and $\word{Q}{\ell}$ above depends on the initial distribution of the first state in $w$, and also the length 
$\ell$ of the word. 

\paragraph{Assumption on the starting state.} We study two reasonable models for the choice of the starting state: (i) a {\bf worst-case} model where
both $P$ and $Q$ begin from the same state $i$, which is chosen in adversarial manner to make $P$ and $Q$ look as much alike as possible;
(ii) an {\bf average-case} model, where the initial distributions $\vect{p}=\vect{q}$ for $P$ and $Q$ either are given to us, or are related to $P$ and $Q$ in 
some natural way\footnote{For example $\vect{p}$ and $\vect{q}$ could be respective stationary distributions of $P$ and $Q$. However, we still want the assumption
that $\vect{p}=\vect{q}$, as otherwise there might be another strategy to distinguish $P$ and $Q$ than observing a long stream of samples $w$ by making the decision 
right away based on one initial sample from $\vect{p}$. Example~\ref{fig:example3} illustrates how 
two Markov chains can produce very similar distributions of words $\word{P}{\ell},\word{Q}{\ell}$ starting from any state for some large $\ell$, and yet have vastly 
different stationary distributions.}. 
Given the assumption on the starting state we want to answer the question of what $\ell$ to pick, so 
that $\word{P}{\ell}$ and $\word{Q}{\ell}$ are far apart in squared Hellinger distance (say $\ge 0.50$). For the worst-case and average-case starting state models we respectfully get 
\begin{align}
\label{eq:forall_states_eigenvalue}
\min_{\ell>0} \quad\ell:& \quad\quad \forall i\in[n] && 0.5 \ge 1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}} = \onevti\circ \left(\srprod{P}{Q}\right)^{\ell} \circ \onev.\\
\min_{\ell>0} \quad\ell:  & && 0.5 \ge 1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}} = \srprodt{\vect{p}}{\vect{q}}\circ \left(\srprod{P}{Q}\right)^{\ell} \circ \onev \nonumber
\end{align}
Due to the relation between Hellinger and total variation distances, the inequality~\eqref{eq:forall_states_eigenvalue} holds
for $1-\dtv{\word{P}{\ell}}{\word{Q}{\ell}}$ but for a slightly different than $0.5$ constant. We call minimal $\ell$ that 
satisfies $\dtv{\word{P}{\ell}}{\word{Q}{\ell}}\ge\frac{2}{3}$ either for all starting states $i\in[n]$, or for fixed $\vect{p},\vect{q}$
the {\em minimal distinguishing length}. We note that \eqref{eq:forall_states_eigenvalue} gives us an estimate on $\ell$ up to a constant factor.

%Is there single natural parameter that captures closeness between $P$ and $Q$ without dependency on $\ell$ and initial state? 
We note that when $\ell$ is large, the behavior of RHS of~\eqref{eq:forall_states_eigenvalue} is governed by {\em the largest eigenvalue} 
$\eigi[1]=\specr{\srprod{P}{Q}}$ of $\srprod{P}{Q}$. 
%In a long run when $\ell\to\infty$ the parameter $\eigi[1]$ captures the rate at which the similarity between the two word distributions decreases (implying an increase in our ability to distinguish the two chains). 
By Perron-Frobenius theorem, we have that the largest eigenvalue of $\srprod{P}{Q}$ is non-negative and 
the corresponding left eigenvector $\eigvli[1]: \eigvlit[1]\circ\srprod{P}{Q}=\eigi[1]\cdot\eigvlit[1]$ 
has non-negative coordinates. In particular, if we choose initial distributions $\vect{p} = \vect{q}$ proportional to $\eigvli[1]$, then
\be
\trans{\vect{p}}\circ\left(\srprod{P}{Q}\right)^{\ell}\circ\onev=\eigi[1]^\ell\cdot\scalprod{\vect{p}}{\onev}=\eigi[1]^\ell.
\label{eq:largest_eigenvalue}
\ee

\begin{claim}
It is always true that $\eigi[1]=\specr{\srprod{P}{Q}}\le 1$. Moreover, $\eigi[1]=1$ iff $P$ and $Q$ have an identical connected component\footnote{or {\em essential 
communicating class} in the terminology of Book~\cite{LPLbook}}.
\label{cl:eigval_less_than_one}
\end{claim} 
\begin{proof}
	Note that $\frac{P+Q}{2}$ is a stochastic matrix that 
	entry-wise dominates matrix $\srprod{P}{Q}$ with non-negative entries. Therefore,
	$
	\eigi[1]\cdot\scalprod{\eigvli[1]}{\onev}=\eigvlit[1]\circ\srprod{P}{Q}\circ\onev\le\eigvlit[1]\circ\left[\frac{P+Q}{2}\right]\circ\onev
	=\eigvlit[1]\circ\onev=\scalprod{\eigvli[1]}{\onev},
	$
	where $\onev$ is vector with all $1$ entries. We get $\eigi[1]\le 1$, since $\scalprod{\eigvli[1]}{\onev}>0$.
	
	For the case of equality, if $P$ and $Q$ have the same connected component $C$, then matrix $\srprod{P}{Q}$ has the same transition 
	probabilities as Markov chains $P$ and $Q$ restricted to the vertices of $C$. We note that $C$ is a stochastic 
	matrix and, therefore, its largest positive eigenvalue is one. Hence, $\specr{\srprod{P}{Q}}\ge\specr{C} = 1.$
	
	If $\specr{\srprod{P}{Q}}=1$, we apply Perron-Frobinius theorem to $\srprod{P}{Q}$ to get  
	that the largest eigenvalue $\eigi[1]=\specr{\srprod{P}{Q}}=1$ has corresponding (left) eigenvector $\eigvli[1]$ with non-negative entries. 
	Similar to the proof of Claim~\ref{cl:eigval_less_than_one} we observe that $\eigvlit[1]\circ\left(\frac{P+Q}{2}-\srprod{P}{Q}\right)\circ\onev=0$, 
	and all entries of the matrix in this expression are non-negative. This implies that $P_{ij}=Q_{ij}$ for every strictly positive coordinates 
	$i$ of the eigenvector $\eigvli[1]$ and any $j\in[n]$. Since $\eigvlit[1]\circ\srprod{P}{Q}=\eigvlit[1]$, we also have $P_{ij}=Q_{ij}=0$ for any positive 
	coordinate $i$ and zero coordinate $j$ of eigenvector $\eigvli[1]$. Therefore, the set of vertices corresponding to positive coordinates of $\eigvli[1]$ 
	form a component (which might have more than one connected component of $P$ and $Q$) such that $P=Q$ on these vertices.  
\end{proof}

We consider the quantity $\eps\eqdef \mathbf{1-\specr{\srprod{P}{Q}}}$ as a proxy for the closeness of Markov chains $P$ and $Q$. 
In particular in \eqref{eq:forall_states_eigenvalue} if $\vect{p} = \vect{q}$ is proportional to $\eigvli[1]$, then 
$\ell\cdot\ln(1-\eps)\le\ln 0.5\implies\ell\ge\frac{\ln 2}{2\eps}$. This shows that in worst-case we need to observe a trajectory of length at least $\Omega(1/\eps)$  before we can satisfactorily distinguish the two chains.
%Also, $\eigi[1]=1$ means that $P$ and $Q$ are indistinguishable at least for a starting state in some connected component of $P$ and $Q$.
Note however that, in general, $\ell$ might need to be larger than 
$O(\frac{1}{\eps})$ as is illustrated in Example~\ref{fig:example2}. 
In the remainder of this section and the following section we study an interesting special case of symmetric Markov chains that avoids such irregular behavior and 
dependency on the starting state.


\paragraph{Symmetric Markov Chains.} The stationary distribution for any symmetric Markov chain is the uniform distribution over all states. 
In this case the starting distributions in the average-case part of equation~\eqref{eq:forall_states_eigenvalue} are $\vect{p}=\vect{q}=\frac{1}{n}\onev$.
%\be
%\min_{\ell>0} \quad\ell: \quad\quad\quad 0.9\ge 1-\hellingersq{\word{P}{\ell}}{\word{Q}{\ell}} = \frac{1}{n}\onevt\circ \left(\srprod{P}{Q}\right)^{\ell} \circ \onev.
%\label{eq:average_states_eigenvalue}
%\ee
%When we start observing a phenomenon 
%obeying Markov Chain $P$, it is reasonable instead of the worst-case assumption on the initial state assume that initial state is distributed 
%according to the stationary distribution of $P$ and measure the distance between $P$ and $Q$ for a random starting state. A natural question here is 
%what $\ell$ is enough to distinguish $P$ and $Q$ with significant probability, i.e.,
%\[
%\frac{1}{2}\ge 1-\hellingersq{\word{P}{\ell+1}}{\word{Q}{\ell+1}} = \frac{1}{n}\onevt\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev
%\]
In this setting of symmetric Markov chains, we can provide sharp bounds on the minimal distinguishing length $\ell$.
\begin{claim}
The necessary and sufficient distinguishing length $\ell$, which allows to distinguish $P$ vs. $Q$ with high probability, 
is $\wTheta{\frac{1}{\eps}}$ (up to a $\log n$ factor), where $\eps=1-\specr{\srprod{P}{Q}}$ under both worst-case and average-case 
assumptions for the starting state.
\label{cl:symm_spectrum}
\end{claim}
\begin{proof}
	We first consider the average-case model for the starting state. Note that $\srprod{P}{Q}$ is a symmetric matrix. 
	Let $\eigvi[1],\dots,\eigvi[n]$ be normalized orthogonal eigenvectors of $\srprod{P}{Q}$, corresponding to 
	real $\eigi[1]\ge\dots\ge\eigi[n]$ eigenvalues. Then for RHS of \eqref{eq:forall_states_eigenvalue} we have
	\be
	\frac{1}{n}\onevt\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev=\frac{1}{n}\onevt\circ\left(\sum_{i=1}^n\eigi\cdot\eigvi\circ\eigvit\right)^\ell\circ\onev
	=\sum_{i=1}^n\eigi^\ell\cdot\frac{1}{n}\iprod{\onev}{\eigvi}^2=(*)
	\label{eq:definition_star}
	\ee
	Now we can write an upper and lower bound on $(*)$ in terms of $\eigi[1]^\ell$ (assuming that $\ell$ is even):
	\begin{multline*}
	\frac{\eigi[1]^\ell}{n}=\frac{\eigi[1]^\ell}{n}\twonorm{\eigvi[1]}^2\le\eigi[1]^\ell\cdot\frac{1}{n}\onenorm{\eigvi[1]}^2
	\le(*) \le
	\sum_{i=1}^n\eigi^\ell\cdot\frac{1}{n}\onenorm{\eigvi}^2\le\sum_{i=1}^n\eigi^\ell\cdot\twonorm{\eigvi}^2=\sum_{i=1}^n\eigi^\ell\le n\cdot\eigi[1]^\ell,  
	\end{multline*}
	where in the second inequality we used Perron-Frobenius theorem stating that all coordinates of $\eigvi[1]$ are non negative. 
	Consequently, these bounds imply that $\ell=\Theta\left(\frac{1}{\eps}\right)$ up to a $\log n$ factor, if $\specr{\srprod{P}{Q}}=\eigi[1]=1-\eps$. 
	I.e., $\ell=\wTheta{\frac{1}{\eps}}$.
	
	For the worst-case assumption on the starting state, it is sufficient to show an upper bound $\ell=\Ocomplex{\frac{\log n}{\eps}}$. 
	In this case~\eqref{eq:definition_star} becomes
	\[
	\onevti\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev=\sum_{i=1}^n\eigi^\ell\cdot\iprod{\onevi}{\eigvi}\cdot\iprod{\onev}{\eigvi}
	\le\sum_{i=1}^n|\eigi|^\ell\cdot\infnorm{\eigvi}\cdot\onenorm{\eigvi}
	\le\sum_{i=1}^n|\eigi|^\ell\cdot \sqrt{n}\le n^{1.5}\cdot\eigi[1]^\ell,
	\]
	since $\onenorm{\eigvi}\le\sqrt{n}\twonorm{\eigvi}=\sqrt{n}$, and $\infnorm{\eigvi}\le\twonorm{\eigvi}=1$.
\end{proof}

%\label{cl:symm_spectrum_worst-case}
We note that, if one could pick the starting state instead of working with average-case or worst-case assumptions of Claim~\ref{cl:symm_spectrum}, then $\ell$ can be much smaller (see Example~\ref{fig:example5}). Claim~\ref{cl:symm_spectrum} gives a strong evidence that $\dist{P}{Q}\eqdef 1-\specr{\srprod{P}{Q}}$ 
is a meaningful and important parameter that captures closeness between $P$ and $Q$. In the following section we will use it as analytical proxy for the distance between 
Markov Chains\footnote{In general this notion of distance should be used with care. One thing about parameter $\dist{P}{Q}=1-\specr{\srprod{P}{Q}}$, is that it is not a metric. In particular, $
\dist{P}{Q}$ violates the triangle inequality ($\dist{M_1}{M_2}=\dist{M_2}{M_3}=0,$ but $\dist{M_1}{M_3}>0$ for some $M_1,M_2,M_3$) as is illustrated by Example~\ref{fig:example1}. 
We note that this problem can only appear for reducible chains, as is shown in Claim~\ref{cl:eigval_less_than_one}. Also it is not always possible to extend the sharp bounds on $\ell$ of 
Claim~\ref{cl:symm_spectrum} from symmetric Markov chains to non-symmetric Markov chains, even if both MC have the uniform distribution as their stationary distribution (see Example~\ref{fig:example4})
}.

%
%
%
%For both General and Symmetric Markov chains, $\eps=1-\specr{\srprod{P}{Q}}$ is a meaningful and important parameter that captures closeness between $P$ and $Q$.
%In the following sections we will use it as proxy for the distance between Markov Chains. 
%
%
%\paragraph{Average-case starting state.} Another reasonable approach is to assume that both Markov chains $P$ and $Q$ had enough time to mix before 
%our observation and, therefore, the initial distributions $\vect{p},\vect{q}$ for the starting state in $P$ and $Q$ are the respective stationary distributions.  
%
%
%
%However, there is a simple condition that quantifies how big the gap between the lower bound
%on $\ell$ from \eqref{eq:largest_eigenvalue} and an upper bound that is sufficient for \eqref{eq:forall_states_eigenvalue} could be: if the right eigenvector $\eigvi[1]$ of $\srprod{P}{Q}$
%($\srprod{P}{Q}\circ\eigvi[1]=\eigi[1]\cdot\eigvi[1]$) has bounded gap between its largest and smallest coordinates, i.e., 
%$\frac{\max_{i}\iprod{\eigvi[1]}{\onevi}}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}\le\kappa$, then 
%\begin{multline*}
%\forall i\in[n]\quad\quad\quad\quad \onevti\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev  \le  
%\onevti\circ\left(\srprod{P}{Q}\right)^{\ell}\circ\frac{\eigvi[1]}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}\\
%=\frac{\iprod{\onevi}{\eigvi[1]}\eigi[1]^\ell}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}
%\le\frac{\eigi[1]^\ell\max_{i}\iprod{\onevi}{\eigvi[1]}}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}=\kappa\cdot\eigi[1]^\ell
%\end{multline*}
%
%
%%We present a novel definition of distance between two Markov chains which captures the difference in the words produced by the chains. 
%%Let $P$ and $Q$ be two Markov chains defined on a set $S$ of $n$ states. We also use $P$ to refer to the transition 
%%matrix of the Markov chain $P$. 
%%
%%Consider the matrix $\srprod{P}{Q}$. The distance between Markov chains $P$ and $Q$ is defined as $1-\specr{\srprod{P}{Q}}$. 
%
%
%\nick{Selling new distance (plan):}
%\begin{itemize}
%\item Given two Markov Chains $P$, $Q$ how to distinguish them with $m$ consequent samples?
%%We want a notion of distance that allows us to say which MC $P$ or $Q$ the word $w$ of certain length $\ell$ was generated from. This is precisely captured by total variation 
%%distance $\dtv{\word{P}{\ell}}{\word{Q}{\ell}}$ between word distributions of length $\ell$. This notion depends on the initial distribution of the first state in $w$, and 
%%also length $\ell$ of the word. Is there single natural parameter that captures closeness between $P$ and $Q$ without dependency on $\ell$ and initial state? 
%%\item As a proxy for $\dtv{\word{P}{\ell+1}}{\word{Q}{\ell+1}}$ we use $\hellingersq{\word{P}{\ell+1}}{\word{Q}{\ell+1}}$. 
%%Precise calculation of $1-\hellingersq{\word{P}{\ell+1}}{\word{Q}{\ell+1}}$. \nick{See section~\ref{sec:hellinger_sq_precise}.}
%%\begin{remark}
%%The Bhattacharya coefficient between two probability distributions $p$ and $q$ supported over $X$ is defined as
%%$BC(p,q) = \sum_{x \in X} \sqrt{p(x)q(x)}$
%%The Bhattacharya coefficient captures the similarity of two distributions under the Hellinger squared distance. 
%%We will show that Hellinger similarity between two Markov chains has a nice form which is captured by the matrix $\srprod{P}{Q}\eqdef\left[\sqrt{P_{ij}\cdot Q_{ij}}~ \right]_{i,j\in[n\times n]}$.
%%\end{remark} 
%
%%For the regime when $\ell$ is large, the behavior of RHS of the above expression is governed by the largest eigenvalue $\eigi[1]$ of 
%%$\srprod{P}{Q}$. In a long run when $\ell\to\infty$ the parameter $\eigi[1]$ captures the rate at which we can distinguish $P$ and $Q$.
%%We recall that by Perron-Frobenius theorem the largest eigenvalue of $\srprod{P}{Q}$ is positive (assuming non-degeneracy conditions on $\srprod{P}{Q}$) 
%%and corresponding eigenvector $\eigvli[1]: \eigvlit[1]\circ\srprod{P}{Q}=\eigi[1]\cdot\eigvlit[1]$ has all positive coordinates. 
%%In particular, if initial state is chosen from the distribution $\vect{p}$ proportional to $\eigvli[1]$, then
%%\be
%%\trans{\vect{p}}\circ\left(\srprod{P}{Q}\right)^{\ell}\circ\onev=\eigi[1]^\ell\cdot\scalprod{\vect{p}}{\onev}=\eigi[1]^\ell\le \frac{1}{2},
%%\label{eq:largest_eigenvalue}
%%\ee
%%If $\eigi[1]=1-\eps$ it means that $\ell\cdot\log(1-\eps)\le\log\frac{1}{2}\implies\ell\ge\frac{\log 2}{2\eps}$. Note that in general $\ell$ might need
%%to be much larger than this bound, as is illustrated in Example 1. However, there is a simple condition that quantifies how big the gap between the lower bound
%%on $\ell$ from \eqref{eq:largest_eigenvalue} and an upper bound that is sufficient for \eqref{eq:forall_states_eigenvalue} could be: if the right eigenvector $\eigvi[1]$ of $\srprod{P}{Q}$
%%($\srprod{P}{Q}\circ\eigvi[1]=\eigi[1]\cdot\eigvi[1]$) has bounded gap between its largest and smallest coordinates, i.e., 
%%$\frac{\max_{i}\iprod{\eigvi[1]}{\onevi}}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}\le\kappa$, then 
%%\begin{multline*}
%%\forall i\in[n]\quad\quad\quad\quad \onevti\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev  \le  
%%\onevti\circ\left(\srprod{P}{Q}\right)^{\ell}\circ\frac{\eigvi[1]}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}\\
%%=\frac{\iprod{\onevi}{\eigvi[1]}\eigi[1]^\ell}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}
%%\le\frac{\eigi[1]^\ell\max_{i}\iprod{\onevi}{\eigvi[1]}}{\min_{j}\iprod{\eigvi[1]}{\onevi[j]}}=\kappa\cdot\eigi[1]^\ell
%%\end{multline*}
   %
%%where $V\circ\Lambda\circ \inv{V}$ is eigenvalue decomposition of matrix $\srprod{P}{Q}$: columns of $V$ are right eigenvectors of $\srprod{P}{Q}$ and $\Lambda$ is diagonal matrix
%%with eigenvalues of $\srprod{P}{Q}$; $\eigvi$ and $\eigvli$ are corresponding to $\eigi$ right and left eigenvectors of $\srprod{P}{Q}$ normalized such that $\scalprod{\eigvli}{\eigvi}=1$. 
 %%
%%columns of matrix $U$ are composed of left eigenvectors $\eigvlit:\eigvlit\circ\srprod{P}{Q}=\eigi\cdot\eigvlit$, columns of matrix $V$ are right eigenvectors 
%%$\eigvi:\srprod{P}{Q}\circ\eigvi=\eigi\cdot\eigvi$, and $\Lambda$ is diagonal matrix composed of eigenvalues of $\srprod{P}{Q}$.
%%
%%first inequality holds true as $\scalprod{\eigvi}{\eigvi}=\twonorm{\eigvi}=1$, to get the first equality
%%we just rewrite $\srprodt{\vect{p}}{\vect{q}}$ in the eigenvector basis of $\srprod{P}{Q}$.
%
%\item Symmetric Markov Chains. 
%%In this case uniform distribution is stationary for both $P$ and $Q$. Hence, when we start observing a phenomenon 
%%obeying Markov Chain $P$, it is reasonable instead of the worst-case assumption on the initial state assume that initial state is distributed 
%%according to the stationary distribution of $P$ and measure the distance between $P$ and $Q$ for a random starting state. A natural question here is 
%%what $\ell$ is enough to distinguish $P$ and $Q$ with significant probability, i.e.,
%%\[
%%\frac{1}{2}\ge 1-\hellingersq{\word{P}{\ell+1}}{\word{Q}{\ell+1}} = \frac{1}{n}\onevt\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev
%%\]
%%Note that $\srprod{P}{Q}$ is symmetric matrix and therefore we have
%%\[
%%\frac{1}{n}\onevt\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev=\frac{1}{n}\onevt\circ\left(\sum_{i=1}^n\eigi\cdot\eigvi\circ\eigvit\right)^\ell\circ\onev
%%=\sum_{i=1}^n\eigi^\ell\cdot\frac{1}{n}\iprod{\onev}{\eigvi}^2=(*)
%%\]
%%Now we can write upper and lower bound on $(*)$ in terms of $\eigi[1]^\ell$ (assume that $\ell$ is even):
%%\begin{multline*}
%%\frac{\eigi[1]^\ell}{n}=\frac{\eigi[1]^\ell}{n}\twonorm{\eigvi[1]}^2\le\eigi[1]^\ell\cdot\frac{1}{n}\onenorm{\eigvi[1]}^2
%%\le(*)\le
%%\sum_{i=1}^n\eigi^\ell\cdot\frac{1}{n}\onenorm{\eigvi}^2\le\sum_{i=1}^n\eigi^\ell\cdot\twonorm{\eigvi}^2=\sum_{i=1}^n\eigi^\ell\le n\cdot\eigi[1]^\ell,  
%%\end{multline*}
%%where in the second inequality we used Perron-Frobenius theorem stating that all coordinates of $\eigvi[1]$ are non negative. 
%%Consequently, these bounds imply that $\ell=\Theta\left(\frac{1}{\eps}\right)$ up to a $\log n$ factor, if $\eigi[1]=1-\eps$. I.e.,
%%$\ell=\wTheta{\frac{1}{\eps}}$. Noticeably, similar upper bound on $\ell$ still holds for the worst-case starting state. In this case we have:
%%$(*)=\onevti\circ \left(\srprod{P}{Q}\right)^{\ell}\circ\onev$
%%\[
%%(*)=\sum_{i=1}^n\eigi^\ell\cdot\iprod{\onevi}{\eigvi}\cdot\iprod{\onev}{\eigvi}
%%\le\sum_{i=1}^n\eigi^\ell\cdot\infnorm{\eigvi}\cdot\onenorm{\eigvi}
%%\le\sum_{i=1}^n\eigi^\ell\cdot n\twonorm{\eigvi}^2\le n^2\cdot\eigi[1]^\ell.
%%\]
%%
%%For both General and Symmetric Markov chains, $\eps=1-\specr{\srprod{P}{Q}}$ is a meaningful and important parameter that captures closeness between $P$ and $Q$.
%%In the following sections we will use it as proxy for the distance between Markov Chains. 
%\item Time dependent Markov Chains. We observe a few i.i.d. runs.
%\end{itemize}
%
%
%\subsection{Bhattacharya coefficient}

\paragraph{Fixed word length.} In some applications the length $\ell$ of the observed word might be given a priori. One such example corresponds to card riffle shuffle, 
where the random choices in the process can be described (see Section~\ref{sec:shuffle} for more detail) as a Markov chain over $O(n^2)$ states ($n=52$ for the card deck), where the
process terminates after $\ell=n$ steps. In this case we can expect a few i.i.d. samples of length-$\ell$ words. For such examples and more generally for the Markov Chains with 
a specified number of steps $T$ it is natural to define
$
\dist{P}{Q}\eqdef\dtv{\word{P}{T}}{\word{Q}{T}}.
%\label{eq:def_dist_fixed_time}
$
Note that now the distance $\dist{P}{Q}$ satisfies triangle inequality. Moreover, due to the relation between Hellinger and total variation distances we 
can estimate $1-\frac{\distsq{P}{Q}}{2}\ge 1-\hellingersq{\word{P}{T}}{\word{Q}{T}}$, where the RHS term admits a nice analytical expression similar 
to \eqref{eq:hellinger_square_algebraic}.



%\subsection{Hellinger Squared Distance between the Word Distributions}
%\label{sec:hellinger_sq_precise}
%Consider any Markov chain $P$. The sequence of states seen in any given run of $P$ is called a word generated by $P$. 
%The words of length $t$ generated by Markov chain $P$ have a distribution which is denoted by $\word{P}{t}$. We will 
%now derive an expression for $\hellinger{\word{P}{t}}{\word{Q}{t}}$.  We define $\hellinger{\word{P}{t}}{\word{Q}{t}}_s$ as follows
%$$HS_s\left(\word{P}{t},\word{Q}{t}\right) = \sum_{\substack{w~:~s_1\ldots s_t, \\ \text{s.t. } w_t=s}}  \sqrt{\Pr_P(w)\Pr_Q(w)}$$
%Note that the Hellinger squared similarity (or Bhattacharya coefficient) is,
%$$1-\hellingersq{\word{P}{t}}{\word{Q}{t}} = \sum_{s \in S} HS_s\left(\word{P}{t},\word{Q}{t}\right).$$
%We also define the $n$-vector $\vec{HS}\left(\word{P}{t},\word{Q}{t}\right)$ as,
%$$\vec{HS}\left(\word{P}{t},\word{Q}{t}\right) = \left(HS_s\left(\word{P}{t},\word{Q}{t}\right) \right)_{s \in S}.$$
%Therefore 
%$$1-\hellingersq{\word{P}{t}}{\word{Q}{t}} = \vec{HS}\left(\word{P}{t},\word{Q}{t}\right)^T \circ \onev.$$
%With these definitions in mind, we begin by considering $HS_s\left(\word{P}{t},\word{Q}{t}\right)$ for some state $s \in S$.
%\begin{eqnarray}
%&& HS_s\left(\word{P}{t},\word{Q}{t}\right) = \sum_{\substack{w~:~s_1\ldots s_t, \\ \text{s.t. } s_t=s}}  \sqrt{\Pr_P(w)\Pr_Q(w)} \\
%&=& \sum_{w~:~s_1\ldots s_{t-1}}  \sqrt{\Pr_P(s_1\ldots s_{t-1})\Pr_Q(s_1\ldots s_{t-1})P(s_{t-1},s)Q(s_{t-1},s)} \\
%&=& \vec{HS}\trans{\left(\word{P}{t-1},\word{Q}{t-1}\right)} \circ \srprod{P}{Q}^{(s)} \\
%\end{eqnarray}
%where $\srprod{P}{Q}^{(s)}$ denotes the $s^{th}$ column of the $\srprod{P}{Q}$ matrix. Therefore we arrive at the following recurrence.
%\begin{eqnarray*}
%\vec{HS}\trans{\left(\word{P}{t},\word{Q}{t}\right)} = \vec{HS}\trans{\left(\word{P}{t-1},\word{Q}{t-1}\right)} \circ \srprod{P}{Q}
%\end{eqnarray*}
%The above recurrence implies,
%$$\vec{HS}\trans{\left(\word{P}{t},\word{Q}{t}\right)} = \vec{HS}\trans{\left(\word{P}{1},\word{Q}{1}\right)} \circ \left(\srprod{P}{Q}\right)^{t-1}$$
%Therefore, 
%\begin{equation}
%\label{eq:dist}
%1-\hellingersq{\word{P}{t}}{\word{Q}{t}} = \srprodt{\vect{p}}{\vect{q}}\circ \left(\srprod{P}{Q}\right)^{t-1} \circ \onev
%\end{equation}





\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		%\includegraphics[scale=0.16]{diagrams/example1.jpg}
		%\includegraphics[width=\textwidth]{diagrams/Example_1.png}
		\includegraphics[width=0.9\textwidth]{Ex1.png}
		\caption{$\dist{M_1}{M_2}=1-\specr{\srprod{M_1}{M_2}}$ is not a metric. $\dist{M_1}{M_2}=\dist{M_2}{M_3}=0,$ but 
			$\dist{M_1}{M_3}> 0$.}
		\vspace{3ex}
		\label{fig:example1}
	\end{subfigure}
	\hspace{5pt}	
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=0.9\textwidth]{Ex5.png}
		\caption{After one step from state $4$, we would know if $w\sim P$, or $w\sim Q$. 
			If $w$ starts from any other state $s_0\neq 4$, it would take many steps.}
		\vspace{3ex}
		\label{fig:example5}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=0.9\textwidth]{Ex2.png}
		\caption{To distinguish $P$ vs. $Q$ walking from a random state we need $\Omega(n)$ steps, but $\dist{P}{Q}=1$.}
		\label{fig:example2}
	\end{subfigure}
	\hspace{3pt}	
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=0.9\textwidth]{Ex3.png}
		\caption{$\dist{P}{Q}=o(1)$, stationary distributions $\vect{q}_0,\vect{p}_0$ 
			are different: $\dtv{\vect{q}_0}{\vect{p}_0}=1-o(1)$.}
		\label{fig:example3}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=0.9\textwidth]{Ex4.png}
		\caption{$\dist{P}{Q}=1$. Uniform is stationary	for both $P$ and $Q$. 
			On average $\Omega(n)$ steps to tell $P\neq Q$.}
		\label{fig:example4}
	\end{subfigure}
	
	\vspace{5ex}
	\begin{tabular}{ | l | p{0.8\textwidth} |}
		\cline{2-2}
		%\multicolumn{1}{|c|}{Description}
		
		\multicolumn{1}{c|}{} &  \multicolumn{1}{c|}{Description} \\ \hline
		Example~\ref*{fig:example1} & Two disjoint connected components. \\ \hline
		Example~\ref*{fig:example5} & $Q$ -- clique $K_n$; $P$ -- clique $K_{n-1}$ and disjoint vertex.
		Eigenvalue of $\srprod{P}{Q}$: $\eigi[1]=\sqrt{\frac{n-1}{n}}=1-o(1)$, 
		$\eigi[2]=\sqrt{\frac{1}{n}}$, $\eigi[3]=\cdots=\eigi[n]=0$	\\  \hline												
		Example~\ref*{fig:example2} & $P$ -- oriented cycle, $Q$ -- cycle with one link substituted by a loop.\\ \hline
		Example~\ref*{fig:example3} & $Q$ -- oriented cycle with edge $e=(v_1v_2)$ substituted by a loop at $v_1$; 
		$P$ is almost like $Q$, but $e$ has weight $\frac{1}{\sqrt{n}}$, loop at $v_1$ 
		has weight $1-\frac{1}{\sqrt{n}}$. Stationary distributions: $\vect{q}_0=\trans{(1,0,\cdots,0)}$ 
		and $\vect{p}_0=\trans{(\frac{\sqrt{n}}{n+\sqrt{n}-1},\frac{1}{n+\sqrt{n}-1},\dots,\frac{1}{n+\sqrt{n}-1})}$. 
		$\specr{\srprod{P}{Q}}=\sqrt{1-\frac{1}{\sqrt{n}}}$.   \\  \hline
		Example~\ref*{fig:example4} & Two oriented cycles $P\eqdef s_1\to s_2\to\cdots\to s_n\to s_1$ and 
		$Q\eqdef s_1\to s_3\to s_4\cdots\to s_n\to s_2\to s_1$.	\\  \hline											
	\end{tabular}
	
	\caption{Examples.} \label{fig:examples}
\end{figure}

%\subsection{Examples}
%
%
%\begin{example}
%\label{example:two_components}
%Two disjoint connected components: $\dist{M_1}{M_2}=1-\specr{\srprod{M_1}{M_2}}$ is not a metric $1-\specr{\srprod{M_1}{M_2}}=1-\specr{\srprod{M_2}{M_3}}=0,$ but 
%$1-\specr{\srprod{M_1}{M_3}}> 0$.
%\end{example}
%
%\begin{example}
%\label{example:starting_position}
%Non symmetric Markov chains: importance of starting position. 
%$P$ -- oriented ring, $Q$ -- the same ring but with a state that has heavy self-loop on one of the vertices. 
%Distance $\dist{P}{Q}=1-\specr{\srprod{P}{Q}}$ can be $0$. However, from some states it takes up to $\Omega(n)$ steps to reach 
%vertex with the loop to see the difference.
%
%\begin{figure}[H]
%	\centering
%		\includegraphics[scale=0.40]{diagrams/example2.jpg}
%	\caption{Example 2.}
%	\label{fig:example2}
%\end{figure}
%\end{example}
%
%\begin{example}
%\label{example:stationary_testing}
%Non symmetric MC: small difference between $P$ and $Q$ ($\dist{\word{P}{\ell}}{\word{Q}{\ell}}$ is small), but stationary distributions $\vect{p}_0$ and $\vect{q}_0$
%are vastly different. $Q$ - a ring with an edge $e=(v_1v_2)$ is removed, $v_1$ has a self-loop instead; $P$ - a similar ring with a loop, but $e$ is not removed but has a lighter
%weight of $\frac{1}{\sqrt{n}}$, while self-loop at $v_1$ has a weight of $1-\frac{1}{\sqrt{n}}$. Stationary distributions: $\vect{q}_0=\trans{(1,0,\cdots,0)}$ and
%$\vect{p}_0=\trans{(\frac{\sqrt{n}}{n+\sqrt{n}-1},\frac{1}{n+\sqrt{n}-1},\dots,\frac{1}{n+\sqrt{n}-1})}$, while $\specr{\srprod{P}{Q}}=\sqrt{1-\frac{1}{\sqrt{n}}}$.   
%%\begin{figure}[H]
%	%\centering
%		%\includegraphics[scale=0.40]{diagrams/example3.jpg}
%	%\caption{Example 3.}
%	%\label{fig:example3}
%%\end{figure}
%
%\end{example}
%\begin{example}
%\label{example:same_stationary_large_dist}
%Non symmetric MC: same stationary (Uniform) distribution, $\dist{P}{Q}=1$, at average it takes $\Omega(n)$ steps to distinguish whether $P=Q$, or not.
%Two oriented cycles, 
%\[
%P\eqdef s_1\to s_2\to\cdots\to s_n\to s_1\quad\quad Q\eqdef s_1\to s_3\to s_4\cdots\to s_n\to s_2\to s_1.
%\]
%%\begin{figure}[H]
%	%\centering
%		%\includegraphics[scale=0.40]{diagrams/example4.jpg}
%	%\caption{Example 4.}
%	%\label{fig:example4}
%%\end{figure}
%\end{example}
%\begin{example}
%\label{example:symmetric}
%Symmetric Markov chains: $Q$ -- complete graph $Q_{ij}=1/n$; $P$ -- clique and disjoint vertex $P_{ij}=\frac{1}{n-1}, i,j\in[n-1]$, $P_{in}=P_{ni}=0, i\in[n-1],$ and 
%$P_{nn}=1$. Then $\eigi[1]=\sqrt{\frac{n-1}{n}}= 1 - \frac{1}{2n}+O(n^2)$, $\eigi[2]=\sqrt{\frac{1}{n}}$, $\eigi[3]=\cdots=\eigi[n]=0$. If Markov Chain starts from state $1$, 
%after one transition we would know almost certainly whether $w\sim P$, or $w\sim Q$. On the other hand, if $w$ starts from any other state, then it would take us about $n$ 
%observations to tell whether $w\sim P$, or $w\sim Q$. If we start from a random state, again we would need about $n$ steps to distinguish $P$ vs. $Q$.
%%\begin{figure}[H]
%	%\centering
%		%\includegraphics[scale=0.40]{diagrams/example5.jpg}
%	%\caption{Example 5.}
%	%\label{fig:example5}
%%\end{figure}
%\end{example}



==> pre-stoc18-version/intro.tex <==
We formulate theories about the laws that govern physical phenomena by making observations and testing them against our hypotheses. A common scenario is when our observations can be reasonably modeled as i.i.d. samples from a distribution that we are trying to understand. This is the setting tackled by most classical work in Statistics. Of course, having access to i.i.d. samples from a distribution is rare and quite commonly a mere approximation of reality. We typically only have access to approximate samples from a stationary distribution, sampled by a Markov chain whose transition matrix/kernel is unknown to us and which can only be observed for some finite time horizon. In fact, to the best of our knowledge, the underlying Markov chain may not even be rapidly mixing, so there is no guarantee that we will ever see samples that are approximately distributed according to the stationary distribution.

These issues are exacerbated in high-dimensional settings, e.g., when observing the configurations of a deck of cards or a weather system, where it may also be completely impractical to work with the high-dimensional stationary distribution itself. Moreover, there are several ways to sample a stationary distribution, so it may be more important to know how it comes to be sampled. For all  these considerations, it may be both more interesting and more practical to understand the ``mechanics'' of the process that generates our observations, namely the transition matrix/kernel of the Markov chain whose evolution we get to observe.

Motivated by these considerations, in this paper we study the problem of testing the identity of Markov chains. We are given access to a {\em single} trajectory $X_0, X_1,\ldots,X_t,\ldots$ of some {\em unknown} Markov chain ${\cal M}$ over some finite state space $[n]$, and we want to test the identity of ${\cal M}$ to some {\em given} Markov chain ${\cal M}'$. Importantly, we do not get to control the distribution of the starting state $X_0$, and we can only observe a single trajectory of ${\cal M}$, i.e. we cannot restart the Markov chain. What could we hope to achieve?

If there is any difference in the transition matrices of $\cal M$ and $\cal M'$, one would think that we would {\em ultimately} be able to identify it by observing a sufficiently long trajectory. This is certainly true if the transition matrices of the two chains differ at a state that belongs to the strongly connected component of $\cal M$ absorbing the observed trajectory $(X_t)_t$. For instance, suppose that $\cal M$ is a chain on states $\{1,2,\ldots,7\}$ whose transition matrix is the random walk matrix on a graph that is the disjoint union of a square on nodes $\{1,\ldots,4\}$ and a triangle on nodes $\{5,6,7\}$, while $\cal M'$'s transition matrix is the random walk matrix on a graph that is the disjoint union of a clique on nodes $\{1,\ldots,4\}$ and a triangle on nodes $\{5,6,7\}$. If our observed trajectory of $\cal M$ lies in the strong connected component defined by states $\{1,\ldots,4\}$, we will easily identify its difference to $\cal M'$. On the other hand, if our observed trajectory of $\cal M$ lies on the strong component defined by states $\{5,6,7\}$, we will not be able to identify that we are not observing a trajectory of $\cal M'$, no matter how long the trajectory is.


%Start axiomatically by saying that the behavior of the two chains is captured by tv of words, then seay that it is not scale invariant and then give the spectral.


For some notion of difference, $\dist{\cal M}{\cal M'}$, between Markov chains, we would like to quantify {\em how long} a trajectory $X_0,\ldots,X_{\ell}$ from an {\em unknown} chain, $\cal M$, we need to observe to be able to distinguish, with probability at least $1-\delta$:
\begin{align}
{\cal M}={\cal M}'~~\text{versus}~~\dist{\cal M}{\cal M'}>\epsilon, \label{eq:gof MC testing}
\end{align}
for some given parameters $\delta \in (0,1)$ and $\epsilon>0$. Let us call this problem {\em single-sample goodness-of-fit (or identity) testing for Markov chains}. We will study it taking $\delta=1/3$, with the understanding that this probability can be boosted to any small constant at the cost of a $O(\log (1/\delta))$-multiplicative factor in the length $\ell$ of the observed trajectory.

What notion of difference between Markov chains is the right one to use to study the afore-described goodness-of-fit testing problem is not clear. One of our contributions is to identify a meaningful measure of difference in Section~\ref{sec:prelim}. What are the desiderata for such a measure? Let us discuss this:
\begin{enumerate}
\item First, as our simple example above illustrates, under a worst-case starting state $X_0$, we may not be able to identify that ${\cal M} \neq {\cal M}'$ from a single trajectory. So, we would like to identify a notion of difference that takes a value $\dist{\cal M}{\cal M'}= 0$, whenever chains $\cal M$ and $\cal M'$ are indistinguishable from a single trajectory. \label{distance property 1}

\item Whenever $\cal M$ and $\cal M'$ {\em are} distinguishable from a single trajectory, whose starting state we do not get to control, i.e. from any starting state, we would like that our difference measure quantifies {\em how different} the chains are. 
%and that it can be used to quantify the number of steps that we need to observe from ${\cal M}$'s trajectory, under a worst-case starting state $X_0$, to tell that ${\cal M} \neq {\cal M}'$. 
Clearly, our notion of difference could not just be a combinatorial property of the connectivity of the state space of $\cal M$ and $\cal M'$, since the combinatorial structure won't reflect the magnitude of the differences in the chains. 
%transitions that may be hard to identify. Rather it should be a probabilistic or spectral property of the transition matrices that can be related to our observations. 
\label{distance property 2}
\end{enumerate}


A natural notion of difference between two chains $\cal M$ and $\cal M'$ is the total variation distance %, $\dtv{\word{\cal M}{\ell}}{\word{\cal M'}{\ell}}$,
 between the trajectories (a.k.a.~{\em words})  $\word{\cal M}{t} \eqdef X_0 X_1 \cdots X_t$ and $\word{\cal M'}{t} \eqdef Y_0 Y_1 \cdots Y_t$ sampled from the two chains in some $t$ steps and starting at some state $X_0=s_0=Y_0$. Indeed, this distance captures how different our $t$-step observations from the two chains are. As the starting state $s_0$ is out of our control, we should rather use the 
\begin{align}
\min_{s_0} \dtv{\word{\cal M}{t}}{\word{\cal M'}{t}~|~X_0=Y_0=s_0}. \label{eq:worst word tv}
\end{align}
In particular, taking the min makes sure that Property~\ref{distance property 1} above is satisfied.

While there is sometimes a natural $t$ to use in~\eqref{eq:worst word tv} as we will see in Section~\ref{sec:shuffle}, where we analyze card shuffles, it is mostly unclear how to set $t$. Setting $t$ to infinity will make the above quantity take $0/1$ values, which is un-informative about {\em how different} the two chains are. Setting $t$ too small would only capture differences in the proximity of the starting state $s_0$. Hence, setting~$t$ to some reasonably large but finite value makes more sense, but how to choose it?

To avoid the conundrum, we propose a notion of difference between Markov chains $\cal M$ and $\cal M'$, which captures the {\em scaling behavior}, as $t \rightarrow \infty$, of~\eqref{eq:worst word tv}. Interestingly, we argue in Section~\ref{sec:prelim} that this scaling behavior is tightly captured by spectral properties of the following matrix:
$$\srprod{P}{Q}\eqdef\left[\sqrt{P_{ij}\cdot Q_{ij}}~ \right]_{ij\in[n\times n]},$$
where $P$ and $Q$ are the transition matrices of the two chains, i.e. $P_{ij}$ and $Q_{ij}$ denote the probabilities of transitioning from state $i$ to state $j$ in the two chains. In Eq.~\eqref{eq:hellinger_square_algebraic}, we show a recursive decomposition that allows us to exactly express the square Hellinger similarity, $1-\hellingersq{\word{\cal M}{t}}{\word{\cal M'}{t}}$ of $\ell$-length words sampled from the two chains in terms of the $\ell$-th power of the above matrix, and the distribution of the starting states $X_0$ and $Y_0$ in the two words. Given the relationship between Hellinger and total variation distance (see Eq.~\eqref{eq:tv hellinger relation}), the $\ell$-the power of $\srprod{P}{Q}$ also captures the total variation distance between words sampled from the two chains. 

To identify a word-length independent measure of difference between the two chains, we argue that the scaling behavior of the Hellinger distance/total variation distance is captured by the largest eigenvalue $\lambda_1=\rho(\srprod{P}{Q})$ of matrix $\srprod{P}{Q}$. We show that always $\lambda_1 \le 1$ (Claim~\ref{cl:eigval_less_than_one}), and that $\lambda_1=1$ if and only if the two chains have an identical connected component (Claim~\ref{cl:eigval_less_than_one}), hence we would be unable to identify the difference between the two chains from a single trajectory and a worst-case starting state, as per our discussion above. Furthermore, the slowest (with respect to the choice of the starting state) that the square Hellinger similarity of the two chains can drop as a function of the length $\ell$ is $\lambda_1^\ell$, up to factors that do not depend on $\ell$; this follows from~\eqref{eq:hellinger_square_algebraic} and~\eqref{eq:largest_eigenvalue}. That is, the slowest that the square Hellinger distance of the two chains can increase is $1-O(\lambda_1^\ell)$.
%\footnote{\costis{I believe these claims to be true. Are they? They are also consistent with what happens when $\lambda_1=1$. Speaking of this, I don't understand why example 1c is not contradicting Claim~\ref{cl:dist_zero}.}} 
Given these, and the intimate relationship between Hellinger and total variation distance (Eq.~\eqref{eq:tv hellinger relation}), we propose the use of 
 %is tightly related to total variation distance, and total variation distance is tightly related to the number of samples needed to distinguish a trajectory sampled from the two chains, we thus propose the use of 
$\dist{\cal M}{\cal M'} = 1-\rho(\srprod{P}{Q})$ as a scale-free and meaningful  measure of difference between Markov chains. As per our discussion, this notion of distance satisfies Desiderata~\ref{distance property 1} and~\ref{distance property 2} outlined above. For symmetric Markov chains, our notion of difference is even more tightly related to the scaling behavior of trajectories sampled from the two chains even for a starting state sampled from the stationary distribution, as per Claim~\ref{cl:symm_spectrum}. Figure~\ref{fig:examples} illustrates how $\dist{\cal M}{\cal M'}$ behaves for different pairs of Markov chains $\cal M$ and $\cal M'$.

\paragraph{Our Results.} Using our proposed measure of difference between Markov chains we provide algorithms for  goodness-of-fit testing of Markov chains, namely Problem~\eqref{eq:gof MC testing}, targeting two interesting regimes. The first targets applications where the state space is polynomial in the representation of the target Markov chain $\cal M'$. The second targets settings where the state space is exponential in the representation of the target chain, but the chain has sparsity and structure. Importantly, this is applicable to testing card shuffles. Our results in the two settings are the following. 

In Section~\ref{sec:symmetric}, we study Problem~\eqref{eq:gof MC testing} under $\dist{\cal M}{\cal M'}=1-\rho(\srprod{P}{Q})$, where $P$ and $Q$ are the transition matrices of  chains $\cal M$ and $\cal M'$. We study this problem when $\cal M$ and $\cal M'$ are both {\em symmetric}, and provide near-optimal upper and lower bounds for the minimum length $\ell$ of a trajectory from the unknown chain $\cal M$ that is needed to determine the correct answer with probability at least $2/3$. In particular, Theorems~\ref{th:symmetric_ub} and~\ref{thm:symm-lower-bound} combined show that the length of the required trajectory from $\cal M$ to answer Problem~\eqref{eq:gof MC testing} is $n/\epsilon$, where $n$ is the size of the state space, up to logarithmic factors and an additive term that does not depend on $\epsilon$ or $\cal M$. Our upper bound is established via an information-efficient reduction from single-sample identity testing for Markov chains with $n$ states to the classical problem of identity testing of distributions over $O(n^2)$ elements, from i.i.d.~samples. The naive way to obtain such a reduction is to look at every $\mixt{\cal M'}$-th step of the trajectory of $\cal M$, where $\mixt{\cal M'}$ is the mixing time of chain $\cal M'$, pretending that these transitions are i.i.d.~samples from the distribution $\{\frac{1}{n} P_{ij}\}_{ij \in [n^2]}$. This incurs an unnecessary blow-up of a factor of $\mixt{\cal M'}$ in the required length of the observed trajectory, which we show how to avoid, exchanging it with an additive term that is quasi-linear in the hitting time.

In Section~\ref{sec:shuffle}, we take on the challenge of testing Markov chains whose nominal state-space is exponentially large in their representation, such as shuffles. Often, shuffles have symmetries that allow studying their transitions in a state space of manageable size. For example, the random choices that the riffle shuffle makes in the course of one step do not depend on the permutation of the cards at the beginning of the step, and can be described succinctly.
 %if $o_t$ and $o_{t+1}$ are two consecutive orderings of the deck after one riffle shuffle, then composing $o_t \circ \pi$ and $o_{t+1} \circ \pi$ with any permutation $\pi$ preserves the information about
Moreover, viewed appropriately the transitions out of any state are typically sparse. In the riffle shuffle, starting from any permutation there are $n+1$ places to cut the deck. And, starting from a cut, every little step of the riffle has two options (whether to drop a card from the left or the right stack). So breaking down one step of the riffle shuffle into a sequence of simple steps makes the transitions very sparse. 

In Definition~\ref{def:sparse} we provide a model of {\em sparse} Markov chains, capturing succinct representations of Markov chains resulting from ``breaking up into trivial steps and projecting into a smaller state space'' of Markov chains with exponentially large state-spaces such as different variants of the riffle shuffle and other shuffles~\cite{BayerDiaconis}. Roughly speaking a sparse Markov chain in our model performs transitions according to a sequence of transition matrices $P_1,\ldots,P_n$, over and over again, ad infinitum. We discuss how this model captures the essential mechanics of the riffle shuffle after Definition~\ref{def:sparse}.

Keeping the riffle shuffle as our running application, we develop tools that allow us to perform goodness-of-fit testing of sparse Markov chains according to our model. What difference measure between chains should we use? Given two sparse chains $P=(P_i)_{i \in [n]}$ and $Q=(Q_i)_{i \in [n]}$, conforming to our model, we could still define our difference measure between them using spectral properties of matrix $\srprod{P_1}{Q_1} \cdots \srprod{P_t}{Q_t}\cdots\srprod{P_n}{Q_n}$. However, we find it more natural in this case to use as difference measure the total variation distance between words sampled in one round of sampling transitions from the sequence of matrices $P_1,\ldots, P_n$ and $Q_1, \ldots, Q_n$.\footnote{We argue, in Section~\ref{sec:shuffle}, that the spectral and total variation distance approaches to define difference in this model are tightly related, as they are in the symmetric case.} This total variation distance captures the divergence of the two chains in one iteration through their transitions matrices; in our running application to riffle shuffle, they correspond to the divergence of two riffle shuffles of different parameters in one iteration of the shuffle. With this notion of difference we provide efficient testers, and sample complexity lower bounds; see Theorems~\ref{th:main_shuffling} and~\ref{thm:sparse-lower-bound}. Our upper bounds imply, in particular, that we can test goodness-of-fit of a given riffle shuffle model, such as the Gilbert-Shannon-Reeds model, against all competing riffle shuffle models at distance $\ge \epsilon$, from $O(n^{3/2}/\epsilon^2)$ shuffles. Our tester, applying to testing any sparse Markov chain model, is based on a modified and pruned $\chi^2$-style statistic, inspired by~\cite{AcharyaDK15}, which tracks the number of times a particular transition between two states occured in the observed trajectory of the Markov chain.




\paragraph{Related Work.}
\input{related}

\paragraph{Organization}
We start with a description of the notational conventions we use and a formal definition of our distance notion between Markov chains in Section \ref{sec:prelim}. In Section~\ref{sec:symmetric}, we study the problem of testing identity of symmetric Markov chains. We present our tester along with a sample complexity lower bound for this problem in this Section. In Section~\ref{sec:shuffle}, we study the identity testing question on riffle shuffles. We present our formulation of this question as a problem of testing identity for sparse Markov chains and present upper and lower bounds for this problem. Finally, in Section~\ref{sec:open}, we conclude with some open questions from the framework introduced in this paper. 

%we do not get to control the starting state of the observed trajectory of the unknown chain, ${\cal M}$, we can only hope to identify that it is different to ${\cal M}'$ if its observed trajectory will

%What we want to quantify is the {\em number of observations} that are needed to distinguish between ${\cal M} = {\cal M'}$ or not, and by ``number of observations'' we mean the {\em length} of the observed trajectory that is required to tell between these two cases. We would like to quantify the required length in terms of some notion of difference, $\dist{\cal M}{\cal M'}$, between Markov chains. Based on our discussion so far, our notion of difference should satisfy the following properties:
%\begin{enumerate}
%\item If ${\cal M}$ and ${\cal M}'$ have identical transitions in some connected component of their state-space, then we should take $\dist{\cal M}{\cal M'}=0$, even if ${\cal M}$ and ${\cal M}'$ are different outside of this connected component. The reason is that, if the observed trajectory of ${\cal M}$ lies in this connected component, then we cannot possibly identify that the chains are not identical, no matter how long a trajectory we observe. Hence, our distance notion should express that ${\cal M}$ and ${\cal M}'$ cannot be distinguished for a worst-case starting state. \label{def of dist: property 1}

%\item If the distribution of words produced starting from state $X_0$ under ${\cal M}$ and ${\cal M}'$ are different, 
%
%, starting at any state, ${\cal M}$ and ${\cal M}'$ produce sequences that are guaranteed to be infinitely often different.
%
%have identical transitions in some connected component of their state-space, then we should take $\dist{\cal M}{\cal M'}=0$, even if ${\cal M}$ and ${\cal M}'$ are different outside of this connected component. The reason is that, if the observed trajectory of ${\cal M}$ lies in this connected component, then we cannot identify that the chains are not identical.
 %
%\end{enumerate}



%We would like to propose a meaningful measure of difference, $\dist{\cal M}{\cal M'}$, between two Markov chains $\cal M$ and $\cal M'$ that both captures {\em how different} the Markov chains are, and can be used to quantify the number of observations that are needed to test whether an observed trajectory comes from a target Markov chain ${\cal M}'$ or some chain ${\cal M}$ that satisfies $\dist{\cal M}{\cal M'}>\epsilon$, for some parameter $\epsilon>0$. 
%
 %In terms of this measure, we quantify the number of observations required to distinguish between:
%$${\cal M}={\cal M'}~~\text{vs}~~\dist{\cal M}{\cal M'}>\epsilon,$$
%from a given Markov chain ${\cal M}'$ and a single trajectory from an unknown Markov chain ${\cal M}$. By ``number of observations'' we mean the {\em length} of the observed trajectory.

%We develop our notion of distance, $\dist{\cal M}{\cal M'}$, between Markov chains in Section~\ref{}. Motivated by the above discussion, our distance satisfies the following properties:
%\begin{enumerate}
%\item 
%\end{enumerate}

==> pre-stoc18-version/intro_old.tex <==
We formulate theories about the laws that govern physical phenomena by making observations and testing them against our hypotheses. A common scenario is when our observations can be reasonably modeled as i.i.d. samples from a distribution that we are trying to understand. This is the setting tackled by most classical work in Statistics. Of course, having access to i.i.d. samples from a distribution is rare and quite commonly a mere approximation of reality. We typically only have access to approximate samples from a stationary distribution, sampled by a Markov chain whose transition matrix/kernel is unknown to us and which can only be observed for some finite time horizon. In fact, to the best of our knowledge, the underlying Markov chain may not even be rapidly mixing, so there is no guarantee that we will ever see samples that are approximately distributed according to the stationary distribution.

These issues are exacerbated in high-dimensional settings, e.g., when observing the configurations of a deck of cards or a weather system, where it may also be completely impractical to work with the high-dimensional stationary distribution itself. Moreover, there are several ways to sample a stationary distribution, so it may be more important to know how it comes to be sampled. For all  these considerations, it may be both more interesting and more practical to understand the ``mechanics'' of the process that generates our observations, namely the transition matrix/kernel of the Markov chain whose evolution we get to observe.

Motivated by these considerations, in this paper we study the problem of testing the identity of Markov chains. We are given access to a {\em single} trajectory $X_0, X_1,\ldots,X_t,\ldots$ of some {\em unknown} Markov chain ${\cal M}$ over some state space $[n]$, and we want to test the identity of ${\cal M}$ to some {\em given} Markov chain ${\cal M}'$. Importantly, we do not get to control the distribution of the starting state $X_0$, and we can only observe a single trajectory of ${\cal M}$, i.e. we cannot restart the Markov chain. What could we hope to achieve?

Of course, if there is any difference in the transition matrices of $\cal M$ and $\cal M'$, one would think that we would {\em ultimately} be able to identify it by observing a sufficiently long trajectory. This is certainly true if the transition matrices of the two chains differ at a state that belongs to the strongly connected component of $\cal M$ absorbing the observed trajectory $(X_t)_t$. For instance, suppose that $\cal M$ is a chain on states $\{1,2,\ldots,7\}$ whose transition matrix is the random walk matrix on a graph that is the disjoint union of a square on nodes $\{1,\ldots,4\}$ and a triangle on nodes $\{5,6,7\}$, while $\cal M'$'s transition matrix is the random walk matrix on a graph that is the disjoint union of a clique on nodes $\{1,\ldots,4\}$ and a triangle on nodes $\{5,6,7\}$. If our observed trajectory of $\cal M$ lies in the strong connected component defined by states $\{1,\ldots,4\}$, we will easily identify its difference to $\cal M'$. On the other hand, if our observed trajectory of $\cal M$ lies on the strong component defined by states $\{5,6,7\}$, we will not be able to identify that we are not observing a trajectory of $\cal M'$, no matter how long the trajectory is.


Start axiomatically by saying that the behavior of the two chains is captured by tv of words, then seay that it is not scale invariant and then give the spectral.


For some notion of difference, $\dist{\cal M}{\cal M'}$, between Markov chains, we would like to quantify {\em how long} a trajectory $X_0,\ldots,X_{\ell}$ from an unknown chain, $\cal M$, we need to observe to be able to distinguish, with probability at least $1-\delta$:
$${\cal M}={\cal M}'~~\text{versus}~~\dist{\cal M}{\cal M'}>\epsilon,$$
for some given parameters $\delta \in (0,1)$ and $\epsilon>0$. Let us call this problem {\em single-sample goodness-of-fit testing for Markov chains}.

What notion of difference between Markov chains is the right one to use to study the afore-described goodness-of-fit testing problem is not clear. One of our contributions is to identify a meaningful measure of difference in Section~\ref{sec:prelim}. What are the desiderata for such a measure? Let us discuss this:
\begin{enumerate}
\item First, as our simple example above illustrates, under a worst-case starting state $X_0$, we may not be able to identify that ${\cal M} \neq {\cal M}'$ from a single trajectory. So, we would like to identify a notion of difference that takes a value $\dist{\cal M}{\cal M'}= 0$, whenever chains $\cal M$ and $\cal M'$ are indistinguishable from a single trajectory. \label{distance property 1}
\item Whenever $\cal M$ and $\cal M'$ {\em are} distinguishable from a single trajectory, we would like that our difference measure quantifies {\em how different} the chains are, and that it can be used to quantify the number of steps that we need to observe from ${\cal M}$'s trajectory, under a worst-case starting state $X_0$, to tell that ${\cal M} \neq {\cal M}'$. Clearly, then, our notion of difference should not just be a combinatorial property of the connectivity of the state space of $\cal M$ and $\cal M'$, since the combinatorial structure won't reflect the magnitude of tiny differences in transitions that may be hard to identify. Rather it should be a probabilistic or spectral property of the transition matrices that can be related to our observations. \label{distance property 2}
\end{enumerate}

We propose a notion of difference between Markov chains $\cal M$ and $\cal M'$, which captures the scaling behavior, as $t \rightarrow \infty$, of the total variation distance between trajectories (a.k.a. {\em words}) $X_0 X_1 \cdots X_t$ and $Y_0 Y_1 \cdots Y_t$ sampled from the two chains from a worst-case starting state $X_0=Y_0=\sigma_0$. In Section~\ref{sec:prelim} we argue that this scaling behavior is tightly captured by spectral properties of the matrix:
$$\srprod{P}{Q}\eqdef\left[\sqrt{P_{ij}\cdot Q_{ij}}~ \right]_{i,j\in[n\times n]},$$
where $P$ and $Q$ are the transition matrices of the two chains, i.e. $P_{ij}$ and $Q_{ij}$ denote the probabilities of transitioning from state $i$ to state $j$ in the two chains. In Eq.~\eqref{eq:hellinger_square_algebraic}, we show a recursive decomposition that allows us to exactly express the square Hellinger similarity of $\ell$-length words sampled from the two chains in terms of the $\ell$-th power of matrix $\srprod{P}{Q}$. Given the relationship between Hellinger and total variation distances (see Eq.~\eqref{eq:tv hellinger relation}), this matrix power also captures the total variation distance between words sampled from the two chains. 

To identify a word-length independent measure of difference between the two chains, we argue that the scaling behavior of the Hellinger distance/total variation distance is captured by the largest eigenvalue $\lambda_1=\rho(\srprod{P}{Q})$ of matrix $\srprod{P}{Q}$. We show that always $\lambda_1 \le 1$ (Claim~\ref{cl:eigval_less_than_one}), and that $\lambda_1=1$ if and only if the two chains have an identical connected component (Claim~\ref{cl:eigval_less_than_one}), hence we would be unable to identify the difference between the two chains from a single trajectory and a worst-case starting state, as per our discussion above. Furthermore, the slowest (with respect to the choice of the starting state) that the square Hellinger similarity of the two chains can drop as a function of the length $\ell$ is $\lambda_1^\ell$ (see~\eqref{eq:largest_eigenvalue}), i.e. the slowest that the square Hellinger distance of the two chains can increase is $1-\lambda_1^\ell$.\footnote{\costis{I believe these claims to be true. Are they? They are also consistent with what happens when $\lambda_1=1$.}} As Hellinger distance is tightly related to total variation distance, and total variation distance is tightly related to the number of samples needed to distinguish a trajectory sampled from the two chains, we thus propose the use of $\dist{\cal M}{\cal M'} = 1-\rho(\srprod{P}{Q})$ as a scale-free and meaningful difference measure between Markov chains. As per our discussion, this notion of distance satisfies Desiderata~\ref{distance property 1} and~\ref{distance property 2} outlined above. For symmetric Markov chains, our notion of difference is even more tightly related to the scaling behavior of trajectories sampled from the two chains even for a starting state sampled from the stationary distribution, as per Claim~\ref{cl:symm_spectrum}. Figure~\ref{fig:examples} illustrates how $\dist{\cal M}{\cal M'}$ behaves for different pairs of Markov chains $\cal M$ and $\cal M'$.

\paragraph{Our Results.}

\paragraph{Related Work.}
%we do not get to control the starting state of the observed trajectory of the unknown chain, ${\cal M}$, we can only hope to identify that it is different to ${\cal M}'$ if its observed trajectory will

%What we want to quantify is the {\em number of observations} that are needed to distinguish between ${\cal M} = {\cal M'}$ or not, and by ``number of observations'' we mean the {\em length} of the observed trajectory that is required to tell between these two cases. We would like to quantify the required length in terms of some notion of difference, $\dist{\cal M}{\cal M'}$, between Markov chains. Based on our discussion so far, our notion of difference should satisfy the following properties:
%\begin{enumerate}
%\item If ${\cal M}$ and ${\cal M}'$ have identical transitions in some connected component of their state-space, then we should take $\dist{\cal M}{\cal M'}=0$, even if ${\cal M}$ and ${\cal M}'$ are different outside of this connected component. The reason is that, if the observed trajectory of ${\cal M}$ lies in this connected component, then we cannot possibly identify that the chains are not identical, no matter how long a trajectory we observe. Hence, our distance notion should express that ${\cal M}$ and ${\cal M}'$ cannot be distinguished for a worst-case starting state. \label{def of dist: property 1}

%\item If the distribution of words produced starting from state $X_0$ under ${\cal M}$ and ${\cal M}'$ are different, 
%
%, starting at any state, ${\cal M}$ and ${\cal M}'$ produce sequences that are guaranteed to be infinitely often different.
%
%have identical transitions in some connected component of their state-space, then we should take $\dist{\cal M}{\cal M'}=0$, even if ${\cal M}$ and ${\cal M}'$ are different outside of this connected component. The reason is that, if the observed trajectory of ${\cal M}$ lies in this connected component, then we cannot identify that the chains are not identical.
 %
%\end{enumerate}



%We would like to propose a meaningful measure of difference, $\dist{\cal M}{\cal M'}$, between two Markov chains $\cal M$ and $\cal M'$ that both captures {\em how different} the Markov chains are, and can be used to quantify the number of observations that are needed to test whether an observed trajectory comes from a target Markov chain ${\cal M}'$ or some chain ${\cal M}$ that satisfies $\dist{\cal M}{\cal M'}>\epsilon$, for some parameter $\epsilon>0$. 
%
 %In terms of this measure, we quantify the number of observations required to distinguish between:
%$${\cal M}={\cal M'}~~\text{vs}~~\dist{\cal M}{\cal M'}>\epsilon,$$
%from a given Markov chain ${\cal M}'$ and a single trajectory from an unknown Markov chain ${\cal M}$. By ``number of observations'' we mean the {\em length} of the observed trajectory.

%We develop our notion of distance, $\dist{\cal M}{\cal M'}$, between Markov chains in Section~\ref{}. Motivated by the above discussion, our distance satisfies the following properties:
%\begin{enumerate}
%\item 
%\end{enumerate}

==> pre-stoc18-version/nota.tex <==
We list the general notational conventions used in this paper. We denote vectors by small letters 
such as $\vect{v}$ and matrices by capital letters such as $A$,$B$,$P$,$Q$. The $i^{th}$ entry 
of vector $\vect{v}$ is denoted by $v_i$ or $v[i]$ and the $(ij)^{th}$ entry of matrix $A$ ($i^{th}$ row, $j^{th}$ column) is 
denoted by $A_{ij}$ or $A[ij]$; $\vect{e}_i$ denotes the standard basis vector with 
$1$ in its $i^{th}$ coordinate and $0$ elsewhere; $\onev$ denotes the vector of all ones. 
The ``entrywise'' $L_1$ and $L_2$ norms of a matrix  $A$ are respectfully denoted as $\onenorm{A}$ and $\twonorm{A}$; 
$\specr{A}$ denotes the spectral radius of matrix $A$, i.e., the maximum absolute eigenvalue of $A$. 
The eigenvalues of $A$ are denoted by $\eigi[1], \dots, \eigi, \dots, \eigi[n]$ and 
the respective right eigenvectors by $\eigvi[1],\dots,\eigvi,\dots,\eigvi[n]$ (left 
eigenvectors by $\eigvli[1],\dots,\eigvli[n])$; for symmetric matrix $A$ we assume that 
$\eigi[1]\ge \dots \ge \eigi \ge \dots \ge \eigi[n]$. 
%Let $P$, $Q$ be $n \times n$ matrices. A quantity 
%which is central to this paper and is used extensively is $\srprod{P}{Q}$, which we call as the 
%square root product of $P$ and $Q$. It is $n \times n$ matrix such that ${\srprod{P}{Q}}_{ij} = 
%\sqrt{P[ij]Q[ij]}$. We also define the square root product of vectors $\vect{p}$ and $\vect{q}$ 
%as $\srprod{\vect{p}}{\vect{q}}[i] = \sqrt{p[i] q[i]}$.\\

%\nishanth{Add description about Poisson Sampling}

%\noindent As already stated, we will use capital letters $P$, $Q$ to denote Markov chains. We will also use $P$,$Q$ to denote their respective transition matrices. \nishanth{TBF}

Before formulating the precise question we study, we need a notion of distance between Markov chains to work with.

==> pre-stoc18-version/notations.tex <==
%% General machinery
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation*}}
\newcommand{\eeq}{\end{equation*}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
%\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{_{#1}}\InBrackets{#2}}
\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{#1}\InBrackets{#2}}
\newcommand{\Exlong}[2][]{\operatornamewithlimits{\mathbf E}\limits_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\newcommand{\Prlong}[2][]{\operatornamewithlimits{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\newcommand{\Var}[2][]{\operatorname{\mathbf{Var}}_{#1}\InBrackets{#2}}
\newcommand{\Varlong}[2][]{\operatornamewithlimits{\mathbf{Var}}\limits_{#1}\InBrackets{#2}}
\def\prob{\Prx}
\def\Prl{\Prlong}
\def\expect{\Ex}
\newcommand{\super}[1]{^{(#1)}}
\newcommand{\dd}{\mathrm{d}}
%\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\vect}[1]{\ensuremath{\overrightarrow{#1}}}
\newcommand{\vect}[1]{\ensuremath{\vec{#1}}}
%%%%%%%%%%%%% New macros %%%%%%%%%%%%%%%%%%
\newcommand{\expec}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\expectation}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\frob}[1]{\left\|#1\right\|_F}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\left(#1\right)}}
\newcommand{\otilde}[1]{\ensuremath{\widetilde{\mathcal{O}}\left(#1\right)}}
\newcommand{\distop}[2]{\ensuremath{dist\left(#1,#2\right)}}
\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\abshigh}[1]{\left|\vphantom{\sum}#1\right|}
\newcommand{\vol}[1]{\textrm{Vol}\left(#1\right)}
\newcommand{\inv}[1]{{#1}^{-1}}

% Linear Algebra
%\newcommand{\srprod}[2]{\left[#1,#2\right]_{_\surd}}
\newcommand{\norm}[1]{\left\| {#1} \right\|}
\newcommand{\onenorm}[1]{\left\| {#1} \right\|_1}
\newcommand{\onenormint}[2]{\left\| {#1} \right\|_{L_1#2}}
\newcommand{\twonorm}[1]{\left\| {#1} \right\|_2}
\newcommand{\infnorm}[1]{\left\| {#1} \right\|_{\infty}}
\newcommand{\iprod}[2]{\langle #1, #2 \rangle}
\newcommand{\scalprod}[2]{\langle #1, #2 \rangle}
\newcommand{\trans}[1]{{#1}^{\top}}
\newcommand{\trace}[1]{\text{Tr}\left(#1\right)}
\renewcommand{\det}[1]{{\rm det}\left(#1\right)}
\newcommand{\srprod}[2]{\left[#1,#2\right]_{\text{\textsurd}}}
\newcommand{\srprodt}[2]{\left[#1,#2\right]_{\text{\textsurd}}^{\top}}
\newcommand{\sqsrprod}[2]{\left[#1,#2\right]_{\text{(\textsurd-\textsurd)}^2}}
\newcommand{\onee}{\vect{e}_1}
\newcommand{\oneet}{\vect{e}_1^{\top}}
\newcommand{\onev}{\vect{\mathds{1}}}
\newcommand{\onevt}{{\trans{\onev}}}
\newcommand{\onevi}[1][i]{\vect{e}_{#1}}
\newcommand{\onevti}[1][i]{{\trans{\onevi[#1]}}}
%\newcommand{\ind}[1]{\mathds{1}\left[\vphantom{\sum}#1\right]}
\newcommand{\specr}[1]{\rho\left(#1\right)}
\newcommand{\eigi}[1][i]{\lambda_{#1}}
\newcommand{\eigvi}[1][i]{\vect{v}_{#1}}
\newcommand{\eigvit}[1][i]{\vect{v}_{#1}^{\top}}
\newcommand{\eigvli}[1][i]{\vect{u}_{#1}}
\newcommand{\eigvlit}[1][i]{\vect{u}_{#1}^{\top}}
\newcommand{\vev}{{\vect{v}}}
\newcommand{\vevt}{{\trans{\vect{v}}}}
\newcommand{\veut}{{\trans{\vect{u}}}}





%Probability & Marcov Chains 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Poisson}[1]{\ensuremath{\mathrm{Poisson}\left(#1\right)}}
\newcommand{\Uniform}[1]{\ensuremath{\mathrm{Unif}\left(#1\right)}}
\newcommand{\covert}[1]{\mathrm{CovT}\left(#1\right)}
\newcommand{\hitt}[1]{\mathrm{HitT}_{#1}}
\newcommand{\mixt}[1]{\mathrm{MixT}_{#1}}
\newcommand{\returnt}[1][i]{\mathrm{Return}_{#1}}
\newcommand{\word}[2]{\mathcal{W}_{_{#1}}^{#2}}
\newcommand{\MCfamily}{\mathcal{MC}}
\newcommand{\dtv}[2]{\mathrm{d}_{_\mathrm{TV}}\left(#1,#2\right)}
\newcommand{\dtvsq}[2]{\mathrm{d}_{_\mathrm{TV}}^{2}\left(#1,#2\right)}
\newcommand{\hellinger}[2]{\mathrm{d}_{_\mathrm{Hel}}\left(#1,#2\right)}
\newcommand{\hellingersq}[2]{\mathrm{d}_{_\mathrm{Hel}}^{2}\left(#1,#2\right)}
\newcommand{\distr}[1][D]{\mathrm{#1}}
\newcommand{\stationp}{\vect{p}}
\newcommand{\stationq}{\vect{q}}
\newcommand{\infmap}[1]{\mathcal{K}_{#1}}
\newcommand{\dist}[2]{\mathrm{Dist}\left(#1,#2\right)}
\newcommand{\distsq}[2]{\mathrm{Dist}^2\left(#1,#2\right)}


%Shuffling Marcov Chains
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\MCseqP}{\left(p_0,\{P_t\}_{t=1}^{n}\right)}
%\newcommand{\MCseqPS}{\left(p_0^*,\{P_t^*\}_{t=1}^{n}\right)}
%\newcommand{\MCseqQ}{\left(q_0,\{Q_t\}_{t=1}^{n}\right)}
%\newcommand{\MCseqQS}{\left(q_0^*,\{Q_t^*\}_{t=1}^{n}\right)}
\newcommand{\MCseqP}{\{P_t\}_{t=1}^{n}}
\newcommand{\MCseqPS}{\{P_t^*\}_{t=1}^{n}}
\newcommand{\MCseqQ}{\{Q_t\}_{t=1}^{n}}
\newcommand{\MCseqQS}{\{Q_t^*\}_{t=1}^{n}}


%%%%%%%Complexity  %%%%%%%%%
\newcommand{\Ocomplex}[1]{O\left(#1\right)}
\newcommand{\wO}[1]{\widetilde{O}\left(#1\right)}
\newcommand{\wTheta}[1]{\widetilde{\Theta}\left(#1\right)}
\newcommand{\wOm}[1]{\widetilde{\Omega}\left(#1\right)}
\newcommand{\Om}[1]{\Omega\left(#1\right)}
% \newcommand{\vdpar}{v_d^{\|}}
% \newcommand{\vdperp}{v_d^{\perp}}
% \newcommand{\wtild}{\widetilde{w}}
% \newcommand{\ft}[1]{\widehat{#1}}
% 
% \DeclareMathOperator{\dict}{dict}

\DeclareMathOperator{\corr}{corr}
\newcommand{\citep}{\cite}
\newcommand{\citet}{\cite}
\newcommand{\citealp}{\cite}
\def\nn{\nonumber}
\newcommand{\sep}{\alpha}




%%%%%from other papers
\newcommand\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\N{\mathbb{N}}
\newcommand\Z{\mathbb{Z}}
\renewcommand\S{\mathbb{S}}
\def\Pbb{\mathbb{P}}
\newcommand{\singmin}[1]{\ensuremath{\sigma_{\min}\left(#1\right)}}
\newcommand{\singmax}[1]{\ensuremath{\sigma_{\max}\left(#1\right)}}
\newcommand{\distw}[2]{\ensuremath{d_w\left(#1,#2\right)}}



\newcommand{\neighb}[1]{\mathcal{N}\left(#1\right)}
\renewcommand\t{{\scriptscriptstyle\top}}
\DeclareMathOperator{\uniqint}{Uniq-intersect}
\DeclareMathOperator{\coeff}{coeff}
%\DeclareMathOperator{\dict}{dict}
\newcommand\wh{\widehat}
\newcommand\wt{\widetilde}
\newcommand{\wn}{\widetilde{\vect{w}}}
\newcommand\eps{\varepsilon}
%\newcommand\veps{\varepsilon}
\newcommand\h{\hat}

\newcommand\tl{\tilde}
\newcommand\sign{\operatorname{sign}}
\newcommand{\tzero}{t_0}


% \newcommand{\indic}[1]{\mathds{1}_{\left\{ #1 \right\}}}
% \newcommand{\poly}[1]{\textrm{poly}\left(#1\right)}
% \newcommand{\projon}[2][]{#2_{#1^\perp}}

% Additions by Nishanth -------------------------------------------------------------
\newenvironment{prevproof}[2]{\noindent {\em {Proof of {#1}~\ref{#2}:}}}{$\hfill\qed$\vskip \belowdisplayskip}









%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\dimen}{d}
% \newcommand{\nv}{n}
% \newcommand{\ver}{\vect{v}}
% \newcommand{\vi}[1][i]{\ver_{#1}}
% \newcommand{\wi}[1][i]{\vect{w}_{#1}}
% \newcommand{\ui}[1][i]{\bu_{#1}}
% \newcommand{\z}{\vect{z}}
% \newcommand{\bv}{\vect{v}}
% \newcommand{\etab}{\vect{\eta}}
% \newcommand{\bu}{\vect{u}}
% \newcommand{\bh}{\vect{h}}
% \newcommand{\V}{{\rm Vert}}
% \newcommand{\x}{\vect{x}}
% \renewcommand{\xi}[1][i]{\x_{#1}}
% \newcommand{\w}{\vect{w}}
% \newcommand{\amin}{a_{\textrm{min}}}
% \newcommand{\amax}{a_{\textrm{max}}}
% 
% \newcommand{\uperp}{\vect{u}_{\perp}}
% \newcommand{\upar}{\vect{u}_{\circ}}
% \newcommand{\zpr}{\boldsymbol{\omega}_{\circ}}
% \newcommand{\zperp}{\vect{z}_{\perp}}
% \newcommand{\zpar}{\vect{z}_{\circ}}
% \newcommand{\fhat}{\widehat{f}}
% \newcommand{\err}{\mathrm{err}}
% 
% \newcommand{\coef}{15^{d-1}\cdot\vol{\S^{d-1}}^{-1}}
% \newcommand{\coeffrac}{\frac{15^{d-1}}{\vol{\S^{d-1}}}}
% \newcommand{\coefm}{15^{d-2}\cdot\vol{\S^{d-2}}^{-1}}
% \newcommand{\imag}{\mathrm{i}}
% \newcommand{\prolate}{\varphi}
% \newcommand{\prolateh}{\widehat{\varphi}}
% \newcommand{\prolateG}{\varphi_{\gamma}}
% \newcommand{\prolatehG}{\widehat{\varphi}_{\gamma}}
% \newcommand{\polylog}{\operatorname{polylog}}
% \newcommand{\Ltwo}{\mathbb{L}^2}
% \newcommand{\gh}{\widehat{g}}
% \newcommand{\conv}{\ast}
% \newcommand{\shift}{{\omega_s}}
% \newcommand{\delshift}{\delta_{\shift}}
% \newcommand{\cprol}{c_{\textrm{prol}}}
% 
% \newcommand{\ratsep}{k}
% \newcommand{\xmax}{x_{\textrm{max}}}


==> pre-stoc18-version/openquestions.tex <==
In this paper, we proposed a new framework for studying property testing questions on Markov chains. 
There seem to be multiple avenues for future research and abundant number of open problems arising from this framework. 
We first list some questions which may be of interest here.
\begin{enumerate}
\item What is the optimal sample complexity for identity testing on symmetric Markov chains? In this paper, we show an upper bound of $\wO{\hitt{Q}\cdot\log\left(\hitt{Q}\right)+\frac{n}{\eps}}$ samples (Theorem \ref{th:symmetric_ub}). We conjecture that $\Theta\left( \frac{n}{\eps}\right)$ (same as our lower bound) is the right sample complexity for this problem and an explicit dependence on the hitting time of chain $Q$ may not be necessary. It is implicitly captured to an extent by the guarantee we get from the parameter $\eps$.
\item What is the optimal sample complexity for identity testing on the sparse Markov chains defined in Section~\ref{sec:shuffle}? In this paper, we show an upper bound of $\widetilde{O}\left( \frac{n^{3/2}}{\epsilon^2} \right)$ (Theorem \ref{th:sparse_ub}). We conjecture that $\Theta\left( \frac{n}{\eps^2}\right)$ (same as our lower bound) is the right sample complexity for this problem.

\item As there is a natural operation of taking a convex combination of Markov chains, it is natural to ask how our spectral definition of distance 
$1-\specr{\srprod{P}{Q}}$ between two symmetric chains changes if we substitute either $P$ or $Q$ with a convex combination of $P$ and $Q$. How does the distance now relate to the original value?
\item How is the distance $\eps=1-\specr{\srprod{P}{Q}}$ between two Markov chains $P$ and $Q$ related to the distance between Markov chains
$P^k$ and $Q^k$,i.e., states in Markov chains $P$ and $Q$ being observed only at intervals of size $k$? 
\item Given $\eps_2 \ge \eps_1$, and access to words from each of two chains, can we distinguish whether the two chains are $\le \eps_1$-close or $\ge \eps_2$-far? This problem, known as closeness testing in literature, is another interesting direction using our framework.
\end{enumerate}
%More broadly, we are interested in the following research directions
%\begin{enumerate}
%\item Testing other properties of Markov chains, e.g., testing closeness of two Markov chains.
%\item Testing Hidden Markov Models.
%\end{enumerate}


%\nishanth{
%Reminders:
%\begin{enumerate}
%\item Do we want to change the title of the paper so as to sell the framework? Although we solve testing problems only, what we have is quite general and can be applied to statistical problems other than testing as well for e.g. learning). 
%
%%\item Add remark saying that we considered other seemingly more natural and simpler distance notion and mention why they don't capture the behavior well. For example, for GSR L1 between the parameter vectors isn't a good distance notion as it gives large weight to parameters which are of little significance.
%\end{enumerate}
%}

==> pre-stoc18-version/outline.tex <==
\begin{itemize}
 \item Intro
 \item Preliminaries
 \item Distance (part of preliminaries)
 \item Symmetric MC Upper bound
 \item Symmetric MC Lower bound
 \item Card Shuffling
\end{itemize}


\nick{For Costis, regarding different dependency on $\eps$ between results for (i) symmetric and (ii) sparse (card shuffling) Markov chains.}
We have $\frac{1}{\eps}$ dependency on $\eps$ in our upper and lower bound results for symmetric Markov chains, and $\frac{1}{\eps^2}$ dependency for the
identity testing of sparse Markov chains. One may think that the cause of this is the difference between Hellinger and total variation distances, but I think 
it is not the case. In fact, in both settings we can avoid using Hellinger distance in our definition of $\eps$.
I believe that the real cause is different definitions of the parameter $\eps$ in two settings. More specifically, $\eps$ is related in different ways
to the total variation distance between word distributions in two settings. In the symmetric setting, we have both $\dtv{\word{P}{\ell}}{\word{Q}{\ell}},
\hellinger{\word{P}{\ell}}{\word{Q}{\ell}} \ge 0.1$ for $\ell=\wTheta{\frac{1}{\eps}}$; while in the second setting $\eps=\dtv{\word{P}{n}}{\word{Q}{n}}$, 
where $n>>\ell\approx\frac{1}{\eps}$ (note that there is explicit polynomial inequality relation between $\eps$ and $n$ 
in our lower bounds, see Theorems~\ref{thm:symm-lower-bound} and Theorem~\ref{thm:sparse-lower-bound}). Because of this relation between $n$ and 
$\eps$, technically speaking, one cannot fix $n$ and study asymptotic dependency on $\eps$. On the other note, the different dependency on $\eps$ might be just 
a difference between more special setting of symmetric Markov chains versus general case. Indeed, we might expect better dependency on 
$\eps$ in a more specialized setting. 

\begin{itemize}
 \item General conventions
 \begin{itemize}
  \item vectors $\vect{v}$ (macro \verb|\vect{v}|)
  \item matrices $A$,$B$,$C$,$D$,$P$,$Q$,$M$.
  \item square root product of matrices and vectors $\srprod{P_t}{Q_t}$, $\srprod{\vect{p}}{\vect{q}}$ (macro \verb|\srprod{P}{Q}|) 
  \item $\onenorm{A}$ ``entrywise'' norm ($L_1$) of a matrix $A$ (macro \verb|\onenorm{A}|) 
  \item $\twonorm{A}$ ``entrywise'' norm ($L_2$) of a matrix $A$ (macro \verb|\twonorm{A}|) 
  \item $\onev$ - vector of all ones (macro \verb|\onev|)
  \item $\srprodt{\vect{p}}{\vect{q}}$  (macro \verb|\srprodt{\vect{p}}{\vect{q}}|)
  \item $\trans{\onev}\circ\srprod{P_t}{Q_t}\circ\onev$ (macro \verb|\trans{\onev}\circ\srprod{P_t}{Q_t}\circ\onev|)
  \item spectral radius $\specr{A}$ of a matrix $A$ (macro \verb|\specr{A}|)
  \item eigenvalues: $\eigi[1]\ge\dots\ge\eigi\ge\dots\ge\eigi[n]$ (macro \verb|\eigi[1],\eigi|)
	\item eigenvectors: $\eigvi[1],\dots,\eigvi,\dots\eigvi[n]$ (macro \verb|\eigvi[1],\eigvi|)
  \item $\dtv{\distr_1}{\distr_2}$ TV distance between $\distr_1$ and $\distr_2$ (macro \verb|\dtv{\distr_1}{\distr_2}|)
  \item $\hellinger{\distr_1}{\distr_2}$ Hellinger distance between $\distr_1$ and $\distr_2$ (macro \verb|\hellinger{\distr_1}{\distr_2}|)
 \end{itemize}
 \item Markov Chain
 \begin{itemize}
 \item number of states $n$
 \item number of steps $T$
 \item transition probabilities, $n\times n$ matrix $P,Q$ or $M$
 \item stationary distributions $\stationp$ and $\stationq$ of $P$ and $Q$ (macro \verb|\stationp , \staionq|)
 \item cover time $\covert{M}$ (macro \verb|\covert{M}|)
 \item hitting time $\hitt{M}$ (macro \verb|\hitt{M}|) 
 \item indexes of states $i,j$, index of time $t$
 \item word distributions $\word{P}{T}$ of length $T$ (macro \verb|\word{P}{T}|) 
 \item word distribution $\word{P}{\infty}$
 \item family of Marcov Chains $\MCfamily$ (macro \verb|\MCfamily|)
 \end{itemize}
 \item number of samples $m$
 \item Card Shuffling
 \begin{itemize}
 \item MC $\MCseqP$, each $P_t$ is a sparse matrix, $p_0$ is initial distribution. (macro \verb|\MCseqP, \MCseqQ|)
 \item $P\eqdef\MCseqP$, $Q\eqdef\MCseqQ$
 \item distance  $\dist{P}{Q}$ between words of length $n$ in $\MCseqP$ and $\MCseqQ$ models. 
 \item generic edge $e$
 \item set of all edges $E(t)$ from states at time $t$ to states at time $t+1$.
 \end{itemize}
 
\end{itemize}


==> pre-stoc18-version/prelim.tex <==
%\noindent \nick{Basic intro and notations on Markov chains.}
A {\em discrete-time} Markov chain is a stochastic process $\{X_t\}_{t \in \{0,1,\ldots \}}$ over a state space $S$ which satisfies the Markov property: 
the probability of being in state $s$ at time $t+1$ depends only on the state at previous time $t$. In this paper, we
only consider Markov chains with a {\em finite state space} such that $|S|=n$. Such Markov chains can be completely specified 
by a $n \times n$ transition matrix (\emph{kernel}) that contains probabilities of transitioning from state $i$ to state $j$ 
in the $i^{th}$ row and $j^{th}$ column. The transition matrix has non-negative entries and is a stochastic matrix. We use capital letters $P,Q,M$ to represent Markov 
chains as well as their respective transition matrices. The stationary distribution $\pi$ of a Markov chain 
$P$ is a distribution over the state space $S$ (written as a column vector) such that it satisfies $\trans{\pi}\circ P = \trans{\pi}$. 
An important parameter in the study of Markov chains is the distribution of the starting state $s_0$ which we denote by $\vect{p}$ (for the Markov chain $P$). It may or not may not be the stationary distribution. In many cases it will be the distribution with all probability mass at a single state. Two popular notions of distance between distributions will be used heavily in this paper. We state their formal definitions below.
\begin{definition}
\label{def:stat_dist}
The {\em total variation} and {\em Hellinger} distances between distributions $p,q$ over $[k]$: 
$\dtv{p}{q}\eqdef\frac{1}{2}\sum\limits_{i\in[k]}\abs{p_i-q_i}$;\quad\quad\quad\quad 
$\hellingersq{p}{q}\eqdef\frac{1}{2}\sum\limits_{i\in[k]}\left(\sqrt{p_i}-\sqrt{q_i}\right)^2= 1-\sum\limits_{i\in[k]}\sqrt{p_i\cdot q_i}$;
\be
\label{eq:tv hellinger relation}
\sqrt{2}\cdot\hellinger{p}{q}\ge\dtv{p}{q}\ge\hellingersq{p}{q}. 
\ee
	%\begin{align}
	%\dtv{p}{q}\eqdef\sup_{A\subset[k]}|p(A)-q(A)|=\frac{1}{2}\sum_{i\in[k]}\abs{p_i-q_i} \notag\\
	%\hellingersq{p}{q}\eqdef\frac{1}{2}\sum_{i\in[k]}\left(\sqrt{p_i}-\sqrt{q_i}\right)^2= 1-\sum_{i\in[k]}\sqrt{p_i\cdot q_i} \notag\\
	%\sqrt{2}\cdot\hellinger{p}{q}\ge\dtv{p}{q}\ge\hellingersq{p}{q}. \label{eq:tv hellinger relation}
	%\end{align}
\end{definition}
%We will also consider symmetric Markov chains where the transition martices are symmetric. We state below a well-known fact about symmetric Markov chains:
%\begin{lemma}
%The uniform distribution $\frac{1}{n}\onev$ is the stationary distribution for any discrete-time, finite-state symmetric Markov chain.
%\end{lemma}
We now state without proof a well-known result which relates the total variation distance between two distributions to the best achievable distinguishability between the two. This will be useful in understanding our proposed notion of distance between two chains.
\begin{lemma}
\label{lem:tv_lemma}
Given two distributions $p,q$ and a sample $x$ drawn from either $p$ or $q$, no algorithm can distinguish whether $x$ was drawn from $p$ or $q$ with probability more than $\frac{1+\dtv{p}{q}}{2}$.
\end{lemma}

 
%We begin by stating some of the notational conventions used in this paper.
%Next, we motivate our framework by looking at a natural question: Given two Markov chains, $P$ and $Q$, how close is their behavior?


==> pre-stoc18-version/related.tex <==
Testing goodness-of-fit for distributions has a long history in Statistics; for some old and more recent references see, e.g.,~\cite{Pearson00,Fisher35,RaoS81,Agresti11}. 
In this literature the emphasis has been on the asymptotic analysis of tests, pinning down their error exponents as the number of samples tends to infinity~\cite{Agresti11,TanAW10}. In 
the last two decades or so, distribution testing has also piqued the interest of theoretical computer scientists~\cite{BatuFFKRW01,Paninski08,LeviRR13,ValiantV14,ChanDVV14, AcharyaDK15,CanonneDGR15,DiakonikolasK16,DaskalakisDSVV13,CanonneRS14}, where the emphasis, in contrast, has been on minimizing the number of samples required to test hypotheses with a strong control for both type I and type II errors. A few recent works have identified tight upper and lower bounds on the sample complexity of various testing problems~\cite{Paninski08,ValiantV14,AcharyaDK15,DiakonikolasK16}. All of the papers in this vast body of literature assume access to i.i.d. samples from the underlying distribution. 

%Classically testing goodness-of-fit of distributions has a long history in statistics, since the early days; for some old and some more recent references see, e.g.,~\cite{Pearson00,Fisher35,RaoS81,Agresti11}. Traditionally, the emphasis has been on the asymptotic analysis of tests, pinning down their error exponents as the number of samples tends to infinity~\cite{Agresti11,TanAW10}. In the last two decades or so, distribution testing  has also piqued the interest of  theoretical computer scientists, where the emphasis has been different~\cite{BatuFFKRW01,Paninski08,LeviRR13,ValiantV14,ChanDVV14, AcharyaDK15,CanonneDGR15,DiakonikolasK16,DaskalakisDSVV13,CanonneRS14}. In contrast to much of the statistics literature, the goal has been to minimize the number of samples required for testing.
%This recent work has identified tight upper and lower bounds on the sample complexity of various testing problems~\cite{Paninski08,ValiantV14,AcharyaDK15,DiakonikolasK16,Paninski08}. However, all of this vast body of literature assumes access to independent and identically distributed samples from the underlying distribution. 

Some work in Statistics has considered the problem of testing with dependent samples. For instance, \cite{Bartlett51, Moore82, GleserM83, MolinaMPV02} and the references therein study goodness-of-fit testing for Markov chains. \cite{TavareA83} and more recently \cite{BarsottiPR16} study the problem of testing the stationary distribution of Markov chains. \cite{Kazakos78} studies the problem of detection between  two Markov chains. All these works focus on the asymptotic regime where the length of the observed trajectories tends to infinity, as opposed to the non-asymptotic regime that we study here. In the computer science literature \cite{BatuFRSW13} considered the problem of testing the property whether a Markov chain is fast mixing or not. They defined a notion of closeness between two random walks started at different states of the same chain, which is similar in spirit to the distance notion we define in this work.

%There has been some work in the statistics community which looked at testing from dependent samples. For instance, \cite{Bartlett51, Moore82, GleserM83, MolinaMPV02} and the references therein study goodness-of-fit testing for Markov chains; \cite{TavareA83} and more recently \cite{BarsottiPR16} study the problem of testing the stationary distribution of Markov chains. \cite{Kazakos78} studies the problem of detection of one of two Markov chains.  All these works focus on the asymptotic regime where the number of samples tends to infinity as opposed to the finite sample regime which is of interest to us here. Within the computer science community \cite{BatuFRSW13} have looked at the problem of testing whether a Markov chain is fast mixing. They define a notion of closeness between two random walks on a Markov chain which is ideologically similar to the distance notion we define in this work.


There is a large body of statistical literature on estimating properties of Markov chains such as mixing time. The question of estimation is related to but different than the goodness-of-fit testing that we perform here. A particularly important parameter is the mixing time of a Markov chain, as it is useful in designing MCMC algorithms. \cite{HsuKS15} and the references therein study the problem of mixing time estimation in Markov chains.

==> pre-stoc18-version/riff_shuffle_test.tex <==
%As in the GSR and CD models described earlier, 
It is natural to parameterize a riffle shuffle by 
(i) the distribution of possible cuts, and (ii) the probability $p_{ab}$ of choosing the next card to be dropped from the left pile for each profile $(a,b)$ of the number of cards left in the two 
piles. In this description each riffle shuffle
can be represented as a random walk on a 2-dimensional grid $(a,b)\in\Z^2$ that starts at a position chosen from a specified distribution on the diagonal $a+b=n$ 
and decreases the sum of the coordinates $a+b$ by one at each move. In fact, we get an almost one-to-one correspondence between riffle shuffles and the aforementioned random walks 
on the $n\times n$ grid (the only shuffle that corresponds to more than one path on the grid is the identical permutation). Therefore, by knowing the initial permutation of cards at the beginning of the shuffle, and by scanning the permutation of cards obtained after
one riffle shuffle we can reconstruct (except for the unimportant case of void shuffle) the random walk of $n$ steps taken by our grid Markov Chain. 
We note that this grid representation might not be enough to accurately model the behavior of a dealer. For example, shufflers often tend to drop chunks of consecutive cards from left or right pile regardless of the pile sizes. To address this issue one might want to introduce 
an extra parameter -- which pile the last card was taken from -- to our grid parameterization, which can be done by doubling the number of states in the Markov 
chain. To capture this and other potential extensions of the Markov chain model for a riffle shuffle we introduce the following general theoretical framework.
 
\begin{definition}[Sparse MC]
\label{def:sparse}
Consider a Markov chain defined by transition matrices $P=\{P_t\}_{t=1}^{n_1}$ over $n_2$ states that proceeds in $n_1$-step rounds, as follows. Starting from some state $X_0=s_0$ it follows a transition according to $P_1$, then $P_2$, etc, then $P_{n_1}$ to arrive at some state $X_1$. Starting from $X_1$ it repeats transitions according to  $P_1,\ldots,P_{n_1}$, in sequence, and so on, ad infinitum. The transition matrices are assumed {\em sparse} having $O(n_3)$ non-zero entries.
\end{definition}
To relate the above definition to the riffle shuffle, we should think of the state space as the set $\{(a,b)| 0 \le a+b \le n\}$, where $n=52$. So in particular, there are $n_2=O(n^2)$ states. There are $n_1=n+1$ transition matrices. $P_1$ takes us from an uncut deck of cards, corresponding to the state $(0,0)$, to a cut deck corresponding to a state in set $\{(a,b)| a+b = n\}$. Then each other transition matrix $P_t$, $t >1$, maps a state in  $\{(a,b): a+b=n-t+2\}$ to states in $\{(a,b): a+b=n-t+1\}$. All transition matrices have $O(n)$ non-zero entries. Note that this way of modeling the riffle shuffle, while forgetting the specific ordering of cards, maintains the essential information that we need to test a riffle shuffle model, and in particular saves exponentially in the size of the state space.

%
%$n_1$ steps, and then repeats these $n_1$. Each transition matrix $P_t$ is a {\em sparse} matrix having at most $O(n)$ non zero entries. The initial distribution (e.g. the initial cut in the riffle shuffle) is modeled as a transition 
%matrix $P_1$ from a single state $\onee$ to the distribution over $n$ states (e.g. in the riffle shuffle the cut choose some state from $\{(a,b): a+b=n-1\}$), each of the matrices $\{P_t\}_{t\ge 2}$ describes transition probabilities among states (e.g. in the riffle shuffle matrix $P_t$ describes transition probabilities from states $\{(a,b): a+b=n-t+1\}$ to states $\{(a,b): a+b=n-t\}$).
%\end{definition}

\vspace{-10pt}\paragraph{Testing sparse Markov chains.} We develop tools for goodness-of-fit testing of sparse Markov chain models. 

\medskip \noindent {\bf Simplification:} To avoid carrying around several parameters, we will henceforth take $n_1=n_3=n$ and $n_2= O(n^2)$, which is what we would need for the riffle shuffle. Our results, namely the use and analysis of our edge tester, extend to the general case. We will also assume that $P_{n_1}$ is the trivial matrix taking all states into a fixed state $s_0$, which is also what we would need for the riffle shuffle, namely $s_0=(0,0)$. Again, our results easily extend to the general case. 

\medskip \noindent With these simplifications in place, we can break an observed trajectory from a sparse Markov chain model into ``samples.'' One sample is a 
word $w=s_0\cdots s_{n}$, whose transitions $s_{t-1}\to s_t$ are performed according to transition 
 matrix $P_t$. 

\smallskip As described in Section \ref{sec:distance}, a natural measure of distance between two Markov chains $Q=\MCseqQ$ and $P=\MCseqP$ is the total variation 
distance between words of certain length sampled from these chains.
 %distributions $\word{Q}{n}$ and $\word{P}{n}$, as it precisely captures our ability to distinguish
%which Markov chain $P$ or $Q$ a single word $w$ of length $n$ was generated from. 
As we have a natural length $n$ to use here, we can take our distance between chains to be $\dist{P}{Q}\eqdef\dtv{\word{P}{n}}{\word{Q}{n}}$.

We note that $\frac{\distsq{P}{Q}}{2}=\frac{\dtvsq{\word{P}{n}}{\word{Q}{n}}}{2}
\le\hellingersq{\word{P}{n}}{\word{Q}{n}}$ and for Hellinger-squared distance 
we can derive a formula similar to \eqref{eq:hellinger_square_algebraic}:
$
1-\hellingersq{\word{P}{n}}{\word{Q}{n}}=\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev.
$ In particular, we could alternatively define our distance using the spectral approach we took in Section~\ref{sec:symmetric}. 
%We show in Appendix~\ref{app:riffle_model} that the two notions are tightly related, but we opt for the use of total variation distance as we find it more natural in this context.
To this end we can define a large matrix $Q^*$ for 
Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$. 
%In our running application to card shuffling, it captures the divergence in one iteration of two riffle shuffles with different para total variation distance of the difference in one step of the shuffle.


%\begin{multline*}
%1-\hellingersq{\word{P}{n}}{\word{Q}{n}}=\sum_{w=s_0\ldots s_{n}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}
%=\trans{\left[\sum_{w=s_0\ldots s_{n-1}s}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{s\in[n]}\circ\onev\\
%=\trans{\left[\sum_{\substack{w=s_0\ldots s_{n-1}\\s_{n-1}=r}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{r\in[n]}\circ\srprod{P_n}{Q_n}\circ\onev
%=\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev.
%\end{multline*}


%\begin{itemize}
%\item Formulation as testing Markov Chains with $n$ steps on a $n\times n$ grid.
%\item General model: sparse Markov Chains with $n$ transition matrices $P_i$, each having a total number of $O(n)$ of non zero entries.
      %We model cut (initial distribution) as a transition $P_1$ from a single state $\onee$ to the distribution over $n$ initial states.    
%\end{itemize}
%
%Derivation of 
%$$\frac{\distsq{P}{Q}}{4}\le\hellingersq{P}{Q}=1-\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev$$
%\begin{remark}
%It is also possible to define $\dist{P}{Q}$ via the spectral radius approach as was done in Section \ref{sec:distance}. To this end we can define a large matrix $Q^*$ for 
%Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
%$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
%We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$.
%\end{remark}
%Alternative description as a long Markov Chain cycled from the state $t=n$ to states $t=0$ according to distribution $p_0$. 
%Relation between spectral radius $\rho(A)$ and $\dist{\MCseqP}{\MCseqQ}$.
%With this distance definition in hand it is a very reasonable question to ask:
%\begin{quote}
%Given a specific probabilistic model for shuffling (a sparse Markov chain $Q$), how many shuffles (samples) does one need to test whether $Q$ is an accurate model for shuffling?
%\end{quote}
With these definitions we are interested in the following testing problem:
%\begin{description}
%\item[Input:] $Q=\MCseqQ$, s.t. each $Q_t$ is sparse, i.e., it has only $O(n)$ non zero entries in total;
%$m$ samples of $w=s_0\cdots s_{n}$ from a sparse Makrov chain $P=\MCseqP$.
%\item[Output:] $P=Q$, or $P\neq Q$ if $\dist{P}{Q}\ge\eps$. 
%\end{description}

\begin{algorithm}[H]
\KwIn{$Q=\MCseqQ$, s.t. each $Q_t$ is sparse, i.e., it has only $O(n)$ non zero entries in total;
$m$ samples of $w=s_0\cdots s_{n}$ from a sparse Markov chain $P=\MCseqP$.}
\KwOut{$P=Q$, or $P\neq Q$ if $\dist{P}{Q}\ge\eps$.}
\end{algorithm}


==> pre-stoc18-version/riffle_model.tex <==
It is also possible to define $\dist{P}{Q}$ via the spectral radius approach as was done in Section \ref{sec:distance}. To this end we can define a large matrix $Q^*$ for 
Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$.


%A commonly used technique to shuffle decks of $n=52$ cards is the riffle shuffle:
%first, the dealer cuts the deck into two piles. Then, the piles are ``riffled'' together:
%the shuffler successively drops cards from the bottom of each pile to form a new pile. There
%are two variable aspects in this procedure. First, the numbers of cards in
%each pile after the initial cut can vary. Second, each time the dealer drops a card she needs to choose the pile from which the card is dropped.
%
%The standard and by far the most well studied mathematical model for riffle shuffle is due to Gilbert, Shannon, and Reeds (GSR-model for short): 
%first, the deck is cut into two packs according to a $(n,0.5)$-binomial random variable where $n$ is the number of cards in the deck; 
%next, cards are dropped one by one from the bottom of one or the other pile with probability proportional to the relative sizes of the
%piles (i.e., if the left pile contains $a$ cards and the right pile $b$ cards, the next card drops from the left pile with probability 
%$\frac{a}{a + b}$). A well known result in this model is due to Bayer and Diakonis~\cite{BayerDiaconis} who gave a sharp mathematical 
%analysis of the mixing time of the riffle shuffle Markov chain showing that ``seven shuffles are necessary and sufficient to approximately randomize $52$ cards'', which actually convinced Las Vegas 
%casinos to increase the number of shuffles in their shuffling procedures.
%
%% Emperical work
%There have also been some statistical studies validating the adequacy of the GSR model for riffle shuffles in practice.
%For example Diaconis and Reeds (see~\cite{DiaconisLectures88}) did empirical analysis of about a hundred riffle shuffles performed by each of them.
%They looked at a few different statistics including the count of consecutive cards dropped from each of the piles. These statistics revealed certain differences between the two
%shufflers, in particular, Diaconis' shuffles (a former professional magician) were much neater and closer to the shuffles of professional dealers in Las Vegas casinos, 
%while Reeds' shuffles were more like ``ordinary person'' shuffles. In another work (see~\cite{DiaconisTechReport02} open problem 5) Chakraborty and Diakonis 
%pointed out that some shuffling machines performing riffle shuffles do not conform to the GSR model. Instead they proposed 
%another model to capture this observed phenomenon (we call it {\em CD-model}), where, in contrast to the GSR model, cards are dropped with probability $\frac{a}{a+b}$ from the pile containing $b$ cards 
%and $\frac{b}{a+b}$ from the pile containing $a$ cards.
%
%Despite a large interest in card shuffling and all the existing work mentioned above, there has not been much theoretical statistical 
%analysis on the question of testing whether a particular shuffling model is accurate. 


==> pre-stoc18-version/shuffle_model.tex <==
A commonly used technique to shuffle decks of $n=52$ cards is the riffle shuffle:
first, the dealer cuts the deck into two piles. Then, the piles are ``riffled'' together:
the shuffler successively drops cards from the bottom of each pile to form a new pile. There
are two variable aspects in this procedure. First, the numbers of cards in
each pile after the initial cut can vary. Second, each time the dealer drops a card she needs to choose the pile from which the card is dropped.

The most well studied mathematical model for riffle shuffle is due to Gilbert, Shannon, and Reeds (GSR-model for short): 
first, the deck is cut into two packs according to a $(n,0.5)$-binomial random variable where $n$ is the number of cards in the deck; 
next, cards are dropped one by one from the bottom of one or the other pile with probability proportional to the relative sizes of the
piles (i.e., if the left pile contains $a$ cards and the right pile $b$ cards, the next card drops from the left pile with probability 
$\frac{a}{a + b}$). A well known result in this model is due to Bayer and Diaconis~\cite{BayerDiaconis} who gave a sharp mathematical 
analysis of the mixing time of the riffle shuffle Markov chain showing that ``seven shuffles are necessary and sufficient to approximately randomize $52$ cards,'' which actually convinced Las Vegas 
casinos to increase the number of shuffles in their shuffling procedures.

% Emperical work
There have been some statistical studies validating the accuracy of the GSR model for riffle shuffles in practice.
For example Diaconis and Reeds (see~\cite{DiaconisLectures88}) did empirical analysis of about a hundred riffle shuffles performed by each of them.
They looked at a few different statistics including the count of consecutive cards dropped from each of the piles. 
%These statistics revealed certain differences between the two
%shufflers: Diaconis' shuffles (a former professional magician) were much neater and closer to the shuffles of professional dealers in Las Vegas casinos, 
%while Reeds' shuffles were more like ``ordinary person'' shuffles. 
In other work (see~\cite{DiaconisTechReport02} open problem 5), Chakraborty and Diaconis 
pointed out that some shuffling machines performing riffle shuffles do not conform to the GSR model. Instead they proposed 
another model to capture this observed phenomenon (we call it {\em CD-model}), where, in contrast to the GSR model, cards are dropped with probability $\frac{a}{a+b}$ from the pile containing $b$ cards 
and $\frac{b}{a+b}$ from the pile containing $a$ cards.

Despite a large interest in card shuffling and all the existing work mentioned above, there has not been much theoretical statistical 
analysis on the question of testing whether a particular shuffling model is accurate. In this section we propose a new theoretical 
framework for the statistical analysis of riffle shuffles. We aim to address the following question:
\begin{quote}
How many trials are needed to test that shuffles are performed according to a specified probabilistic model?   
\end{quote}





==> pre-stoc18-version/sparse_lb.tex <==
In this section we will show that any algorithm that tests identity of a sparse Markov chain representing 
card riffle shuffling requires at least $\Omega\left({\frac{n}{\eps^2}}\right)$ independent trials, where 
each trial is a $n$-length word generated by a sparse Markov chain.
We recall Definition~\ref{def:sparse} of a sparse Markov chain adapting it slightly for the convenience of lower bound presentation.
Sparse Markov chains $P=\{P_t\}_{t=1}^{T}, Q=\{Q_t\}_{t=1}^{T}$: each independent run consists of $T=O(n)$ time steps; has $O(n)$ states for each time $t$;  Markov chain starts
from a single state at $t=0$ ; there are only $O(1)$ possible transitions $P_t(ij)\neq 0$ from each state 
$i$ to other states for all but the very first time step $t>0$.

\begin{theorem}
\label{thm:sparse-lower-bound}
There is an instance of Identity testing problem for a sparse Markov chain $Q$ that requires
at least $m\ge\Omega(\frac{n}{\eps^2})$ i.i.d. samples to check identity of $Q$ with $99$\% confidence\footnote{We assume
	$\eps=\omega(n^{-1/6})$ in the requirement $\dist{P}{Q}\ge\eps$, when $P\neq Q$.}.
%There exists a constant $c>0$, such that any algorithm which, given the description of a sparse Markov chain $Q$ with 
%$O(n)$ layers and each layer containing $O(n)$ states, and sample access to words from another sparse Markov chain $P$ 
%over the same set of states as $Q$, distinguishes between the cases $P \equiv Q$ and $\dist{P}{Q} \ge \eps$ with 
%probability at least $99/100$ requires at least $k \geq \frac{cn}{\eps^2}$ samples.
\end{theorem}
%Complete argument is provided in Appendix~\ref{app:sec_riffle_lb}. 

\begin{proof}
	The high-level proof idea is similar to that of Theorem~\ref{thm:symm-lower-bound}, but particular details and proofs are more involved. At an abstract level, we construct a sparse Markov chain $Q$, 
	with respect to which we are interested in testing identity, and a class of sparse Markov chains $\mathcal{P}$ such that 
	\begin{enumerate}
		%\item $\mathcal{Q}$ is a single Markov chain $Q$ which identity we are testing. 
		\item Every $P \in \mathcal{P}$ is at least $\eps$ far from $Q$, i.e., $\dtv{\word{P}{T}}{\word{Q}{T}}\ge \eps$ for any $P \in \mathcal{P}$.
		\item There is a constant $c > 0$, such that it is impossible to distinguish $m$ i.i.d. samples of $T$-length words generated by 
		a random Markov chain $\bar{P}\sim \mathcal{P}$ from the samples produced by $Q$ with probability 
		equal to or greater than $\frac{99}{100}$, for $m\le\frac{cn}{\eps^2}$.
	\end{enumerate}
	
	We denote the joint distribution of $m$ i.i.d. samples from $Q$ by $Q^{\otimes m}$ and that from $\bar{P}$ by $\bar{P}^{\otimes m}$.
	To prove the last point we show that $\dtv{Q^{\otimes m}}{\bar{P}^{\otimes m}}$ is small for some $m=\Om{\frac{n}{\eps^2}}$.
	We now describe our construction. To simplify presentation, we use multi-edges in the description of sparse Markov chains.
	We convert this instance into simple edge graph by the same duplicating trick we employed in 
	the lower bound construction of Theorem~\ref{thm:symm-lower-bound}.
	
	%We respectively denote the words of length $m$ obtained from $Q$ by $\word{Q}{m}$, and from a Markov chain $\bar{P}\sim\mathcal{P}$ by $\word{\bar{P}}{m}$.\\
	%We will assume $n$ is odd without loss of generality for the following lower bound construction.
	%\noindent 
	
	
	\begin{description}
		\item[Markov Chain $Q$:] $T=2n+1$ time steps; single state at $t=0$, states $[2n]$ at each $1\le t\le T$.
		All states are divided into two categories: {\em Frequently} visited ($F$) $\eqdef\{2i-1, i\in[n]\}$ and {\em Rare} ($R$) $\eqdef\{2i,i\in[n]\}$.
		Table below describes weighted multi-graph $Q=\{Q_t\}_{t=1}^{T}$: $x\in F,$ $y\in R$, $x,y\in [2n]$ denote respective generic frequent and rare states. 
		We adopt notational convention: $0\eqdef 2n$, $2n+1\eqdef 1$.   
		
		\begin{tabular}{r|c|c|c|c}
			&  $F\to F$        & $F\to R$       & $R\to F$       &     $R\to R$   \\ 
			%				&  $(2i\to 2j)$    & $(2i\to 2j+1)$ & $(2i+1\to 2j)$ & $(2i+1\to 2j+1)$ \\ 
			\hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=1:} }
			&  $(1\to x)\in E$                  & \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} 
			& \multicolumn{1}{|c}{\multirow{2}{*}{$\emptyset$}}                  \\ %\hline
			& $Q_{1}(1,x)=\frac{1}{n}$       &                                                   &                                                     &              \\ \hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=2k:} }
			& $(x\to x)\in E$             &  $(x\to x\pm 1)\in E$           &  $(y\to y\pm 1)\in E$           & \multicolumn{1}{|c}{\multirow{2}{*}{$\emptyset$}}     \\ %\hline
			& $Q_t(x,x)=1-\frac{2}{n}$ &  $Q_t(x,x\pm 1)=\frac{1}{n}$ &  $Q_t(y,y\pm 1)=\frac{1}{2}$ &                                                       \\ \hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=2k+1:} }				
			&  $(x\to x)\in E$            &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} 
			&  $(y\to y)_{1,2}\in E$                               \\ %\hline
			&  $Q_t(x,x)=1$            &                                                     &                                                     
			&  $Q_t(e_1)=Q_t(e_2)=\frac{1}{2}$                                  \\ %\hline
		\end{tabular}
		%\begin{align*}
		%t=1:& \quad\quad \forall 2i+1\in[2n]\quad \quad (1,2i+1)\in E\quad  \quad Q_{1}(1\to 2i+1)=\frac{1}{n}\\
		%t=2k:& \quad\quad \forall i\in[2n]\quad \quad (1i)\in E\quad  \quad Q_{1}(1i)=\frac{1}{2n}\\
		%t=2k+1:& \quad\quad \forall i\in[2n]\quad \quad (1i)\in E\quad  \quad Q_{1}(1i)=\frac{1}{2n}
		%%Q_{(ij)_1}=\frac{1}{2(n-1)} \quad\quad Q_{(ij)_2}=\frac{1}{2(n-1)}\quad\quad \text{ for any } i\neq j.
		%\end{align*}
		\item[Family $\mathcal{P}$:] every $P \in \mathcal{P}$ has the same set of states and edges as $Q$.
		Similar to the construction in Section~\ref{sec:symmetric_lb}, we only change weights of the multi-edge 
		pairs (independently and uniformly at random for each pair $(y\to y)_{1,2}$ and time $t$): 
		\[
		P_{t}(e_{1,2})=\frac{1\pm 4\eps}{2} \quad\quad\text{ or }\quad\quad
		P_{t}(e_{1,2})=\frac{1\mp 4\eps}{2}.
		\]
	\end{description}
	
	%The family $\mathcal{P}$ of Markov chains is constructed by making slight random perturbations to the multi-edge 
	%transitions in $Q$. In particular, every $P \in \mathcal{P}$ has the same set of states as $Q$. In each $P$, every 
	%transition is identical to those in $Q$ except the multi-edge transition probabilities from a rare state in an 
	%even-indexed layer to the corresponding rare state in the next layer. Instead of having a $1/2$ transition probability 
	%on each edge from $(2i,2t)$ to $(2i,2t+1)$, we will have as transition probabilities either $1/2(1 \pm 2\eps)$ or 
	%$1/2(1 \mp 2\eps)$ chosen uniformly at random. Hence this creates a class of sparse Markov chains which contains 
	%$2^{O(n^2)}$ sparse Markov chains.
	%
	%
	%\begin{itemize}
	%\item \textbf{The Markov Chain $Q$}\\
	%$Q$ will have $2n+1$ layers each with $n$ states along with an additional initial layer which has transitions with 
	%probability $2/n+1$ from state 1 to each of the odd indexed states in layer 2. Label the states in layer $t$ as 
	%$(1,t),(2,t)\ldots,(n,t)$. States $(2i-1,t)$ are frequent states and states $(2i,t)$ are rare states for each $t > 1$. 
	%From every frequent state in an even-indexed layer $(2i-1,2t)$, there exists a transition to frequent state $(2i-1,2t+1)$ 
	%with probability $(1-2/n)$ and a transition to rare state $(2i,2t+1)$ with probability $1/n$ and to rare state 
	%$(2i-2,2t+1)$ with probability $1/n$. If $i=1$ (or $i=n$), then for any even-indexed layer $2t$ there is a transition 
	%from $(1,2t)$ ($(n,2t)$) to the rare state $(2,2t+1)$ ($(n,2t+1)$) with probability $2/n$ instead. From every frequent 
	%state in an odd-indexed layer $(2i-1,2t-1)$ there is a transition to the frequent state $(2i-1,2t)$ with probability 1. 
	%From each rare state in an even-indexed layer $(2i-1,2t)$, there are two transitions to rare state $(2i-1,2t+1)$ with 
	%probability $1/2$ and $1/2$. These are the only multi-edge transitions in the construction of $Q$. From each rare state 
	%in an odd-indexed layer $(2i,2t+1)$, there are transitions with probability $1/2$ to frequent states $(2i+1,2t+2)$ and 
	%with probability $1/2$ to $(2i-1,2t+2)$. This completes a description of the construction of the sparse Markov chain $Q$.
	%
	%\item \textbf{Constructing the family $\mathcal{P}$}\\
	%The family $\mathcal{P}$ of Markov chains is contructed by making slight random perturbations to the multi-edge 
	%transitions in $Q$. In particular, every $P \in \mathcal{P}$ has the same set of states as $Q$. In each $P$, every 
	%transition is identical to those in $Q$ except the multi-edge transition probabilities from a rare state in an 
	%even-indexed layer to the corresponding rare state in the next layer. Instead of having a $1/2$ transition probability 
	%on each edge from $(2i,2t)$ to $(2i,2t+1)$, we will have as transition probabilities either $1/2(1 \pm 2\eps)$ or 
	%$1/2(1 \mp 2\eps)$ chosen uniformly at random. Hence this creates a class of sparse Markov chains which contains 
	%$2^{O(n^2)}$ sparse Markov chains.
	%\end{itemize}
	
	%\begin{remark}
	%To convert the above constructions involving multi-edges into ones with simple edges we do the following. Firstly, 
	%note that the only multi-edge transitions are from a rare state to another rare state. To make this instance a simple 
	%graph with at most one directed edge between any pair of vertices we apply a standard graph theoretic transformation: 
	%we make a copy $i'$ for each vertex $i$ involved in a double edge; for each pair of double edges $e_1=(ij)_1, e_2=(ij)_2$ 
	%construct $4$ edges $(ij),(ij'),(i'j),(i'j')$ with weights $w(ij)=w(i'j')=w(e_1)$ and $w(ij')=w(i'j)=w(e_2)$. This 
	%increases the total number of states in a layer by a factor of $3/2$.
	%\end{remark}
	
	%Now, we state a simple claim about the distance between two sparse Markov chains.
	%\begin{claim}
	%\label{clm:dist-monotone}
	%Consider two sparse Markov chains $P$ and $Q$, each with $n$ layers. For any $1 \le t \le n$, let
	%$$\hellingersq{P}{Q}_t = 1 - \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\onev.$$
	%Then, we have that, for any $1 \le t < n$,
	%$$\hellingersq{P}{Q}_t \le \hellingersq{P}{Q}_{t+1}.$$
	%\end{claim}
	%\begin{proof}
	%Let $\vect{v}^{\top} = \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}$. Then $\vect{v}^{\top} 
	%\circ \onev =  \onenorm{\vect{v}}$. Since $P_{t+1}$ and $Q_{t+1}$ are stochastic matrices, 
	%$\srprod{P_{t+1}}{Q_{t+1}}$ has non-negative entries and moreover from Perron-Frobenius theorem we have that 
	%$\srprod{P_{t+1}}{Q_{t+1}} \circ \onev \le \onev$ entry-wise. Hence $\vect{v}^{\top} \circ 
	%\srprod{P_{t+1}}{Q_{t+1}} \circ \onev \le \onenorm{\vect{v}}$ implying the claim.
	%\end{proof}
	
	The idea of this construction is that a typical trajectory of Markov chain $Q$ or $P\in\mathcal{P}$ 
	stays in frequent states almost all the time and very rarely visits one of the rare states.  However,
	a typical trajectory has constant probability of visiting a rare state.
	\begin{lemma}
		\label{clm:p-far-from-q shuffle}
		Any $P \in \mathcal{P}$ is at least $\eps$-far from $Q$, i.e., $\dist{P}{Q}= \dtv{\word{P}{T}}{\word{Q}{T}}\ge\eps$.
	\end{lemma}
	\begin{proof}
		Consider a $P \in \mathcal{P}$. First, we argue that probability of any word $w$
		with only a single visit to a rare state (at even $t=2k$) satisfies $\left| \Prx[Q]{w} - \Prx[P]{w}\right|  = 4\eps\cdot\Prx[Q]{w}.$
		%We will show $\dist{P}{Q}$ is large by arguing that the probability of any word 
		%with only one visit to a rare state at even time step $t=2k$ differs under $Q$ and under $P$ by at least $2\eps$ factor. 
		Indeed, let visit to the rare state $2i$ in $w$ happen at the time $t=2k$, then
		\[
		\begin{cases}
		\Prx[Q]{w} = \Prx[Q]{s_1 \ldots s_{2k}}\cdot \frac{1}{2} \cdot \Prx[Q]{s_{2k+1} \ldots s_{2n+1}|s_{2k+1}}\\
		\Prx[P]{w} = \Prx[P]{s_1 \ldots s_{2k}}\cdot \frac{1}{2}(1 \pm 4\eps) \cdot \Prx[P]{s_{2k+1} \ldots s_{2n+1}|s_{2k+1}}.
		\end{cases}
		\]
		Therefore, as $Q$ and $P$ have the same transitional probabilities of $s_t\to s_{t+1}$ for $t\neq 2k$, we get 
		$$\left| \Prx[Q]{w} - \Prx[P]{w}\right|  = 4\eps\cdot\Prx[Q]{w}.$$ 
		Now, the probability of visiting a rare state exactly once (at even $t$) in $Q$ is precisely 
		\[
		\sum_{\substack{w \text{ with}\\ \text{1 rare visit}}} \Prx[Q]{w} = n\cdot\frac{2}{n}\cdot\left(1-\frac{2}{n}\right)^{n-1}> 2\cdot e^{-2}>\frac{1}{4},
		\]
		where we used inequality $(1-\frac{1}{n})^{n-1}> e^{-1}$ to get the estimate in the right hand side.
		%The probability of 0 visits to rare states is $(1-2/n)^{n} \le e^{-4}$. Conditioned on there being a visit to a 
		%rare state, the probability of 0 additional visits to rare states in even-indexed layers is $(1-2/n)^{2n-2} \le 
		%4e^{-4}$ for $n \ge 4$. Hence the probability of exactly one rare state visit in an even-indexed layer is 
		%$\ge (1-e^{-4})(1-4e^{-4}) \ge 1/2$. 
		Hence, 
		\begin{align*}
		\dtv{\word{P}{T}}{\word{Q}{T}} \ge \sum_{\substack{w \text{ with}\\ \text{1 rare visit}}} 
		\left|\Prx[Q]{w} - \Prx[P]{w}  \right| =  \sum_{\substack{w \text{ with}\\ \text{1 rare visit}}}4\eps\cdot\Prx[Q]{w} 
		\ge 4\eps\cdot\frac{1}{4} = \eps.
		\end{align*}
		%From the relation between total variation and Hellinger squared distances and Claim \ref{clm:dist-monotone}, we 
		%have that, $\dist{P}{Q} \ge \hellingersq{P}{Q} \ge \hellingersq{P}{Q}_2$. Under our construction, $\oneet \circ 
		%\srprod{P_1}{Q_1} = \frac{1}{n}\onev^{\text{T}}$ and it can be seen that $\oneet \circ \srprod{P_1}{Q_1} \circ 
		%\srprod{P_2}{Q_2} \circ \onev \le 1-\eps$. Hence $\hellingersq{P}{Q}_2 \ge \eps$ thereby proving the claim.
	\end{proof}
	
	
	%We group transitions within a single word into two categories: Those which occur from a frequent state and those 
	%which occur from a rare state. Note that from a rare state, the transition has to happen to a frequent state. 
	We define collisions and $3$-way collisions similar to the proof of Theorem~\ref{thm:symm-lower-bound}. Namely,
	a collision is a transition that occurs in two samples (3-way collision -- in at least three samples) of $Q^{\otimes m}$ or $P^{\otimes m}$ from the 
	same state and at the same time. Moreover, as $P\sim\mathcal{P}$ and $Q$ are the same except for the double edges
	between rare states, we are only interested in the collisions along multi-edges between rare states. 
	%If the same transition repeats in two samples, we call it a collision. If it occurs in 3 distinct samples, we 
	%call it a 3-way collision. We make the following observations about $Q$ and $\mathcal{P}$.
	
	
	\begin{lemma}
		\label{clm:num-collisions shuffle}
		The expected number of collisions in samples $Q^{\otimes m}$ is $O\left(\frac{m^2}{n^2} \right) = O\left(\frac{1}{\eps^4} \right)$.
		%Consider a sample from $Q^{\otimes m}$. The expected number of collisions among transitions from a rare state 
		%to another rare state is $O\left(\frac{m^2}{n^2} \right) = O\left(\frac{1}{\eps^4} \right)$.
	\end{lemma}
	\begin{proof}
		Let $I_w(m_1,m_2,y,t)$ indicate the event that either of the transitions along edges $e_{1,2}=y\to y$ at time $t$, occurred in samples $m_1$ and $m_2$. 
		Note that at each fixed time all of the $n$ frequent states are equally likely to occur in a sample from $Q$. Therefore, the probability of visiting given
		rare state $y$ at time $t$ in a single run is at most $O(1/n^2)$. 
		%probability is uniformly spread over all $n$ frequent states and the probability of 
		%transitioning to a rare state from a frequent state is $2/n$.
		This implies 
		$\Prx[Q]{I_w(m_1,m_2,y,t) = 1} = O\left(\frac{1}{n^2}\cdot \frac{1}{n^2}\right) = 
		O(1/n^4)$.
		%because at each time probability is uniformly spread over all $O(n)$ frequent states and the probability of 
		%transitioning to a rare state from a frequent state is $2/n$. 
		Let $X$ denote the total number of collisions.
		\begin{align*}
		\Ex{X} &= \sum_{m_1 \neq m_2}\sum_{i\neq j} \Ex{I_w(m_1,m_2,y,t)} = O\left(m^2n^2 \frac{1}{n^4} \right) = 
		O\left(\frac{m^2}{n^2} \right)
		\end{align*}
	\end{proof}
	
	
	\begin{lemma}
		\label{clm:3-way collision shuffle}
		The probability of a 3-way collision in samples $Q^{\otimes m}$ is $o(1)$.
		%Consider $m=\frac{n}{\eps^2}$ samples from either $Q$. The probability of a 3-way collision 
		%among the $m$ samples is $o(1)$.
	\end{lemma}
	\begin{proof}
		Similar to the proof of Lemma~\ref{clm:num-collisions shuffle} we can give an upper bound on the expected number of 
		$3$-way collisions being $\Ocomplex{n^2m^3\cdot\frac{1}{n^6}\cdot }=\Ocomplex{\frac{m^3}{n^4}}$. Markov's inequality concludes 
		the proof.
	\end{proof}
	
	Now consider a typical set of $m$ words generated by $Q$ (or equivalently drawn from $Q^{\otimes m}$).
	%$\bar{P}\sim\mathcal{P}$. 
	As we know from Lemma~\ref{clm:3-way collision shuffle} it has no 3-way collisions and by Markov's inequality 
	and Lemma~\ref{clm:num-collisions shuffle} has at most $O(\frac{1}{\eps^2})$ collisions with probability greater 
	than $9/10$ (for sufficiently small $c>0$ and $m=\frac{cn}{\eps^2}$). As we show next a typical set of $m$ words drawn from 
	$Q$ has similar probability under the $\bar{P}\sim\mathcal{P}$ and $Q$ models.
	
	\begin{lemma}
		\label{clm:no-collision-analysis shuffle}
		At least $1/2$ of the sets $S = \{w_1,\ldots,w_m\}$ of samples from $Q^{\otimes m}$ satisfy 
		$$ \frac{1}{2}\cdot\prob[Q^{\otimes m}]{S}<\prob[\bar{P}^{\otimes m}]{S} < 2\cdot \prob[Q^{\otimes m}]{S}$$
	\end{lemma}
	\begin{proof}
		We consider the ratio of the respective probabilities $(*)\eqdef\frac{\prob[\bar{P}^{\otimes m}]{S}}{\prob[Q^{\otimes m}]{S}}$. As in 
		Lemma~\ref{clm:no-collision-analysis}, both probabilities in the numerator and denominator can be expressed in terms of 
		simple statistics for the set $S$, specifically the number of single step transitions between pairs of states. 
		Also similar to the Lemma~\ref{clm:no-collision-analysis}, the corresponding multiplicative terms for $\bar{P}^{\otimes m}$ 
		and $Q^{\otimes m}$ are identical except for the collisions along multi-edges between two rare states (at least two transitions between
		a pair of rare states). Moreover, we also differentiate type I and type II collisions between rare states: (type I) transitions between
		rare states $y\to y$ at time $t$ were made along different edges $e_1$ and $e_2$; (type II) two transitions were made along the same edge
		either $e_1$, or $e_2$. Per type I and II collisions the corresponding terms in $(*)$ are respectively
		$(1-4\eps)(1+4\eps)=1-16\eps^2$ and $1+16\eps^2$.
		
		We further continue following the proof of the Lemma~\ref{clm:no-collision-analysis}, and make sure that with high probability there are only $X=O(\frac{1}{\eps^4})$ collisions and
		no $3$-way collisions in $S$. We can make sure that the difference between numbers of type I and type II collisions is at most $O(\sqrt{X})=O(\frac{1}{\eps^2})$ 
		with probability at least $3/4$, as the choice of collision type in $w$ under $Q$ model is uniform between type I and type II and independent across different collisions.
		For small enough $m=\Omega(\frac{n}{\eps^2})$ we can make sure that at least $\frac{1}{2}$ fraction of words $w$ under $Q$ model have the number of collisions
		at most $\frac{c_1}{\eps^4}$ and also have the difference between number of type I and type II collisions at most $\frac{c_2}{\eps^2}$, for some small constants $c_1,c_2>0$.
		In this case we get the following bounds on $(*)$.
		\[
		2>\left(1+16\eps^2\right)^{\frac{c_2}{\eps^2}}>\frac{\prob[\bar{P}^{\otimes m}]{S}}{\prob[Q^{\otimes m}]{S}}>
		\left(1-256\eps^4\right)^{\frac{c_1}{2\eps^4}}\cdot \left(1-16\eps^2\right)^{\frac{c_2}{\eps^2}}>1/2
		\]
		
		
		%For each feasible set of samples $S$ under $Q$, i.e., $S$ such that $\prob[Q]{S}>0$
		%\[
		%\Prlong[Q]{S}=\left(\frac{1}{2(n-1)}\right)^{m-1}
		%\quad\quad 
		%\Prlong[\bar{P}\sim\mathcal{P}]{w}=\prod_{j>i}\sum_{\bar{P}_{(ij)_1}=\frac{1\pm\sqrt{8\eps}}{2(n-1)}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|} 
		%\]
		%
		%First, if $w$ has only one transition along edge $(ij)$, then the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{w}$ 
		%\[
		%\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1}{2}\left(\frac{1+\sqrt{8\eps}}{2(n-1)}+\frac{1-\sqrt{8\eps}}{2(n-1)}\right)=
		%\frac{1}{2(n-1)}.
		%\]
		%From Claim \ref{clm:3-way collision shuffle}, we know that probability of a $3$-way collision in $S$ is $o(1)$ under $Q$ model. We observe that for a $2$-way collision $(ij)$
		%(a collision which is not a $3$-way collision), the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{S}$  for the case of transition along two different 
		%edges $(ij)_1$ and $(ij)_2$ is
		%\[
		%\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1+\sqrt{8\eps}}{2(n-1)}\cdot\frac{1-\sqrt{8\eps}}{2(n-1)}=
		%\frac{(1-8\eps)}{4(n-1)^2}.
		%\] 
		%We call this type of collision {\em type I} collision. For the other case ({\em type II} collisions) of transition along the same edges the respective probability is 
		%$\frac{(1+8\eps^2)}{4n^2}$. By Claim~\ref{clm:num-collisions shuffle} and by Markov inequality the total number of collisions is $O(\frac{1}{\eps^4})$ with probability $\frac{3}{4}$. 
		%We can also make sure that out of these collisions number of type I and type II collisions is roughly the same. More precisely, the difference between numbers of 
		%type I and type II collisions is at most $O(\frac{1}{\eps^2})$ with probability of at least $\frac{3}{4}$. Indeed, the choice of edge collision type in $w$ is uniform 
		%between type I and type II, and is independent across all collision edges. Now, for small enough $m$ we can make sure that at least $\frac{1}{2}$ fraction of words $w$ 
		%has number of collisions at most $\frac{c_1}{\eps^4}$ and the difference between number of type I and II collisions is at most $\frac{c_2}{\eps^2}$, for some small 
		%constants $c_1,c_2>0$. Thus the corresponding density functions can be related as follows.
		%\[
		%2>\left(1+8\eps^2\right)^{\frac{c_2}{\eps^2}}>\frac{\prob[\bar{P}\sim\mathcal{P}]{w}}{\prob[Q]{w}}>
		%\left(1-64\eps^4\right)^{\frac{c_1}{2\eps^4}}\cdot \left(1-8\eps^2\right)^{\frac{c_2}{\eps^2}}>1/2
		%\]
	\end{proof}
	
	Lemma~\ref{clm:no-collision-analysis shuffle} shows that $\dtv{Q^{\otimes m}}{\bar{P}^{\otimes m}} \leq \frac{3}{4}$ for $m 
	\leq \frac{cn}{\eps^2}$ for some constant $c$, which implies that no algorithm can successfully distinguish $Q$ from the family 
	$\mathcal{P}$ with probability greater than $\frac{3}{4}$ for some $m=\Omega(\frac{n}{\eps^2})$.
\end{proof}

==> pre-stoc18-version/sparse_ub.tex <==
For the upper bound, one might consider an appropriately defined statistic on the number of visits to a particular state $s_{i,t}$ to distinguish between the two cases. Such statistics however can be mathematically difficult to deal with and we obtain worse bounds on the moments. In this paper, instead, we consider a different statistic. We look at all one-step transitions that can have positive probability in the Markov chain $Q$ or $P$, we call these one-step transitions as {\em edges}. 
We denote a generic edge from a state $s_{i,t-1}$ to a state $s_{j,t}$ by $e$; the set of all possible edges by $E$; the set of transitions in $E$ between 
states at time $t-1$ and time $t$ by $E(t)$ for each $t\in[n]$. For each edge $e$, let $q_e$ and $p_e$ be the probabilities that there was a transition along 
edge $e$ in one sample $s_1\cdots s_n$ from $Q$, or from $P$, respectively. Our statistic is defined on these edges. From a high level perspective, it consists of two steps: 

\paragraph{Pruning.} We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. We show that the Markov chain obtained post pruning and renormalization is still close to the original chain (Lemma \ref{cl:rejection_Q}). This step is necessary as rare instances of such transitions along {\em rare edges} could potentially shift the value of the statistic by a lot and we want to avoid that. Let $E^*$ be 
the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
rejected samples. Otherwise, we continue to the next step. In Lemma \ref{cl:error_prob_pruning} we show that returning $P \neq Q$ in this step doesn't affect the success probability by too much.
\paragraph{$\chi^2$-statistic on edges.} For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
  \[
      Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
  \]
We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold. This test is similar in spirit to that of \cite{AcharyaDK15} but requires much more involved analysis.
Indeed, in our stetting it is not clear which statistic to use: one can attempt to count frequencies of state visits in the MC, or employ other state dependent statistics.
After many trials and errors we figured out that doing the analysis across separate edges was the best approach.
Indeed, since we are dealing with non i.i.d. but dependent samples, obtaining a non-trivial variance bound for our edge statistic proves to be a challenging task. 
Similar to the classical i.i.d. setting, Poissonization helps to ease the analysis in our setting too. However, we rely on it in more subtle way: 
the effects of Poissonization at the top layer of $n$ states percolate nicely through to the bottom layers of the chain as shown in Lemma~\ref{cl:ind_poisson}. We show that $\Var{Z} = \Ocomplex{kn^3}$ 
in Lemmas~\ref{cl:var_z} and~\ref{cl:var_z_easy}. Another challenge for us was to relate the new definition of distance between two non stationary Markov chains with 
the parameters in the description of their kernels, as e.g. in our Lemma~\ref{cl:expectation_dist}.
%\begin{description}
 %\item[Pruning.] We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. Let $E^*$ be 
%the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
%rejected samples. Otherwise, we continue to the next step.
 %\item[$\chi^2$-statistic on edges.] For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
%{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
  %\[
      %Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
  %\]
  %We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold.
%\end{description}
Our $\chi^2$ test yields the following guarantee on the number of samples
\begin{theorem}
There is an algorithm that can tell whether $P=Q$, or $P\neq Q$, when $\dist{P}{Q}\ge\eps$,  
with probability at least $\frac{2}{3}$ using $O(\frac{n^{3/2}}{\eps^2})$ samples.
\label{th:main_shuffling}
\end{theorem}
Note that, while we state the above theorem in terms of the number of samples, we really mean that we observe a single trajectory from the sparse Markov chain which we have partitioned into segments of length $n$. In particular, the length of the required trajectory for the above statements is a factor of $n$ larger than the stated number of samples. Additionally note that to properly compare to our results from Section~\ref{sec:symmetric} we should note that the number of states here is $O(n^2)$.
All details are provided in Section~\ref{sec:riffle_ub_details}. We also have a complementary lower bound which is presented in Section \ref{sec:sparse_lb}. 


\subsection{More Details on the Tester for Sparse Markov Chains}
\label{sec:riffle_ub_details}
We consider all one-step transitions that can have positive probability in the Markov chain $Q$ or $P$, we call these one-step transitions as {\em edges}. 
We denote a generic edge from a state $s_{i,t-1}$ to a state $s_{j,t}$ by $e$; the set of all possible edges by $E$; the set of transitions in $E$ between 
states at time $t-1$ and time $t$ by $E(t)$ for each $t\in[n]$. 
%We also add new edges $E(0)$ to $E$, which indicate transitions to the original states at 
%time $t=0$ with positive probabilities in $q_0$ or $p_0$. 
For each edge $e$, let $q_e$ and $p_e$ be the probabilities that there was a transition along 
edge $e$ in one sample $s_1\cdots s_n$ from $Q$, or from $P$, respectively.
Our test, from a high level perspective, consists of two steps: 
\begin{description}
	\item[Pruning.] We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. Let $E^*$ be 
	the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
	rejected samples. Otherwise, we continue to the next step.
	\item[$\chi^2$-statistic on edges.] For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
	{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
	\[
	Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
	\]
	We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold.
\end{description}
In the remainder of this section we mostly focus on the latter step. Specifically, we analyze the $\chi^2$ edge statistic in the case when 
$q_e\ge\Omega(\frac{\eps^2}{n^2})$ for all $e\in E$ and $p_e=0$ for all $e\notin E$. At the end of the section we explain why after the pruning step these conditions 
are satisfied. 

%Poisson number of samples with expectation $m$.
\paragraph{Poisson Sampling.} Throughout the analysis of $\chi^2$ statistic, we use the standard Poissonization approach. 
Instead of drawing exactly $m$ samples from $P$, we first draw $m'\sim\Poisson{m}$, and then draw $m'$ samples from $P$. 
The benefit of this is that the number of times different elements in the support of the cut distribution occur in the sample become 
independent, giving simpler analysis. Moreover, the number of transitions observed along the edge 
$e\in E(t)$, $n_e$, for a fixed $t$ will be distributed as $\Poisson{m\cdot p_e}$, independently for all $e\in E(t)$ (see Lemma~\ref{cl:ind_poisson}). As 
$\Poisson{m}$ is tightly concentrated around $m$, this additional flexibility comes only at a sub-constant cost in 
the sample complexity with an inversely exponential in $m$, additive increase in the error probability. We note that 
as in equations $(1-2)$ from~\cite{AcharyaDK15} the expectation and variance of our $\chi^2$ statistic are as follows.
\[
\Ex{Z_e}=m\cdot\frac{(p_e-q_e)^2}{q_e} 
\quad\text{and}\quad 
\Var{Z_e}=2\frac{p_e^2}{q_e^2}+m\cdot\frac{p_e(p_e-q_e)^2}{q_e^2}.
\]

\begin{lemma}
	\label{cl:ind_poisson}
	The number of transitions $n_e$ along an edge $e$ is distributed as $\Poisson{m\cdot p_e}$ and all $n_e$ are independent for $e\in E(t)$, for any
	$t\in[n]$.
\end{lemma}
\begin{proof}
	The proof proceeds by induction on $t$ and is based on the following two standard observations on Poisson random variables:
	
	\textit{(Observation I)} for any discrete distribution $\distr$, $k\sim\Poisson{\lambda}$ i.i.d. samples from
	$\distr$ form a collection of jointly independent Poisson random variables for the occurrences of each element in 
	the support of $\distr$, i.e., distribution $\prod_i\Poisson{\lambda\cdot\Prx[x\sim\distr]{x=i}}$;
	
	\textit{(Observation II)} the sum of two independent Poisson random variables with distributions $\Poisson{\lambda_1}$ and $\Poisson{\lambda_2}$
	is a Poisson random variable with the distribution $\Poisson{\lambda_1+\lambda_2}$.
	
	For $t=1$ as we start with $\Poisson{m}$ samples,  Observation I gives us the desired result. For the induction step (from $t=k$ to $t=k+1$), we observe that counts of visits to each particular state $i$ at time $t$ are independent Poisson random variables by Observation II. Now, Observation I 
	applied to the states at time $t$ yields the desired result.
\end{proof}

The following procedure correctly distinguishes between the case $P=Q$, or $\dist{P}{Q}\ge\eps$, in the regime when $q_e\ge\Omega(\frac{\eps^2}{n^2})$ 
for all $e\in E(Q)$ and $p_e=0$ for all $e\notin E$.

\begin{algorithm}[H]
	\caption{$\chi^2$ Edge Test}
	\label{alg:chi_sq_edges}
	\KwIn{$\eps$; an explicit $k$-sparse Markov Chain $Q=\MCseqQ$; (Poisson) $m$ samples from a Markov Chain $P=\MCseqP$, where $n_e$ 
		denotes the number of transitions along the edge $e$.}
	\KwOut{Accept if $P=Q$, or reject if $\dist{P}{Q}\ge\eps$}
	\BlankLine
	$E\leftarrow\{e: q_e> 0\}$\;  
	$Z\leftarrow\sum\limits_{e\in E} \frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$\; 
	%\eIf{$Z\le\frac{\eps\cdot m}{4}$}
	\eIf{$Z\le 2\sqrt{k}n^{3/2}$}
	{
		\KwRet \textsc{Accept}\;  
	}
	{
		\KwRet \textsc{Reject}\;  
	}
\end{algorithm}

\begin{theorem} 
	Algorithm~\ref{alg:chi_sq_edges} is correct with probability at least $4/5$, if $m\ge\frac{C n^{3/2}}{\eps^2}$ for some $C=O(1)$, 
	$q_e\ge\frac{\eps^2}{kn^2}$ for all $e\in E$, and $p_e=0$ for all $e\notin E$.
	\label{th:sparse_ub}
\end{theorem}
\begin{proof} To get the desired result we analyze expectation and variance of $Z$. First, we relate the expected value of $Z$ with the distance $\dist{P}{Q}$ between $P$ and $Q$.
	
	\begin{lemma}
		\label{cl:expectation_dist}
		%%$\Ex{Z}\ge m\cdot\hellingersq{P}{Q}.$
		$\Ex{Z}\ge \frac{m}{4}\cdot\distsq{P}{Q}.$
	\end{lemma}
	\begin{proof}
		We recall that 
		\begin{multline}
		\label{eq:dist_P_Q_sum}
		\hellingersq{P}{Q}  =1-\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev\\
		= \oneet\circ\left(\frac{P_1+Q_1}{2}\right)\circ\cdots\circ\left(\frac{P_n+Q_n}{2}\right)\circ\onev-
		\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\srprod{P_n}{Q_n}\circ\onev\\
		=\sum_{t=1}^{n} \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\left(\frac{P_t+Q_t}{2}-\srprod{P_t}{Q_t}\right)\circ\left(\frac{P_{t+1}+Q_{t+1}}{2}\right)\cdots
		\left(\frac{P_{n}+Q_{n}}{2}\right)\circ\onev\\
		=\frac{1}{2}\sum_{t=1}^{n} \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_{t-1}}{Q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev,
		\end{multline}
		where in the last line $\sqsrprod{P_t}{Q_t}=\left(\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2\right)_{ij}$. Indeed, the first equality holds true as
		$P_t\circ\onev=Q_t\circ\onev=\onev$ for any $t\in[n]$; the second equality is a telescopic sum; the last equality is simply the formula for the complete square. 
		Let $q_t$ and $p_t$ be the respective distribution vectors over the states $s_{i,t}$, $i\in[n]$ in $Q$ and $P$ Markov chains. We also define distributions $p_0=q_0=\onee$.
		
		By applying Cauchy-Schwarz inequality to the corresponding Bhattacharya coefficient of $P$ and $Q$ at a fixed state $i$ and time $t$  
		we obtain
		\begin{align*}
		\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_{t}}{Q_{t}}\circ\onevi=
		HS_i\left(\word{P}{t},\word{Q}{t}\right)  = \sum_{\substack{w=s_0\ldots s_t \\ \text{s.t. } s_t=i}}  \sqrt{\Prl[P]{w}\Prl[Q]{w}}\\
		\le\sqrt{\sum_{\substack{w=s_1\ldots s_t \\ \text{s.t. } s_t=i}}  \Prl[P]{w}\sum_{\substack{w=s_1\ldots s_t \\ \text{s.t. } s_t=i}}\Prl[Q]{w}} 
		=\sqrt{p_t(i)\cdot q_t(i)}.
		\end{align*}
		We plug in this estimate to \eqref{eq:dist_P_Q_sum} and obtain
		\[
		\frac{1}{4}\cdot\distsq{P}{Q}=\frac{1}{4}\dtvsq{P}{Q}\le \hellingersq{P}{Q}  \le \frac{1}{2}\sum_{t=1}^{n} \srprodt{p_{t-1}}{q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev,
		\]
		%where $p_{-1}=q_{-1}$ is a probability distribution with one element in the support and $P_0$ and $Q_0$ are the $1\times n$ matrices corresponding to $p_0$ and $q_0$ vectors. 
		We examine each term of the summation in the right hand side of the last equation
		\be
		\label{eq:dist_sqrtpq}
		\frac{1}{2}\srprodt{p_{t-1}}{q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev=\sum_{i}\frac{\sqrt{p_{t-1}(i)\cdot q_{t-1}(i)}}{2}\cdot\sum_{j:(ij)\in E(t)}
		\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2,
		\ee
		We show that corresponding terms in $\Ex{Z}=\sum\limits_{i,t}\sum\limits_{e:(ij)\in E(t)}\Ex{Z_e}$ give an upper bound on \eqref{eq:dist_sqrtpq} for each fixed state $i$.
		
		\begin{multline}
		\frac{1}{m}\sum_{e:(ij)\in E(t)}\Ex{Z_e}=\sum_{e:(ij)\in E(t)}\frac{(p_e-q_e)^2}{q_e}=\sum_{j:(ij)\in E(t)}
		\frac{\left(p_{t-1}(i)P_t(ij)-q_{t-1}(i)Q_t(ij)\right)^2}{q_{t-1}(i)Q_t(ij)}\\
		%=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\frac{P_t^2(ij)}{Q_t(ij)}-2p_{t-1}(i)\sum_{j:(ij)\in E(t)}P_t(ij)+q_{t-1}(i)\sum_{j:(ij)\in E(t)}Q_t(ij)\\
		=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\left(\sum_{j:(ij)\in E(t)}\frac{P_t^2(ij)}{Q_t(ij)}\right)-2p_{t-1}(i)+q_{t-1}(i)\\
		%=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\frac{\left(P_t(ij)-Q_t(ij)\right)^2}{Q_t(ij)}+
		%2P_t(ij)-Q_t(ij)\right)-2p_{t-1}(i)+q_{t-1}(i)\\
		=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\frac{\left(P_t(ij)-Q_t(ij)\right)^2}{Q_t(ij)}+
		\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\\
		%= \frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2\left(\frac{\sqrt{P_t(ij)}+\sqrt{Q_t(ij)}}{\sqrt{Q_t(ij)}}\right)^2+
		%\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\\
		\ge \frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2+\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)},
		\label{eq:inequality_sqrtpq}
		\end{multline}
		where the third and forth equalities hold true as $\sum_{j:(ij)\in E(t)}P_t(ij)=\sum_{j:(ij)\in E(t)}Q_t(ij)=1$, and to get the last inequality one can simply use identity 
		$\frac{(a-b)^2}{b}=(\sqrt{a}-\sqrt{b})^2\left(\frac{\sqrt{a}+\sqrt{b}}{\sqrt{b}}\right)^2$. Now, we claim that the expression in RHS of \eqref{eq:inequality_sqrtpq} is 
		at least RHS of \eqref{eq:dist_sqrtpq} for a given $i$, i.e., we need to show that
		\be
		\label{eq:inequality_four_deg_poly}
		\left(\frac{p_{t-1}^2(i)}{q_{t-1}(i)}-\frac{\sqrt{p_{t-1}(i)q_{t-1}(i)}}{2}\right)\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-
		\sqrt{Q_t(ij)}\right)^2+\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\ge 0.
		\ee
		The inequality is obviously true, if $\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\ge\frac{\sqrt{p_{t-1}(i)q_{t-1}(i)}}{2}$.
		Otherwise, without loss of generality, we can substitute the term 
		\[
		\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2
		\] 
		with an upper bound of $2$. Furthermore, by denoting $x=\sqrt{\frac{p_{t-1}(i)}{q_{t-1}(i)}}$ the inequality \eqref{eq:inequality_four_deg_poly} can be rewritten as
		$q_{t-1}(i)\cdot\left(2x^4-x+(x^2-1)^2\right)\ge 0$, and, indeed, one can verify that this fourth degree polynomial is always positive.
	\end{proof}
	
	Now we estimate the variance of random variable $Z$
	
	\begin{lemma}
		$\Ex{Z}\ge \left(\frac{12\sqrt{2k}}{C}+\frac{2\sqrt{2}+\sqrt{k}}{\sqrt{C}}\right)\cdot\sqrt{\Var{Z}}$, when $m\ge \frac{C\cdot n^{3/2}}{\eps^2}$ and $\dist{P}{Q}\ge \eps$.
		\label{cl:var_z}
	\end{lemma}
	\begin{proof}
		We recall that $Z=\sum_{e\in E}Z_e$ and by Lemma~\ref{cl:ind_poisson} all $Z_e$ for a fixed $t$ and $e\in E(t)$ are independent.
		For any random variables $X_1,\dots, X_n$ it is true that 
		\[
		\Var{X_1+\cdots+X_n}\le\left(\sqrt{\Var{X_1}}+\cdots+\sqrt{\Var{X_n}}\right)^2.
		\]
		We use this estimate for $X_t=\sum_{e\in E(t)}Z_e$ to obtain
		\[
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\Var{Z_e}}=\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}+m\cdot\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\]
		We further simplify the above expression by using the fact that $\sqrt{x+y}\le \sqrt{x}+\sqrt{y}$.
		\be
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}}+\sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\label{eq:var_sqrt_ub}
		\ee
		
		On the other hand, by Lemma~\ref{cl:expectation_dist}
		\be
		\label{eq:expectation_def_eps}
		\Ex{Z}\ge \frac{1}{2}\Ex{Z} + \frac{m}{8}\distsq{P}{Q} =  m\cdot\left(\frac{1}{2}\sum_{e\in E}\frac{(p_e-q_e)^2}{q_e}+\frac{\eps^2}{8}\right).
		\ee
		In the following we use \eqref{eq:expectation_def_eps} to give separate upper bounds on each of the two summation terms in the 
		RHS of \eqref{eq:var_sqrt_ub}. 
		
		\paragraph{First term of \eqref{eq:var_sqrt_ub}.} To estimate the first term, we split $E$ into two sets 
		\[
		E_1\eqdef\{e\in E: p_e\le 2q_e\} \quad\text{and}\quad E_2\eqdef\{e\in E: p_e> 2q_e\}
		\]
		We define accordingly the sets $E_1(t)$ and $E_2(t)$ for each $t\in[n]$. Again we have
		\beq
		\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}}\le \sum_{t=1}^n\sqrt{\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}} + \sum_{t=1}^n\sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}}.
		\eeq
		\textbf{Estimate for $\mathbf{E_1}$.} 
		We have $2\frac{p_e^2}{q_e^2}\le 8$ for any edge $e\in E_1$. Therefore, by the sparsity condition $\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}\le 8n\cdot k$, where $k=O(1)$.
		Thus, 
		%\nick{determine $c_1$}
		\be
		\sum_{t=1}^n\sqrt{\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}}\le \sqrt{8k}\cdot n^{3/2}\le \frac{\sqrt{8k}}{C} \cdot m\cdot \eps^2 \le \frac{4\sqrt{8k}}{C}\cdot\Ex{Z} 
		\label{eq:e1}
		\ee
		\textbf{Estimate for $\mathbf{E_2}$.} We have $\frac{(p_e-q_e)^2}{q_e}\ge \frac{p_e^2}{4q_e}$ for any $e\in E_2$. Therefore,
		%\nick{$c_2\cdot m\frac{\eps^2}{4n^{3/2}}=1$}
		\begin{multline}
		\frac{\sqrt{32k}}{C}\cdot\Ex{Z}\ge \frac{\sqrt{32k}m}{C}\cdot\sum_{t=1}^n\left(\frac{1}{16}\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e}+\frac{\eps^2}{8n}\right)
		\ge \frac{\sqrt{32k}m}{C}\sqrt{\frac{4\eps^2}{16\cdot 8n}}\sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e}}\\
		\ge \frac{\sqrt{32k}m}{C}\sqrt{\frac{\eps^2}{32n}}\cdot\sqrt{\frac{\eps^2}{kn^2}}\sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}}
		\ge \sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}},
		\label{eq:e2}
		\end{multline}
		where the first inequality holds by \eqref{eq:expectation_def_eps}; the second inequality is simply AM-GM inequality; and to get the third
		inequality we used the bound $q_e\ge\frac{\eps^2}{kn^2}$.
		
		\paragraph{Second term  of \eqref{eq:var_sqrt_ub}.} We split $E$ into another two sets $E_3,E_4$ (similarly define $E_3(t)$ and $E_4(t)$): 
		\[
		E_3\eqdef\{e\in E: p_e\le 2\sqrt{n}q_e\} \quad\text{and}\quad E_4\eqdef\{e\in E: p_e> 2\sqrt{n}q_e\}
		\]
		\[
		\text{Again}\quad \sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}+
		\sum_{t=1}^n\sqrt{\sum_{e\in E_4(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\]
		\textbf{Estimate for $\mathbf{E_3}$.} We have 
		\begin{multline}
		2\sqrt{\frac{2}{C}}\cdot\Ex{Z}\ge \sqrt{\frac{2}{C}}m\cdot\sum_{t=1}^n\left(\sum_{e\in E_3(t)}\frac{(p_e-q_e)^2}{q_e}+\frac{\eps^2}{4n}\right)\ge
		\sqrt{\frac{2}{C}}m\sqrt{\frac{\eps^2}{n}}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{(p_e-q_e)^2}{q_e}}\\
		\ge m\sqrt{\frac{2\eps^2}{Cn}}\cdot \sqrt{\frac{1}{2n^{1/2}}}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		= \sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}},
		\label{eq:e3}
		\end{multline}
		where the first inequality holds by \eqref{eq:expectation_def_eps}, the second inequality is AM-GM inequality, to get the third inequality
		we use definition of $E_3$ that $\frac{p_e}{q_e}\le 2\sqrt{n}$.\newline
		\textbf{Estimate for $\mathbf{E_4}$.} We have $p_e-q_e\ge \left(1-\frac{1}{2\sqrt{n}}\right)p_e$ for any $e\in E_4$. Therefore,
		\begin{multline}
		\frac{\sqrt{k}}{\sqrt{2C}\left(1-\frac{1}{2\sqrt{n}}\right)}\cdot\Ex{Z}\ge \frac{m\sqrt{k}}{\sqrt{2C}}\sum_{e\in E_4}\frac{p_e(p_e-q_e)}{q_e}\ge
		\sqrt{m}\sqrt{\frac{km\cdot2\eps^2 }{2C\cdot kn^{3/2}}}\sum_{e\in E_4}\frac{p_e^{1/2}(p_e-q_e)}{q_e}\\
		\ge\sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E_4(t)}\frac{p_e^{1/2}(p_e-q_e)}{q_e}},
		\label{eq:e4}
		\end{multline}
		where the first inequality follows from\eqref{eq:expectation_def_eps}, to get the second inequality we estimate $\sqrt{p_e}\ge \sqrt{2n^{1/2}q_e}\ge\sqrt{\frac{2\eps^2}{kn^{3/2}}},$
		to get the last inequality we simply use that $\sqrt{x}+\sqrt{y}\ge\sqrt{x+y}$. 
		
		Finally, combining estimates \eqref{eq:e1},\eqref{eq:e2},\eqref{eq:e3},\eqref{eq:e4} we obtain the desired bound on the variance.
	\end{proof}
	
	\begin{lemma}
		If $P=Q$, then $\Var{Z}\le\sqrt{k}n^{3/2}$.
		\label{cl:var_z_easy}
	\end{lemma}
	\begin{proof}
		Using similar estimate as in the proof of Lemma~\ref{cl:var_z} we get
		\[
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\Var{Z_e}}=\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{q_e^2}{q_e^2}}\le n\cdot\sqrt{kn}.
		\]
	\end{proof}
	
	To conclude the proof of Theorem~\ref{th:sparse_ub} it remains to notice that in case $P=Q$ the error probability (Algorithm~\ref{alg:chi_sq_edges} returns ``reject'') is at most
	\[
	\Prx{Z> 2\sqrt{k}n^{3/2}}\le\Prx{Z> 2\sqrt{\Var{Z}}}\le \frac{1}{5},
	\]
	where the first inequality follows from Lemma~\ref{cl:var_z_easy}, the last is Cantelli's inequality, since $\Ex{Z}=0$.
	On the other hand, when $\dist{P}{Q}\ge \eps$, then $\Ex{Z}\ge m\cdot\frac{\eps^2}{4}$. If Algorithm~\ref{alg:chi_sq_edges} makes an error by returning ``accept'', 
	then $Z\le 2\sqrt{k}n^{3/2}\le \frac{2\sqrt{k}}{C}\Ex{Z}$. Thus $Z-\Ex{Z}\le (\frac{2\sqrt{k}}{C}-1)\Ex{Z}$. Now if $C$ is such that
	$1-\frac{2\sqrt{k}}{C}\ge 2\cdot\left(\frac{12\sqrt{2k}}{C}+\frac{2\sqrt{2}+\sqrt{k}}{\sqrt{C}}\right)$ (any constant 
	$C\ge\max\left(\sqrt{k}(42\sqrt{2}+4),(8\sqrt{2}+4\sqrt{k})^2\right)$ would work), then $Z-\Ex{Z}\le -2\sqrt{\Var{Z}}$ by Lemma~\ref{cl:var_z}. Furthermore,
	by Cantelli's inequality 
	\[
	\Prx{Z\le 2\sqrt{k}n^{3/2}}\le \Prx{Z-\Ex{Z}\le -2\sqrt{\Var{Z}}}\le \frac{1}{5},
	\]
	i.e., probability of Algorithm~\ref{alg:chi_sq_edges}'s error in the case $P\neq Q$ is at most $\frac{1}{5}$.  
\end{proof}


\paragraph{Analysis of pruning step.} Here we slightly modify Markov Chains $Q$ and $P$ so that the probability of traversing any edge in $Q$ is $\Omega(\frac{\eps^2}{n^2})$ and that 
$P$ only uses these edges. To this end, we sequentially remove edges from $Q$ that have too low probability of traversal in $Q$. Effectively, in the pruning process we are sampling from $Q$, but rejecting all the 
samples that use a ``rare'' edge. We choose the threshold for the ``rare'' edges in such a way that we would reject at most $\eps^2$ fraction of samples from $Q$. Recall that the Markov chain obtained by pruning $Q$ is denoted as $Q^*$.
After pruning of $Q$, we do the corresponding empirical rejection sampling for $P$ (see Algorithm~\ref{alg:pruning}) which is equivalent to obtaining samples from the modified Markov chain $P^*$. If there are too many rejected samples, 
we conclude that $\dist{P}{P^*}>\dist{Q}{Q^*}$ with high probability, and thus $P\neq Q$. Otherwise we proceed to Algorithm~\ref{alg:chi_sq_edges} for the modified $Q$ and pruned samples 
from $P$. 

\begin{algorithm}%[H]
	\caption{Pruning Test. In the pruned Markov Chain $Q^*$ all edges with $q_e>0$ satisfy $q_e\ge\frac{\eps^2}{kn^2};$ samples from Markov Chain $P^*$ can only go along these edges.}
	\label{alg:pruning}
	\SetKwData{Recompute}{Recompute}\SetKwData{Samples}{PrunedSamples}\SetKwData{Count}{RejectCount}
	\SetKwFunction{Delete}{Delete}
	\KwIn{$\eps$; an explicit $k$-sparse Markov Chain $Q=\MCseqQ$; $m$ samples from a Markov Chain $P=\MCseqP$}
	\KwOut{$m\cdot(1-2\eps^2)$ i.i.d. samples from pruned $P^*$ and pruned $Q^*$ s.t., each $q_e=\Omega(\frac{\eps^2}{n^2})$; reject $P$ if there are not enough samples.}
	\BlankLine
	Let $E^*=\{e: q_e>0\}$\;
	\While{$\exists~e\in E^*:q_{e}<\frac{\eps^2}{k\cdot n^2}$}{
		$E^*\leftarrow E^*\setminus e$\tcc*{$e=(ij)$, $e\in E(t)$}
		\Delete($e,Q$)\tcc*{set $Q_t(ij)=0$, re-normalize row $i$ in $Q_t$}
		\lForEach{edge $e\in E^*$}{\Recompute{$q_e$}}
	}
	\For{$w=s_1\cdots s_n \sim P$}{
		\lIf{$\forall~t~ (s_ts_{t+1})\in E^*$}{Add $w$ to \Samples}
		\lElse{increase \Count}
	}
	\eIf{\Count$>2m\eps^2$}
	{
		\KwRet \textsc{Reject}\;  
	}
	{
		\KwRet \Samples\;  
	}
\end{algorithm}


Let $Q^*$ be a modified Markov Chain $Q$ that sample $w\sim Q$ and reject any $w$ with $e\notin E^*$.
\begin{lemma}
	$\dist{Q}{Q^*}\le 2\eps^2$
	\label{cl:rejection_Q}
\end{lemma}   
\begin{proof}
	By definition of the set of pruned edges $E^*$, by removing each new edge we lose at most $\frac{\eps^2}{kn^2}$ fraction of samples.
	As there are only at most $kn^2$ edges in $Q$, the probability of avoiding removed edges is at least
	$(1-\frac{\eps^2}{kn^2})^{kn^2}\ge 1-\eps^2$. Thus at most $\eps^2$ fraction of words $\word{Q}{n}$ are rejected in $\word{Q^*}{n}$, which implies that
	$2\eps^2\le\dtv{\word{Q}{n}}{\word{Q^*}{n}}=\dist{Q}{Q^*}$.
\end{proof}

We need to argue about probability of error in Algorithm~\ref{alg:pruning}. First, in the case $P=Q$ Algorithm~\ref{alg:pruning} could incorrectly return ``reject''.
Our next Lemma~\ref{cl:error_prob_pruning} provides the necessary bound. On the other hand, when $P\neq Q$ and  Algorithm~\ref{alg:pruning} does not return ``reject'', we 
want Algorithm~\ref{alg:chi_sq_edges} to be able to distinguish $P^*$ and $Q^*$. To this end, Lemma~\ref{cl:error_prob_pruning} shows that $\dist{P^*}{Q^*}=\Omega(\eps)$ 
with high probability.  


%Therefore, in the case $P=Q$ we have $\dist{P}{P^*}\le 2\eps^2$. In this case we show that Algorithm~\ref{alg:pruning} does not reject $P$
%with high probability. On the other hand, if $P\neq Q$ and Algorithm~\ref{alg:pruning} does not reject $P$, 
%we want to make sure that Algorithm~\ref{alg:chi_sq_edges} will distinguish $P^*$ and $Q^*$. To this end, we need to provide a lower bound on 
%$\dist{P^*}{Q^*}\ge\eps-\dist{P}{P^*}-\dist{Q}{Q^*}$. As $\dist{Q}{Q^*}\le 2\eps^2$, for a lower bound of $\dist{P^*}{Q^*}\ge\frac{\eps}{4}$ 
%it would suffice to show that $\dist{P^*}{P}\le\frac{\eps}{2}$.
\begin{lemma}~
	\label{cl:error_prob_pruning}
	
	(1) If $P=Q$, then Algorithm~\ref{alg:pruning}'s error of rejecting $P$ is at most $0.1$.
	
	(2) If $\dist{P}{Q}\ge \eps$, then either $\dist{P^*}{Q^*}=\Omega(\eps)$, or Algorithm~\ref{alg:pruning} correctly rejects $P$ with probability at least $0.9$.
\end{lemma}
\begin{proof}
	Let $X_\ell$ be Bernoulli random variables for $\ell\in[m]$ denoting ($X_\ell=1$) whether $\ell$-th sample from $P$ was rejected, or accepted to $P^*$ ($X_\ell=0$).  
	Then the number of rejected samples $X=\sum_{\ell=1}^m X_\ell$. Variables $X_\ell$ are i.i.d. Let $x=\Prx{X=1}$.
	
	1. If $P=Q$, then probability of rejecting a sample from $P$ is not more than $\eps^2$, i.e., $x\le \eps^2$. $\Ex{X}=m\cdot x, \Var{X}=m\cdot(x-x^2)$. Then
	\[
	\Prx{X\ge 2m\eps^2}\le\Prx{X\ge \Ex{X}+3\sqrt{\Var{X}}}\le\frac{1}{10},
	\]
	where the first inequality holds because $2m\eps^2> m\cdot \eps^2 + 3\sqrt{m\eps^2}>\Ex{X}+3\sqrt{\Var{X}}$; the second is Cantelli's inequality.
	
	2. We first observe that $\dist{P^*}{Q^*}\ge\eps-\dist{Q}{Q^*}-\dist{P}{P^*}$. We want to argue that if $\dist{P}{P^*}\ge 6\eps^2$, then
	Algorithm~\ref{alg:pruning} rejects $P$ with probability at least $9/10$. Indeed, then probability $x$ of rejecting a sample from $P$ must be at least 
	$\frac{1}{2}\dist{P}{P^*}\ge 3\eps^2$, then $\Ex{X}\ge 3m\eps^2$ and
	\[
	\Prx{X\le 2m\eps^2}\le\Prx{X-\Ex{X}\le -\frac{\Ex{X}}{3}}\le\Prx{X-\Ex{X}\le -3\sqrt{\Var{X}}}\le\frac{1}{10}.
	\]
	Thus we get $\dist{P^*}{Q^*}\ge\eps-\dist{Q}{Q^*}-\dist{P}{P^*}\ge\eps-2\eps^2-6\eps^2\ge\frac{\eps}{2}$ if $\eps$ is small enough constant. 
\end{proof}

\begin{theorem}
	Together, Algorithm~\ref{alg:pruning} and Algorithm~\ref{alg:chi_sq_edges} tell whether $P=Q$, 
	or $P\neq Q$, when $\dist{P}{Q}\ge\eps$,  with probability at least $\frac{2}{3}$ using $O(\frac{n^{3/2}}{\eps^2})$ samples.
	%\label{th:main_shuffling}
\end{theorem}
\begin{proof}
	In case $P=Q$, Algorithm~\ref{alg:pruning} produces $P^*=Q^*$ and $m(1-2\eps^2)$ samples from $P^*$ with probability at least $0.9$.
	Furthermore, Algorithm~\ref{alg:chi_sq_edges} converts these $m(1-2\eps^2)$ samples into Poisson $m'=\Omega(m)$ samples and accepts
	$P=Q$ with $4/5$ probability. Overall, we have $4/5\cdot 0.9>2/3$ probability of correctly accepting $P=Q$.
	
	When $\dist{P}{Q}\ge\eps$, Algorithm~\ref{alg:pruning} either correctly rejects $P^*$, or produces $P^*$ and $Q^*$ s.t. $\dist{P^*}{Q^*}\ge\frac{\eps}{2}$ with probability at least $0.9$. In the latter case Algorithm~\ref{alg:chi_sq_edges} correctly rejects $P^*$ with probability at least $4/5$. Overall, we get the probability of correctly rejecting $P$ to be at least $4/5\cdot 0.9>2/3$.
\end{proof}

==> pre-stoc18-version/symm_lower_bound.tex <==

\label{sec:symm-lower-bound}
In this section we provide nearly matching lower bound to our result in Theorem~\ref{th:symmetric_ub}. 
%will show that any algorithm that tests identity of a symmetric Markov chain requires a word of length $\Omega\left({\frac{n}{\eps}}\right)$ from the Markov chain. 
%where $n$ is the number of states in the Markov chain.
%We will use Le Cam's two point method to show our lower bound.
\begin{theorem}
\label{thm:symm-lower-bound}
There is an instance of Identity testing problem for symmetric Markov chain $Q$ that requires
a word of length at least $\Omega(\frac{n}{\eps})$ to check identity of $Q$ with $99$\% confidence.
%There is an instance of the identity testing problem for symmetric Markov chain $Q$ on $n$ states 
%that requires a word of length at least $\Omega(\frac{n}{\eps})$ from $P$ to distinguish between cases 
%$P=Q$ vs. $1-\specr{\srprod{P}{Q}} \ge \eps$  with probability at least $\frac{99}{100}$, for $\eps=\omega(n^{-1/3})$.
%
%There exists a constant $c>0$,such that any algorithm which is given the description of a symmetric Markov chain $Q$ and 
%sample access to words from a symmetric Markov chain $P$ on $n$ states, and distinguishes between the cases $P \equiv Q$ 
%and $1-\specr{\srprod{P}{Q}} \ge \eps$ with probability at least $99/100$ requires at least $k \geq \frac{cn}{\eps}$ samples.
\end{theorem}
\begin{proof}%[Proof outline]
%We will assume $n$ is such that $n > 1/\eps$ for the following lower bound construction. This assumption is a fair one 
%to make as we are interested in the regime where $\eps$ is a constant and $n$ grows large. \nishanth{word this better}
%The proof of Theorem~\ref{thm:symm-lower-bound} follows via an application of Le Cam's two-point method to word 
%distributions arising from Markov chains. 
We use Le Cam's two point method and construct a class of Markov chains $\mathcal{P}$ s.t.  
(i) every $P \in \mathcal{P}$ is at least $\eps$ far from $Q$ for a given constant $\eps$. That is $1-\specr{\srprod{P}{Q}} \geq \eps$ for any $P \in \mathcal{P}$;
(ii) there is a constant $c > 0$, s.t. it is impossible to distinguish a word of length $m$ generated by a randomly chosen 
Markov chain $\bar{P} \sim \mathcal{P}$, from a word of length $m$ produced by $Q$ with probability equal to or greater than $\frac{99}{100}$ for $m\le\frac{cn}{\eps}$.
To prove (ii) we show that the total variation distance between the $m$-word distributions obtained from the two processes, $Q$ and $\bar{P}$, is small when $m<\frac{cn}{\eps}$ for 
some constant $c$. We denote distribution of length $m$ words obtained from $Q$ by $\word{Q}{m}$, and from MC $\bar{P}\sim\mathcal{P}$ by $\word{\mathcal{P}}{m}$. 
%\begin{itemize}
%\item The word distribution of words of length $t$ obtained from $Q$ (represented by $\word{Q}{t}$).
%\item The word distribution of words of length $t$ obtained from a Markov chain $\bar{P}$ chosen uniformly at random from the family $\mathcal{P}$ (represented by $\word{\bar{P}}{t}$).
%\end{itemize}
We represent symmetric MC as undirected weighted graphs $G=(V,E)$. 
We allow graph to have multi-edges (this is helpful to provide an intuitive understanding of the lower bound construction and is not 
essential). We can ultimately remove all multi-edges and give a construction with only simple edges by 
doubling the number of states.

\begin{description}
\item[Markov Chain $Q$:] complete double graph on $n$ vertices with uniform weights, i.e., 
\[
\forall \quad i\neq j \quad\quad (ij)_1, (ij)_2\in E  \quad\quad  Q_{(ij)_1}=Q_{(ij)_2}=\frac{1}{2(n-1)}.
%Q_{(ij)_1}=\frac{1}{2(n-1)} \quad\quad Q_{(ij)_2}=\frac{1}{2(n-1)}\quad\quad \text{ for any } i\neq j.
\]
\item[Family $\mathcal{P}$:] for any pair of vertices $i\neq j$ there are two bidirectional edges $(ij)_1$, $(ij)_2$
with weights randomly (and independently for each pair of $(i,j)$) chosen to be either
\[
P_{(ij)_1}, P_{(ij)_2}=\frac{1\pm \sqrt{8\eps}}{2(n-1)},
\quad\quad\text{ or }\quad\quad
P_{(ij)_1},P_{(ij)_2}=\frac{1\mp \sqrt{8\eps}}{2(n-1)}.
\]
%\[
%\begin{cases}
%P_{(ij)_1}&=\frac{1+4\sqrt{\eps}}{2n-2}, \\
%P_{(ij)_2}&=\frac{1-4\sqrt{\eps}}{2n-2}
%\end{cases}
%\text{ or }
%\begin{cases}
%P_{(ij)_1}&=\frac{1-4\sqrt{\eps}}{2n-2}, \\
%P_{(ij)_2}&=\frac{1+4\sqrt{\eps}}{2n-2}
%\end{cases}  
%\]
%
%
%for every state $i$, bidirectional transition probabilities to states $j$ and $j'$, for each $j > i$, 
%are randomly chosen to be either $\frac{1+4\sqrt{\eps}}{2n-2},\frac{1-4\sqrt{\eps}}{2n-2}$ or 
%$\frac{1-4\sqrt{\eps}}{2n-2},\frac{1+4\sqrt{\eps}}{2n-2}$ respectively. The family consists of every 
%Markov chain which can be generated by this process.
%for every state $i$, bidirectional transition probabilities to states $j$ and $j'$, for each $j > i$, 
%are randomly chosen to be either $\frac{1+4\sqrt{\eps}}{2n-2},\frac{1-4\sqrt{\eps}}{2n-2}$ or 
%$\frac{1-4\sqrt{\eps}}{2n-2},\frac{1+4\sqrt{\eps}}{2n-2}$ respectively. The family consists of every 
%Markov chain which can be generated by this process.
\end{description}
To make this instance a simple graph with at most one bidirectional edge between any pair of vertices we apply 
a standard graph theoretic transformation: we make a copy $i'$ for each vertex $i$; for each pair of double edges 
$e_1=(ij)_1, e_2=(ij)_2$ construct $4$ edges $(ij),(ij'),(i'j),(i'j')$ with weights $w(ij)=w(i'j')=w(e_1)$ and $w(ij')=w(i'j)=w(e_2)$. 
%See Appendix~\ref{app:sec_symm_lb} for complete proof.
%We complete the rest of the proof in Section \ref{app:sec_symm_lb}.
%We apply standard graph theoretic transformation to make this instance a simple graph with one bidirectional edge
%between any pair of vertices. To this end we make a copy $i'$ for each vertex $i$ and for each pair of double edges 
%$e_1=(ij)_1, e_2=(ij)_2$ construct $4$ edges $(ij),(ij'),(i'j),(i'j')$ with weights $w(ij)=w(i'j')=w(e_1)$ and $w(ij')=w(i'j)=w(e_2)$.
%In fact, we will ultimately remove this assumption and give a construction with only simple edges by 
%increasing the number of states by a factor of 2. \nishanth{intuition about construction goes here}
%All Markov chains in our lower bound construction will have the same set $S$ of states and $|S| = 2n$. Hence each 
%transition matrix is a $2n \times 2n$ square matrix whose row $i$ contains the transition probabilities from state 
%$i$ to the other states.

As all Markov chains $Q$ and $P\in\mathcal{P}$ are symmetric with respect to the starting state, we can assume without loss of generality that word $w$ starts from
the state $i=1$. First, we observe that for the simple graph $2n$-state representation  
\begin{lemma}
	\label{clm:p-far-from-q}
	Every Markov chain $P \in \mathcal{P}$ is at least $\eps$-far from $Q$.
\end{lemma}
\begin{proof}
	For any $P \in \mathcal{P}$, it can be seen that 
	$$\srprod{P}{Q}\circ \onev = \left(\frac{\sqrt{1+\sqrt{8\eps}}+\sqrt{1-\sqrt{8\eps}}}{2}\right)\cdot\onev.$$
	By Perron-Frobenius theorem $\onev$ is the unique eigenvector corresponding to the largest absolute value eigenvalue.  
	%and since all its entries are non-negative, by Perron-Frobenius theorem for non-negative matrices, we get that $\onev$ is the 
	%eigenvector corresponding to the eigenvalue with the largest absolute value. 
	Hence, $\specr{\srprod{P}{Q}} = \frac{\sqrt{1+\sqrt{8\eps}}+\sqrt{1-\sqrt{8\eps}}}{2}$ which by Taylor series expansion implies $1-\specr{\srprod{P}{Q}}\ge\eps+\frac{5}{2}\eps^2+o(\eps^2)
	\ge \eps$ for any $\eps<\frac{1}{8}$.
	%\begin{align}
	%1-\rho\left(\srprod{P}{Q} \right) &= 1-\frac{\sqrt{1+4\sqrt{\eps}}+\sqrt{1-4\sqrt{\eps}}}{2} \notag\\
	%&\geq 1-\left(\frac{1+\frac{4\sqrt{\eps}}{2}-\frac{16\eps}{8}+\frac{64\eps^{1.5}}{16}+1-\frac{4\sqrt{\eps}}{2}-\frac{16\eps}{8}+\frac{64\eps^{1.5}}{16}}{2}\right) \label{eq:bytaylor}\\
	%&\geq 2\eps - 4\eps^{1.5} \notag\\
	%&\geq \eps \label{eq:eps-small}
	%\end{align}
	%where (\ref{eq:bytaylor}) follows from Taylor's inequality and (\ref{eq:eps-small}) follows for small enough $\eps$\nishanth{technically inaccurate}.
\end{proof}

%\nishanth{Collision definition changes now due to duplication of states.}
We say that a given word $w=s_1\ldots s_m$ from a Markov chain $P$ represented as a multi-edge graph on $n$ states has a $(ij)$ {\em collision}, 
if any state transition between states $i$ and $j$ (in any direction along any of the edges $(ij)_1,(ij)_2$) occurs more than once in $w$. We now 
state and prove the following claims about the Markov chain family $\mathcal{P}$.


\begin{lemma}
	\label{clm:num-collisions}
	Consider a word $w$ of length $m$ drawn from $Q$. The expected number of collisions in $w$ is
	at most $\Ocomplex{\frac{m^2}{n^2}}=\Ocomplex{\frac{1}{\eps^2}}$. 
	%and the probability of $w$ having a collision is $\leq \frac{t^2}{2(n-1)^2}$.
\end{lemma}
\begin{prevproof}{Lemma}{clm:num-collisions}
	Let $I_w(t_1,t_2,(ij))$ indicate the event that in the multi-edge interpretation of the Markov chain $P$, the transition along $(ij)$ edge occurs at times $t_1<t_2$  in $w$. 
	%That is, $I_w(t_1,t_2,i \rightarrow j) = 1$ if $s_{t_1} = i, s_{t_1+1} = j$ and $s_{t_2} = i, s_{t_2+1} = j$. $I_w(t_1,t_2,i \rightarrow j) = 0$ otherwise. 
	First, we observe that $\Prx{s_{t_1}=s | s_{t_1-1}=x} \leq \frac{1}{n-1}$ and $\Prx{s_{t_2}=s | s_{t_1-1}=x} \leq \frac{1}{n-1}$ for all $x$ and both $s=i$ or $s=j$.
	Thus for any $t_2\ge t_1+2$ by a union bound for all four possible cases of $s_{t_1},s_{t_1+1},s_{t_2},s_{t_2+1}\in\{i,j\}$ we have 
	$$\E\left[I_w(t_1,t_2,(ij)) \right] \leq \frac{4}{(n-1)^4}.$$
	Similarly, for the case $t_2=t_1+1$ we can obtain 
	$$\E\left[I_w(t_1,t_2,(ij)) \right] \leq \frac{2}{(n-1)^3}.$$
	%$$\Prx{s_{t_1}=i} \leq \frac{1}{n-1}$$
	%when considering the worst possible distribution of state $s_1$. This is because $\Prx{s_{t_1}=s | s_{t_1-1}=x} \leq 1/(n-1)$ for all $x$. 
	%Similarly $\Prx{s_{t_2} = i} \leq \frac{1}{n-1}$. Since $\Prx{s_{t_1+1}=j | s_{t_1}=i} = \frac{1}{n-1}$,
	%$$\E\left[I_w(t_1,t_2,i \rightarrow j) \right] \leq \frac{1}{(n-1)^4}.$$
	Let $X$ denote the random variable which is equal to the total number of collisions in the word $w$. Then,
	\begin{align*}
	\Ex{X} &= \sum_{t_2 \ge t_1+2}\sum_{i\neq j} \Ex{I_w(t_1,t_2,(ij))} + \sum_{t_1=1}^{m-1}\sum_{i\neq j} \Ex{I_w(t_1,t_1+1,(ij))}\\
	& \le \frac{4}{(n-1)^4}\cdot\frac{m^2}{2}\cdot\frac{n(n-1)}{2}+ \frac{2}{(n-1)^3}\cdot m\cdot\frac{n(n-1)}{2}
	=\Ocomplex{\frac{m^2}{n^2}}
	\end{align*}
	%\begin{align*}
	%X &= \sum_{t_1 \neq t_2}\sum_{i,j} I_w(t_1,t_2,i \rightarrow j) \\
	%\implies \E[X] &= \sum_{t_1 \neq t_2}\sum_{i,j} \E\left[ I_w(t_1,t_2,i \rightarrow j) \right] \\
	%\implies \E[X] &\leq \frac{1}{(n-1)^4}\frac{t^2}{2}n^2 \\
	%&= \frac{t^2}{2(n-1)^2}
	%\end{align*}
	%Applying Markov's inequality on $X$ gives us that,
	%$$\Prx{ X > 0} = \Prx{X \geq 1} \leq \frac{t^2}{2(n-1)^2}.$$
\end{prevproof}

We also consider 3-way collisions which are collisions where there was at least 3 different transition between a pair of states $i$ and $j$ in the word $w$. 

\begin{lemma}
	\label{cl:3way-collisions}
	Consider a word $w$ of length $m$ drawn from $Q$. The probability of $w$ having a $3$-way collision is at most $O(\frac{m^3}{n^4})=o(1).$
\end{lemma}
\begin{prevproof}{Lemma}{cl:3way-collisions}
	Similar to the proof of Lemma~\ref{clm:num-collisions} we can give a sharp upper bound on the expected number of $3$-way collisions with the most significant term
	being $\frac{8m^3}{6 (n-1)^6}\cdot\frac{n(n-1)}{2}$, i.e., the expected number of $3$-way collisions is $\Ocomplex{\frac{m^3}{n^4}}$. By Markov inequality we  
	obtain the required bound on the probability of a $3$-way collision.   
\end{prevproof}

Now consider a typical word $w$ generated by $Q$. 
%$\bar{P}\sim\mathcal{P}$. 
As we know from Lemma~\ref{cl:3way-collisions} it has no 3-way collisions and by Markov inequality
and Lemma~\ref{clm:num-collisions} has at most $O(\frac{1}{\eps^2})$ collisions with high probability. As we show next a typical word $w$ has similar probabilities under $Q$ or 
$\bar{P}\sim\mathcal{P}$ models.

\begin{lemma}
	\label{clm:no-collision-analysis}
	For $m=O(\frac{n}{\eps})$ at least $\frac{1}{2}$ fraction of words $w=s_1\cdots s_m$ generated by $Q$ satisfy 
	\[
	\frac{1}{2}\cdot\prob[Q]{w}<\prob[\bar{P}\sim \mathcal{P}]{w} < 2\cdot \prob[Q]{w}
	\]
\end{lemma}
\begin{prevproof}{Lemma}{clm:no-collision-analysis}
	For each feasible word $w$ in $Q$, i.e., $w$ such that $\prob[Q]{w}>0$
	\[
	\Prlong[Q]{w}=\left(\frac{1}{2(n-1)}\right)^{m-1}
	\quad\quad 
	\Prlong[\bar{P}\sim\mathcal{P}]{w}=\prod_{j>i}\sum_{\bar{P}_{(ij)_1}=\frac{1\pm\sqrt{8\eps}}{2(n-1)}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|} 
	\]
	
	First, if $w$ has only one transition along edge $(ij)$, then the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{w}$ 
	\[
	\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1}{2}\left(\frac{1+\sqrt{8\eps}}{2(n-1)}+\frac{1-\sqrt{8\eps}}{2(n-1)}\right)=
	\frac{1}{2(n-1)}.
	\]
	From Lemma~\ref{cl:3way-collisions}, we know that probability of a $3$-way collision in $w$ is $o(1)$ under $Q$ model. We observe that for a $2$-way collision $(ij)$
	(a collision which is not a $3$-way collision), the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{w}$  for the case of transition along two different 
	edges $(ij)_1$ and $(ij)_2$ is
	\[
	\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1+\sqrt{8\eps}}{2(n-1)}\cdot\frac{1-\sqrt{8\eps}}{2(n-1)}=
	\frac{(1-8\eps)}{4(n-1)^2}.
	\] 
	We call this type of collision {\em type I} collision. For the other case ({\em type II} collisions) of transition along the same edges the respective probability is 
	$\frac{(1+8\eps)}{4(n-1)^2}$. By Lemma~\ref{clm:num-collisions} and by Markov inequality the total number of collisions is $O(\frac{1}{\eps^2})$ with probability $\frac{3}{4}$. 
	We can also make sure that out of these collisions number of type I and type II collisions is roughly the same. More precisely, the difference between numbers of 
	type I and type II collisions is at most $O(\frac{1}{\eps})$ with probability of at least $\frac{3}{4}$. Indeed, the choice of edge collision type in $w$ is uniform between type I and type II, and is
	independent across all collision edges. Now, for small enough $m$ we can make sure that at least $\frac{1}{2}$ fraction of words $w$ has number of collisions at most 
	$\frac{c_1}{\eps^2}$ and the difference between number of type I and II collisions is at most $\frac{c_2}{\eps}$, for some small constants $c_1,c_2>0$. Thus the corresponding density 
	functions can be related as follows.
	\[
	2>\left(1+8\eps\right)^{\frac{c_2}{\eps}}>\frac{\prob[\bar{P}\sim\mathcal{P}]{w}}{\prob[Q]{w}}>\left(1-64\eps^2\right)^{\frac{c_1}{2\eps^2}}\cdot \left(1-8\eps\right)^{\frac{c_2}{\eps}}>1/2
	\]
	%First, we observe that if a word $w$ has no collisions then $\prob[Q]{w} = \prob[\bar{P}]{w}$. From Claim \ref{cl:3way-collisions}, 
	%we know that the probability of a word $w$ of length $m = o(n/\eps)$ having a 3-way collision is $< 1/20$ under either $Q$ or $\bar{P}$ 
	%processes. Therefore, the claim holds true for such words. It remains to show the claim to be true for words with at least one 2-way 
	%collision and at most $1/\eps^2$ 2-way collisions. Since collisions are of two types as explained in the description, each one can be 
	%regarded as a coin toss. If the Markov chain was indeed $Q$, then it would be a fair coin toss between the two collision types. If it 
	%was $\bar{P}$ then each collision would correspond to a coin toss with the bias of the coin as $\pm O(\eps)$. Therefore the maximum 
	%$\frac{\prob[Q]{w}}{\prob[\bar{P}]{w}}$ can be is
	%$$(1+\eps)^{(1/\eps^2)} \leq \exp(1/\eps)$$
	%Consider a word $w$ with no collisions. We have,
	%$$\Prx{w=s_1 \ldots s_t} = \Prx{s_1}\Pr{s_2 | s_1} \ldots \Prx{s_t | s_{t-1}}.$$
	%Under $Q$, $\Prx[Q]{w} = 1/n^{t}$.
	%We will now bound $\Prx[\bar{P}]{w}$. Any transition $s_i \rightarrow s_j$ exists in exactly $(1-\eps)^2$ fraction of the Markov chains in family $\mathcal{P}$. And given any sequence of states with no collisions, they will have TBF
	%$\Prx[\bar{P}]{s_{i+1} |s_i}\leq (1-\eps)^2\frac{1}{n(1-\eps)^2} = \frac{1}{n}$.
	%
	%Therefore,
	%$$\Prx[\bar{P}]{w} \leq \frac{1}{n^{t}} = \Prx[Q]{w}.$$
\end{prevproof}


Lemma~\ref{clm:no-collision-analysis} shows that $\dtv{\word{Q}{m}}{\word{\mathcal{P}}{m}} \leq \frac{3}{4}$, which implies that
no algorithm can successfully distinguish $Q$ from the family $\mathcal{P}$ with probability greater than $\frac{3}{4}$ for some
$m=\Omega(\frac{n}{\eps})$.

%\begin{itemize}
%
%\item \textbf{The Markov Chain $Q$}\\
%We denote the $2n$ states as $1,\ldots,i,\ldots,n,1',\ldots,i',\ldots,n'$. For each state $i$, there is a corresponding state $i'$. Each row in the transition matrix of $Q$ is constructed the same way. In particular, row $i$ of the transition matrix $Q$, has transitions to every state other than $i$ and $i'$ with probability $1/(2n-2)$. Note that $Q$ is symmetric.
%
%\item \textbf{Constructing the family $\mathcal{P}$}\\
%The family $\mathcal{P}$ of Markov chains is constructed as follows: For every state $i$, bidirectional transition probabilities to states $j$ and $j'$, for each $j > i$, are randomly chosen to be either $\frac{1+4\sqrt{\eps}}{2n-2},\frac{1-4\sqrt{\eps}}{2n-2}$ or $\frac{1-4\sqrt{\eps}}{2n-2},\frac{1+4\sqrt{\eps}}{2n-2}$ respectively. The family consists of every Markov chain which can be generated by this process.
%\end{itemize}

\end{proof}


==> pre-stoc18-version/symm_upper_bound.tex <==
As we have formalized a notion of distance between symmetric Markov Chains in the previous section we get 
a well defined framework from property testing literature \cite{BatuFFKRW01,Paninski08,LeviRR13} for testing 
properties of distributions generated by Markov Chains. Arguably, the next fundamental question, 
after deciding one out of two given distributions (we call it {\em $A$-$B$ testing}), is identity testing problem. 
In this problem the goal is to test from a stream of samples whether the real distribution (which
unlike the case of $A$-$B$ testing is completely unknown to us) coincides with a given hypothesis distribution. 
In this section, we present our results for identity testing of symmetric Markov chains. 
We first present a polynomial time algorithm that provides an efficient reduction to the identity testing problem with i.i.d. samples.
The algorithm improves on the performance of a naive reduction, which waits for a period of time to get an independent sample
and as such suffers a multiplicative loss of mixing time $\mixt{Q}$ of Markov Chain $Q$.
Our algorithm suffers only an {\em additive loss} of $\wO{\hitt{Q}\cdot\log\left(\hitt{Q}\right)}$ in sampling complexity and allows us 
to reduce the problem to testing identity with respect to squared Hellinger distance of a distribution supported on a domain of size $n^2$ and with access to i.i.d. samples.
In the next subsection we provide a nearly matching lower bound for the identity testing problem.
%\nishanth{More intro needed?}
%\corrected{In this section, we present our algorithm for testing identity of symmetric Markov chains. The precise problem definition is stated below:}
We begin by giving a formal statement of the identity testing problem below:
%\begin{description}
%\item[Input:] $\eps$; symmetric transition matrix $Q$; stream of $m$ consecutive samples from symmetric Markov Chain $P$.
%\item[Output:] $P=Q$, or $P\neq Q$ if $1-\specr{\srprod{P}{Q}}>\eps$. 
%\end{description}

\begin{algorithm}[H]
\KwIn{$\eps$; explicit symmetric Markov chain $Q$; $m$ consecutive samples $s_1\cdots s_m$ from a symmetric Markov Chain $P$.}
\KwOut{$P=Q$, or $P\neq Q$ if $1-\specr{\srprod{P}{Q}}>\eps$.}
\end{algorithm}
\paragraph{Our approach.} We consider a mapping $\infmap{\vect{k}}$ from infinite words $\word{M}{\infty}$ of an irreducible Markov chain $M$ to $\prod_{i=1}^{n}
[n]^{k_i}$, where $\vect{k}=(k_1,\cdots,k_n)$ is a vector of $n$ non negative integers, as follows. For each infinite word $w=s_1s_2\cdots$ and each state 
$i\in[n]$ we look at the first $k_i$ visits to state $i$ (i.e., at times $t=t_1,\dots,t_{k_i}$ with $s_{t}=i$) and write down the corresponding 
transitions in the infinite word $w$, i.e., $s_{t+1}$. We note that every state is visited almost surely in $w$, since $M$ is an irreducible finite-state Markov chain. 
Therefore, mapping $\infmap{\vect{k}}$ defines a probability distribution on $\prod_{i=1}^{n}[n]^{k_i}$. We note that this distribution is independent across 
all different states and/or independent for a particular state $i$ because of the Markov property of Markov chains. Furthermore, a specific draw for a copy of a state $i$ is distributed 
according to the $i$-th row of the transition matrix $M$.

In Lemma~\ref{lem:large_deviation_bound} we show that for a big enough number of samples $ m=\widetilde{O}\left(\hitt{Q}\log\left(\hitt{Q}\right)\right. \allowbreak +\left. \frac{n}{\eps}\right)$ \footnote{in this paper, $\widetilde{O}$ always hides poly $\log(n/\eps)$ factors.} and 
$k_i=O(\Ex{\text{\# visits to } i})=O(\frac{m}{n})$ the mapping $\infmap{\vect{k}}$ is well defined for a finite $m$ number of samples for all 
but a small fraction of the words in $\word{M}{m}$. This effectively allows us to generate a large number of independent samples from a discrete distribution
corresponding to matrix $P$: pick uniformly at random a state $i\in[n]$ and then observe transition from $i$ according to transition probabilities of $P$.
Indeed, to this end, we first simulate $m'=\Theta\left(\frac{m}{\log^2 (n/\eps)}\right)$ i.i.d. samples from $[n]$. Let 
$\vect{k}$ be the histogram of these $m'$ samples (note that $\max_{i} k_i \le O(m'\log n /n)$ with high probability). 
We apply $\infmap{\vect{k}}$ mapping to our stream of $m$ consecutive samples of Markov chain $P$, which is well defined with high probability. 
Apart from some small probability events ($\max_{i} k_i$ is too large, or $\infmap{\vect{k}}$ is not defined) we obtain the desired $m'$ i.i.d. 
samples. 
%Large deviation bound
\begin{lemma} 
If $m=\wO{\log\left(\hitt{Q}\right)\hitt{Q}}$, then $\Prx{\exists \text{ state }i: |\{t: i=s_t\in w\}|<\frac{m}{8e\cdot n}}\le\frac{\eps^2}{n}.$ 
%If the number of steps $m=\wO{\log\left(\hitt{Q}\right)\hitt{Q}}$, then
%\[
%\Prx{\exists \text{ state }i: |\{t: i=s_t\in w\}|<\frac{m}{8e\cdot n}}\le\frac{\eps^2}{n}.
%\] 
\label{lem:large_deviation_bound}
\end{lemma}
\begin{proof}
	To simplify notations we denote by $\Delta\eqdef 2\hitt{Q}$. By union bound over all states $i$ it is enough to show that $\Prx{|\{t: i=s_t\in w\}|<\frac{m}{8e\cdot n}}\le\frac{\eps^2}{n^2}$ 
	for each fixed state $i$. We can make sure that in the first $\frac{m}{2}$ steps state $i$ is visited at least once with probability 
	at least $1-\frac{\eps^2}{n^3}$. Once we visited state $i$, instead of hitting time for state $i$ we can analyze the {\em return time} $\returnt$ for $i$.
	Note that for symmetric Markov chains $\frac{1}{n}\onev$ (uniform distribution) is a stationary distribution. Therefore, every state appears at average once 
	in every $n$ steps in an infinite word from $\word{Q}{\infty}$. In other terms, the expectation of $\returnt$ for each 
	state $i$ is exactly $n$. By definition of hitting time we have that in $\frac{\Delta}{2}$ steps the probability 
	of reaching a particular state $i$ from any other state $j$ is greater than $1-1/e$ (or any other given constant). It implies that $\Prx{\returnt \ge \frac{\Delta}{2}\cdot C}\le e^{-C}$
	for any $C\in\N$. Indeed, one can show this by induction on parameter $C$. 
	Notice that if the random walk did not return to $i$ after $C-1$ steps it has stopped at some state $j\neq i$. Then for any choice of $j$ by definition of the hitting time 
	the random walk will return to $i$ with probability at least $1/e$ in the next $\frac{\Delta}{2}$ steps. It is not hard to get a similar bound $\Prx{\returnt \ge \Delta\cdot C}\le e^{-C}$ for any $C\ge 1, C\in\R$. To simplify notations we use $X$ to denote the random variable $\returnt$ 
	and $X_1,\dots,X_\ell$ to denote $\ell$ i.i.d. samples of $X$. We have  
	
	\be
	X\ge 0\quad\text{and}\quad\forall C\in\R_{\ge 1},\Prx{X \ge \Delta\cdot C}\le e^{-C} \quad\text{and}\quad \Ex{X}=n.
	\label{eq:ineq_return}
	\ee
	
	We only need to show that $\Prx{X_1+\cdots+X_\ell > m/2} \le \frac{\eps^2}{n^2}$ for $\ell=\frac{m}{8e\cdot n}$.
	To this end, we use a standard technique for large deviations and apply Markov's inequality to the moment generating function of $X_1 + \cdots + X_\ell$,
	
	%\begin{multline*}
	\be
	\Prx{X_1+\cdots+X_\ell > m/2}=\Prx{e^{\theta\cdot(X_1+\cdots+X_\ell)} > e^{\theta\cdot m/2}}\le\frac{\Ex{e^{\theta\cdot(X_1+\cdots+X_\ell)}}}{e^{\theta\cdot m/2}} \\
	=\frac{\Ex{e^{\theta X}}^\ell}{e^{\theta\cdot m/2}}
	\label{eq:MGF_markov}
	\ee
	%\end{multline*}
	We note that given restrictions \eqref{eq:ineq_return} on $X$ maximum of $\Ex{e^{\theta X}}$ for any fixed $\theta>0$ is attained at 
	\[
	X^*\sim
	\begin{cases}
	\Delta\cdot x  & x\in[C_0,\infty) \text{ with probability density function } e^{-x}\\
	0 & \text{with remaining probability }1-e^{-C_0},
	\end{cases}
	\]
	where constant $C_0>1$ is such that $\Ex{X^*}=n$. Indeed, distribution $X^*$ maximizes \eqref{eq:MGF_markov} due to simple variational inequality:
	$\epsilon\cdot e^{\theta\cdot a}+\epsilon\cdot e^{\theta\cdot b}<\epsilon\cdot e^{\theta\cdot (a-c)}+\epsilon\cdot e^{\theta\cdot (b+c)}$ for any $b \ge a \ge c > 0$, and probability mass $\epsilon>0$.
	This inequality allows us to increase $\Ex{e^{\theta\cdot X}}$ and not change $\Ex{X}$ by tweaking density function $f(x)$ of $X$ 
	$f'(a-c)=f(a-c)+\epsilon$, $f'(a)=f(a)-\epsilon$, $f'(b)=f(b)-\epsilon,$ $f'(b+c)=f'(b+c)+\epsilon$, ($f'(x)=f(x)$ for all other $x$), for some $c\le a$. 
	The only time we cannot apply this incremental change is when $X=X^*$.
	
	We have 
	\be
	\label{eq:C0}
	\Ex{X^*}=\Delta(C_0+1)e^{-C_0} = n.
	\ee 
	We set $\theta\eqdef\frac{1}{2\Delta\log\Delta}$ in \eqref{eq:MGF_markov}. Now we are ready to estimate $\Ex{e^{\theta\cdot X}}$.
	To simplify notations we denote $\gamma\eqdef\frac{1}{2\log\Delta}$.
	\begin{multline}
	\Ex{e^{\theta\cdot X}}=1-e^{-C_0}+\int_{C_0}^{\infty}e^{\theta\cdot\Delta\cdot x}\cdot e^{-x}\,\mathrm{d}x=
	1-e^{-C_0}+\int_{C_0}^{\infty}e^{-x\cdot(1-\frac{1}{2\log\Delta})}\,\mathrm{d}x\\
	=1-e^{-C_0}+\frac{e^{-C_0(1-\gamma)}}{1-\gamma}=1+e^{-C_0}\left(\frac{e^{C_0\gamma}}{1-\gamma}-1\right).
	\label{eq:expectation_MGF}
	\end{multline}
	We notice that $\gamma C_0<1$, since from \eqref{eq:C0} we can conclude that $\frac{e^{C_0}}{C_0+1}=\frac{\Delta}{n}\implies C_0<2\log\Delta=1/\gamma$. The last implication can be obtained as follows: for $C_0 > 2.52,$ we have $C_0 - \frac{C_0}{2}\le C_0-\ln(1+C_0)=\ln(\frac{\Delta}{n})$. Now, we can estimate $e^{\gamma C_0}\le 1 + e\cdot\gamma C_0$ in \eqref{eq:expectation_MGF}. Furthermore, since $\gamma<1/2$ we have
	the term $\frac{e^{C_0\gamma}}{1-\gamma}-1$ in \eqref{eq:expectation_MGF} to be at most $2e\gamma(C_0+1)$. With this estimate we continue \eqref{eq:expectation_MGF}
	\be
	\Ex{e^{\theta\cdot X}}\le 1+e^{-C_0}2e\gamma(C_0+1)=1+\frac{e\cdot n}{\Delta\log\Delta}.
	\label{eq:expectation_MGF2}
	\ee
	We apply estimate~\eqref{eq:expectation_MGF2} and formula $\theta=\frac{1}{2\Delta\log\Delta}$ to~\eqref{eq:MGF_markov} to obtain
	\[
	\Prx{X_1+\cdots+X_\ell > m/2}\le \frac{\left(1+\frac{e\cdot n}{\Delta\log\Delta}\right)^\ell}{e^{m/4\Delta\log\Delta}}
	\le\frac{e^{m/8\Delta\log\Delta}}{e^{m/4\Delta\log\Delta}}=e^{\frac{-m}{8\Delta\log\Delta}}<\frac{\eps^2}{n^2},
	\]
	where in the second inequality we used the fact $\left(1+\frac{e\cdot n}{\Delta\log\Delta}\right)^{\frac{\Delta\log\Delta}{e\cdot n}}<e$, and to get the last inequality
	we used $m=\wOm{\Delta\log\Delta}$ (where in $\widetilde{\Omega}$ the hidden dependency is only on  $\log \eps$ and $\log n$).
\end{proof}




\begin{algorithm}[H]
\caption{Independent Edges Sampler.}
\label{alg:symmetric_MC}
\SetKwData{Histogram}{Histogram}\SetKwData{Samples}{Samples}\SetKwFunction{IdentityTest}{IdentityTestIID}
\SetKwFunction{Uniform}{Uniform}
%\KwIn{$\eps$; explicit symmetric Markov chain $Q$; $m$ consecutive samples $s_1\cdots s_m$ from a symmetric Markov Chain $P$.}
%\KwOut{$P=Q$, or $P\neq Q$ if $1-\specr{\srprod{P}{Q}}>\eps$.}
\BlankLine
$\vect{k}~\leftarrow$ \Histogram($\Theta\left(\frac{m}{\log^2 (n/\eps)}\right)$ i.i.d. \Uniform[n] samples)\;
\For{$t\leftarrow 1$ \KwTo $m-1$}{
\lIf{$|\Samples[s_t]|<\vect{k}[s_t]$}{Add $(s_t\to s_{t+1})$ to $\Samples[s_t]$}
}
\eIf{$\exists i, \text{ s.t., } |\Samples[i]|<\vect{k}[i]$}{
\KwRet \textsc{Reject};
}
{
$\Samples\leftarrow\Samples[1]\cup\dots\cup\Samples[n]$\;
\KwRet \IdentityTest($\eps,$ $\{q_{ij}=\frac{1}{n}\cdot Q_{ij}\}_{i,j\in[n]}$, \Samples)\;
}
\end{algorithm}
We use as a black-box the following recently proposed identity test under the Hellinger distance\footnote{this result uses a test similar to \cite{AcharyaDK15} and is based on private communication with an author on that paper}. %We state the sample complexity of this result here.
\begin{lemma}
\label{lem:hellinger_idtest}
Given a discrete distribution $q$ supported on $[n]$ and access to i.i.d. samples from a discrete distribution $p$ on the same support, there is an algorithm which can distinguish whether $p=q$ or $\hellinger{p}{q} \ge \eps$ with probability $\ge 2/3$ using $\Ocomplex{\frac{\sqrt{n}}{\eps^2}}$ samples.
\end{lemma}
As a corollary of the lemma, we get a test that can distinguish whether $P=Q$, or $\hellingersq{\frac{1}{n}P}{\frac{1}{n}Q}\ge\eps$ using $m=\Ocomplex{\frac{n}{\eps^2}}$ i.i.d samples from $\frac{1}{n}P$, which can be viewed as a distribution on a support of size $n^2$. Lemma~\ref{lem:rho_l1_distances} shows that the required distance condition for the i.i.d. sampler is implied by our input guarantee.

\begin{lemma}
$\frac{1}{2}\sum\limits_{i,j\in[n]}\left(\sqrt{\frac{P_{ij}}{n}}-\sqrt{\frac{Q_{ij}}{n}}\right)^2=
\hellingersq{\frac{1}{n}P}{\frac{1}{n}Q}\ge\eps.$
\label{lem:rho_l1_distances}
\end{lemma}
\begin{proof}
	We note that, as $P$ and $Q$ are symmetric matrices, so is $\srprod{P}{Q}$. Thus we have
	\be
	\label{eq:sv_def}
	1-\eps = \specr{\srprod{P}{Q}} = \max_{\twonorm{\vev}=1} \vevt\circ\srprod{P}{Q}\circ\vev.
	\ee
	If we use a particular $\vev=\frac{1}{\sqrt{n}}\onev$ in \eqref{eq:sv_def}, then we get the following inequality.
	\begin{align*}
	1-\eps \ge & \frac{1}{\sqrt{n}}\onevt\circ\srprod{P}{Q}\circ\frac{1}{\sqrt{n}}\onev = \frac{1}{n}\sum\limits_{i,j} \sqrt{P_{ij}\cdot Q_{ij}} =  1-\hellingersq{\frac{1}{n}P}{\frac{1}{n}Q},
	\end{align*}
	which implies $\hellingersq{\frac{1}{n}P}{\frac{1}{n}Q}\ge\eps$.
\end{proof}

Next we get a bound on sampling complexity of Algorithm~\ref{alg:symmetric_MC}.

%\begin{lemma}
%$\frac{1}{n}\onenorm{P-Q}\ge 2\eps.$
%\label{lem:rho_l1_distances}
%\end{lemma}
%\begin{proof}
%We note that, as $P$ and $Q$ are symmetric matrices, so is $\srprod{P}{Q}$. Thus we have
%\be
%\label{eq:sv_def}
%1-\eps = \specr{\srprod{P}{Q}} = \max_{\twonorm{\vev}=1} \vev\circ\srprod{P}{Q}\circ\vevt.
%\ee
%If we use a particular $\vev=\frac{1}{\sqrt{n}}\onev$ in \eqref{eq:sv_def}, then we get the following inequality.
%\begin{align*}
%1-\eps \ge & \frac{1}{\sqrt{n}}\onev\circ\srprod{P}{Q}\circ\frac{1}{\sqrt{n}}\onevt = \frac{1}{n}\sum\limits_{i,j} \sqrt{P_{ij}\cdot Q_{ij}}\\
       %=  &\frac{1}{2n}\sum\limits_{i,j}\left(P_{ij}+Q_{ij}\right)-\frac{1}{2n}\sum\limits_{i,j}\left(P_{ij}+Q_{ij}-2\sqrt{P_{ij}\cdot Q_{ij}}\right)\\
        %= & 1 - \frac{1}{2n}\sum\limits_{i,j}\left(\sqrt{P_{ij}}-\sqrt{Q_{ij}}\right)^2 \ge 
        %1 - \frac{1}{2n}\sum\limits_{i,j}\left|\sqrt{P_{ij}}-\sqrt{Q_{ij}}\right|\cdot\left|\sqrt{P_{ij}}+\sqrt{Q_{ij}}\right|\\
        %= & 1 - \frac{1}{2n}\sum\limits_{i,j}\left|P_{ij}-Q_{ij}\right|=1 - \frac{1}{2n}\onenorm{P-Q}.
%\end{align*}
%Therefore, we conclude that $\frac{1}{n}\onenorm{P-Q}\ge 2\eps.$
%\end{proof}

\begin{theorem}
Algorithm~\ref{alg:symmetric_MC} provides correct output with probability at least $2/3$, with a single sample stream 
of length $m=\wO{\hitt{Q}\cdot\log\left(\hitt{Q}\right)+\frac{n}{\eps}}$ from $P$. 
\label{th:symmetric_ub}
\end{theorem}
\begin{proof}
	In the case $P=Q$, the probability that Algorithm~\ref{alg:symmetric_MC} proceeds to IID tester, i.e., it
	does not reject $P$, because of small number of visits to a state, is at least
	$\Prx{\forall i: |\{t\in w: s_t=i\}|>\frac{m}{8e\cdot n}}\cdot\Prx{\forall i: \frac{m}{8e\cdot n}>k_i} \ge 
	\left(1-\frac{\eps^2}{n}\right)\cdot\left(1-\frac{\eps^2}{n}\right)\ge 1-\frac{2\eps^2}{n}$. In the previous estimate, we used Lemma~\ref{lem:large_deviation_bound} 
	to bound $\Prx{\forall i: |\{t\in w: s_t=i\}|>\frac{m}{8e\cdot n}}$, the fact that $\Prx{\frac{m}{8e\cdot n} \le k_i} \le \frac{\eps^2}{n^2}$ (follows from a Chernoff bound), and a union bound.  IID tester then correctly accepts $P=Q$ with probability at least $4/5$.
	Hence, the error probability is at most $1/5+\frac{2\eps^2}{n}<1/3$.
	
	For the case $P\neq Q$, Lemma~\ref{lem:rho_l1_distances} says that if $1-\specr{\srprod{P}{Q}}>\eps$, then distributions passed down to the IID tester 
	$\{p: p_{ij}=\frac{1}{n}P_{ij}\}$ and $\{q: q_{ij}=\frac{1}{n}Q_{ij}\}$ are at least $\eps$ far in Hellinger-squared distance. Classic results on identity testing
	with independent samples give sharp bounds of $\Theta(\frac{n}{\eps^2})$ on sampling complexity with respect to total variation distance for distributions with support size $n^2$. 
	This estimate can be improved to work for Hellinger distance (Lemma \ref{lem:hellinger_idtest}). In our case this implies a  $\Ocomplex{\frac{n}{\eps}}$ sampling complexity for the IID tester.
	Furthermore,
	random mapping $\infmap{\vect{k}}:\word{P}{\infty}\to p$ (where $\vect{k}$ is a histogram of $m'=\Theta\left(\frac{m}{\log^2 (n/\eps)}\right)$ i.i.d. uniform samples from $[n]$) produces
	$m'$ i.i.d. samples from $p$. Hence, if Algorithm~\ref{alg:symmetric_MC} has sufficient samples from $P$ to define the mapping $\infmap{\vect{k}}$, it would be able to distinguish $p$ and $q$ with probability
	at least $2/3$. On the other hand, if Algorithm~\ref{alg:symmetric_MC} gets finite number of samples which are not sufficient to define the mapping $\infmap{\vect{k}}$, then 
	it correctly rejects $P$ before even running the IID tester.
	
	Thus in both cases the probability of error is at most $1/3$.
\end{proof}


%Our approach:
%\begin{enumerate}
%\item We define a mapping $\infmap{\vect{k}}$ from infinite words $\word{M}{\infty}$ of an irreducible Markov chain $M$ to $\prod_{i=1}^{n}
%[n]^{k_i}$, where $\vect{k}=(k_1,\cdots,k_n)$ is a vector of $n$ positive integers, as follows. For each infinite word $w=s_1s_2\cdots$ and each state 
%$i\in[n]$ we look at the first $k_i$ visits to state $i$ (i.e., at times $t=t_1,\dots,t_{k_i}$ with $s_{t}=i$) and write down the corresponding 
%transitions in the infinite word $w$, i.e., $s_{t+1}$. We note that every state is visited almost surely in $w$, since $M$ is an irreducible Markov chain. 
%Therefore, mapping $\infmap{\vect{k}}$ defines a probability distribution on $\prod_{i=1}^{n}[n]^{k_i}$. We note that by construction the realized values 
%in $\prod_{i=1}^{n}[n]^{k_i}$ of each fixed state $i$ and across all different 
%states are independent.
%\item We show that for large enough $m=\wO{\covert{M}+n\cdot f(\eps)}$ and 
%$k_i=\frac{\Ex{\text{\# visits to } i}}{\log^2 n}=\frac{m}{n\log^2 n}$ the mapping
%$\infmap{\vect{k}}$ is well defined for a finite $m$ number of samples for all but a small fraction of the words in $\word{M}{\infty}$. (Here we use 
%the fact that $M$ is symmetric irreducible MC, implying that $\onev$ is the stationary distribution.)
%\item We are going to use as a black-box \cite{AcharyaDK15} for identity $L_1$-testing with i.i.d. samples from a distribution with a support of size $n^2$. We want to simulate a number of i.i.d samples where we first pick uniformly at random a state $i\in[n]$ and then observe  
%transition from $i$ according to transition probabilities of $P$. We first simulate $m'$ (to be determined later) i.i.d. samples from $[n]$. Let 
%$\vect{k}$ be the histogram of these $m'$ samples (note that $\max_{i} k_i \le O(m'\log n /n)$ with high probability). 
%We apply $\infmap{\vect{k}}$ mapping to our stream of $m$ consecutive samples of Markov chain $P$, which is well defined with high probability. 
%Apart from a small fraction of events (when $\max_{i} k_i$ is too large, or $\infmap{\vect{k}}$ is not defined) we obtain the desired $m'$ i.i.d. 
%samples. 
%
%Now \cite{AcharyaDK15} says that we can test using $m=\Ocomplex{\frac{n}{\eps^2}}$ samples whether $P=Q$, or tell that $P\neq Q$, if $\frac{1}{n}\onenorm{P-Q}\ge\eps$. We use our $m'=\wO{\frac{n}{\eps^2}}$ samples to detect whether $\frac{1}{n}\onenorm{P-Q}\ge\eps$. It remains to show that the latter guarantee is implied by our notion of distance.
%
%We note that, as $P$ and $Q$ are symmetric matrices, so is $\srprod{P}{Q}$. Thus we have
%\be
%\label{eq:sv_def}
%1-\eps = \specr{\srprod{P}{Q}} = \max_{\twonorm{\vev}=1} \vev\circ\srprod{P}{Q}\circ\vevt.
%\ee
%
%If we use a particular $\vev=\frac{1}{\sqrt{n}}\onev$ in \eqref{eq:sv_def}, then we get the following inequality.
%\begin{align*}
%1-\eps \ge & \frac{1}{\sqrt{n}}\onev\circ\srprod{P}{Q}\circ\frac{1}{\sqrt{n}}\onevt = \frac{1}{n}\sum\limits_{i,j} \sqrt{P_{ij}\cdot Q_{ij}}\\
       %=  &\frac{1}{2n}\sum\limits_{i,j}\left(P_{ij}+Q_{ij}\right)-\frac{1}{2n}\sum\limits_{i,j}\left(P_{ij}+Q_{ij}-2\sqrt{P_{ij}\cdot Q_{ij}}\right)\\
        %= & 1 - \frac{1}{2n}\sum\limits_{i,j}\left(\sqrt{P_{ij}}-\sqrt{Q_{ij}}\right)^2 \ge 
        %1 - \frac{1}{2n}\sum\limits_{i,j}\left|\sqrt{P_{ij}}-\sqrt{Q_{ij}}\right|\cdot\left|\sqrt{P_{ij}}+\sqrt{Q_{ij}}\right|\\
        %= & 1 - \frac{1}{2n}\sum\limits_{i,j}\left|P_{ij}-Q_{ij}\right|=1 - \frac{1}{2n}\onenorm{P-Q}.
%\end{align*}
%
%Therefore, we conclude that $\frac{1}{n}\onenorm{P-Q}\ge 2\eps.$
%
%\end{enumerate}

==> preamble.tex <==


%%% USED FOR COMMENTS

\def\a{\alpha}
\def\b{\beta}
\def\c{\chi}
\def\d{\delta}
\def\D{\Delta}
%\def\e{\epsilon}
\def\e{\eta}
\def\eps{\ve}
\renewcommand{\epsilon}{\ve}
\def\ve{\varepsilon}
\def\f{\phi}
\def\F{\Phi}
\def\g{\gamma}
\def\G{\Gamma}
\def\k{\kappa}
\def\K{\Kappa}
\def\z{\zeta}
\def\th{\theta}
\def\Th{\Theta}
\def\l{\lambda}
\def\la{\lambda}
%\def\L{\Lambda}
\def\m{\mu}
\def\n{\nu}
\def\p{\pi}
\def\P{\Pi}
\def\r{\rho}
\def\R{\Rho}
\def\s{\sigma}
\def\S{\Sigma}
\def\t{\tau}
\def\om{\omega}
\def\Om{\Omega}
\def\smallo{{\rm o}}
\def\bigo{{\rm O}}
\def\to{\rightarrow}
\def\ex{{\bf Exp}}
\def\cd{{\cal D}}
\def\rme{{\rm e}}
\def\hf{{1\over2}}
\def\R{{\bf  R}} 
\def\cala{{\cal A}}
\def\calt{{\cal T}}
\def\cale{{\cal E}}
\def\Fscr{{\cal F}}
\def\cc{{\cal C}}
\def\calc{{\cal C}}
\def\call{{\cal L}}
\def\calm{{\cal M}}
\def\calh{{\cal H}}
\def\cali{{\cal I}}
\def\bk{\backslash}

\def\rad{r}
\def\bigrad{R}
\def\dh{d_H}
\def\Poi{\text{Poi}}

\newcommand{\Exp}{\mbox{\bf Exp}}
\newcommand{\E}{\mbox{\bf E}}
\newcommand{\Ee}[1]{\mbox{\bf E}\left[#1\right]}
\newcommand{\Eee}[2]{\mbox{\bf E}_{#1}\left[#2\right]}
\newcommand{\CEe}[2]{\mbox{\bf E}\left[#1\vline #2\right]}
\newcommand{\CEee}[3]{\mbox{\bf E}_{#1}\left[#2 \vline #3 \right]}

\newcommand{\Var}{\mbox{\bf Var}}
\newcommand{\sign}{\mbox{\bf sign}}

\newcommand{\erf}{\mbox{\text erf}}
\newcommand{\erfc}{\mbox{\text erfc}}

\newcommand{\pr}[2][]{\mbox{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[#2\right]}
\newcommand{\given}{\ \mid\ }
\newcommand{\reals}{\mathbb{R}}

\newcommand{\U}{\mathcal{U}_n}
\newcommand{\I}{\mathcal{I}_n}

\newcommand{\twonorm}[1]{\left\lVert #1 \right\rVert_2}
\newcommand{\onenorm}[1]{\left\lVert #1 \right\rVert_1}


\newcommand{\limninf}{\lim_{n \rightarrow \infty}}
\newcommand{\proofstart}{{\bf Proof\hspace{2em}}}
\newcommand{\tset}{\mbox{$\cal T$}}
\newcommand{\proofend}{\hspace*{\fill}\mbox{$\Box$}}
\newcommand{\bfm}[1]{\mbox{\boldmath $#1$}}
%\newcommand{\reals}{\mbox{\bfm{R}}}
%\newcommand{\expect}{\mbox{\bf Exp}}
\newcommand{\he}{\hat{\e}}
\newcommand{\card}[1]{\mbox{$|#1|$}}
\newcommand{\rup}[1]{\mbox{$\lceil{ #1}\rceil$}}
\newcommand{\rdn}[1]{\mbox{$\lfloor{ #1}\rfloor$}}
\newcommand{\ov}[1]{\mbox{$\overline{ #1}$}}
\newcommand{\inv}[1]{$\frac{1}{ #1}$}
\newcommand{\dtv}{d_{\mathrm {TV}}}
\newcommand{\dk}{d_{\mathrm K}}
\newcommand{\dkl}{d_{\mathrm {KL}}}
\newcommand{\dskl}{d_{\mathrm {SKL}}}
\newcommand{\Tr}{{\mathrm {Tr}}}
\newcommand{\abss}[1]{\left\lvert {#1} \right\rvert}
\newcommand{\cnote}[1]{ {\red #1} }


\newtheorem{theorem}{Theorem}
\newtheorem{metatheorem}{Meta Theorem}
\newtheorem{nontheorem}{Non Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{case}{Case}
\newtheorem{dfn}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\newtheorem{openquestion}{Open Question}
\newtheorem{res}{Result}
\newcommand{\ignore}[1]{}
\providecommand{\poly}{\operatorname*{poly}}

\newenvironment{proofsketch}{\noindent {\em {Proof (sketch):}}}{$\blacksquare$\vskip \belowdisplayskip}
\newenvironment{prevproof}[2]{\noindent {\em {Proof of {#1}~\ref{#2}:}}}{$\hfill\qed$\vskip \belowdisplayskip}

%\newenvironment{prevproof}[2]{\noindent {\em {Proof of
%{#1}~\ref{#2}:}}}{$\blacksquare$\vskip \belowdisplayskip}

% Allow argmax operation
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\img}{img}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\avg}{avg}

%\def\qedsymbol{\blksquare}
\newcommand{\bg}[1]{\medskip\noindent{\bf #1}}
%\newcommand{\ed}{{\hfill\qedsymbol}\medskip}
\newenvironment{proofof}[1]{\bg{Proof of #1 : }}{\qed}



%%%
%%% Packed enumerate / itemize
%%%

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\definecolor{Red}{rgb}{1,0,0}
\def\red{\color{Red}}
\newcommand{\costasnote}[1]{{\red #1}}
\newcommand{\oldbound}[1]{{}}


\newcommand{\sparse}{\mathrm{sparse}}
\newcommand{\lrg}{\mathrm{large}}

\newcommand{\goodgamma}{\chi_{\tau_2}}
\newcommand{\dm}{d_{\max}}
\newcommand{\ind}{\mathbbm{1}}
\DeclareMathOperator{\sech}{sech}


==> reduction_to_advers_testing.tex <==
x

Let $\ell=C\frac{\log n}{\eps}$ be the sufficient length of the word from Claim~\ref{cl:symm_spectrum} that allows us to distinguish between $P$ and 
$Q$ from a word of length $\ell$ with probability at least $1/2$, i.e., such $\ell$ that $\dtv{\word{P}{\ell}}{\word{Q}{\ell}}\ge \frac{1}{2}.$

We have $m$ consecutive samples drawn from MC $P$. For each transition from state $v$ we calculate $\dtv{P_v}{Q_v}$. We split these $m$ samples into $\frac{m}{\ell}$
blocks and analyze each block separately. First, let us calculate the expected value of the average TV distance between $P_v$ and $Q_v$, where $v$ is also a random state
reached within $\ell$ consecutive steps. To this end 
we define random variable $\xi(s_0)$ 
\[
\xi(w)\eqdef\sum_{s\in w} \dtv{P_s}{Q_s},\quad\quad \text{where } w=s_0\ldots s_\ell\sim \word{P}{\ell}
\] 
that corresponds to the average TV distance between $P$ and $Q$ if we start from state $s_0$ and follow Markov Chain $P$. Then 

\be
\Ex{\xi(s_0)}=\sum_{t=0}^{\ell-1}
\Exlong[\substack{s_t\in w\\ w\sim \word{P}{t}}]{\dtv{P_{s_t}}{Q_{s_t}}}=
\sum_{t=0}^{\ell-1}\dtv{\onevti[s_0]\circ P^t\circ P}{\onevti[s_0]\circ P^t\circ Q}.
\label{eq:expected_tv_ell}
\ee

On the other hand, we have 

\begin{multline}
\dtv{\word{P}{\ell}}{\word{Q}{\ell}} =\sum\limits_{s_1,\ldots,s_\ell}
\left|
P_{s_0s_1}\cdot P_{s_1s_2}\ldots \cdot P_{s_{\ell-1}s_{\ell}}-
Q_{s_0s_1}\cdot Q_{s_1s_2}\ldots \cdot Q_{s_{\ell-1}s_{\ell}}
\right|\\
\le\sum\limits_{s_1,\ldots,s_\ell}\sum\limits_{i=0}^{\ell-1} 
P_{s_0s_1}\ldots P_{s_{i-1}s_i}\left|P_{s_i s_{i+1}}-Q_{s_i s_{i+1}}\right|
Q_{s_{i+1}s_{i+2}}\ldots Q_{s_{\ell-1}s_{\ell}}
%P_{s_0s_1}\ldots P_{s_is_{i+1}}Q_{s_{i+1}s_{i+2}}\ldots Q_{s_{\ell-1}s_{\ell}}-
%Q_{s_{i}s_{i+1}}\ldots Q_{s_{\ell-1}s_{\ell}}
\\
=\sum\limits_{i=0}^{\ell-1}\sum\limits_{s_1,\ldots,s_{i+1}} 
P_{s_0s_1}\ldots P_{s_{i-1}s_i}\left|P_{s_i s_{i+1}}-Q_{s_i s_{i+1}}\right|
=\sum\limits_{i=0}^{\ell-1} 
\dtv{\onevti[s_0]\circ P^i\circ P}{\onevti[s_0]\circ P^i\circ Q}
\label{eq:dtv_telescopic_MC}
\end{multline}

Combining previous bound with the expression~\eqref{eq:expected_tv_ell} for the expectation of $\xi(s_0)$ we obtain
\[
\Ex{\xi(s_0)}\ge\dtv{\word{P}{\ell}}{\word{Q}{\ell}}\ge\frac{1}{2},
\]
where the last inequality is the result of our choice of $\ell$ for any starting state $s_0$. 
Now we observe that the expectation over all $\frac{m}{\ell}$ blocks is at least $\frac{m\cdot\eps}{2\cdot C\cdot \log n}$.
On the other hand, the random variables $\xi$ for each new block only depends on the initial state $s_{k\cdot\ell}$ and is bounded between $[0,\ell]$. 
Thus, we can employ Azuma-Hoeffding inequality to obtain exponential tail bound for the sum $\sum_{k=0}^{\lfloor m/\ell\rfloor}\xi(s_{k\cdot\ell})$ (which is a super-martingale).
We note that the length $\ell=O\left(\frac{\log n}{\eps}\right)$ is negligible compared to the number of blocks $m/\ell$ and to our lower bound of $\frac{m\cdot\eps}{2\cdot C\cdot \log n}$ on the 
expectation. Now if $m_1,m_2,\ldots,m_n$ are the number of visits to states from $1$ to $n$ in the $m$ consecutive samples from $P$ we get the following bound on the average TV distance between transitions in Markov Chains $P$ and $Q$.

\begin{lemma}
$\sum_{v\in[n]}m_v\cdot\dtv{P_v}{Q_v}\ge\frac{m\cdot\eps}{2\cdot C\cdot \log n}$ with very high probability (the error probability decreases exponentially with $n$).
\label{lem:total_TV_bound}
\end{lemma}


==> riff_shuffle_test.tex <==
%As in the GSR and CD models described earlier, 
It is natural to parameterize a riffle shuffle by 
(i) the distribution of possible cuts, and (ii) the probability $p_{ab}$ of choosing the next card to be dropped from the left pile for each profile $(a,b)$ of the number of cards left in the two 
piles. In this description each riffle shuffle
can be represented as a random walk on a 2-dimensional grid $(a,b)\in\Z^2$ that starts at a position chosen from a specified distribution on the diagonal $a+b=n$ 
and decreases the sum of the coordinates $a+b$ by one at each move. In fact, we get an almost one-to-one correspondence between riffle shuffles and the aforementioned random walks 
on the $n\times n$ grid (the only shuffle that corresponds to more than one path on the grid is the identical permutation). Therefore, by knowing the initial permutation of cards at the beginning of the shuffle, and by scanning the permutation of cards obtained after
one riffle shuffle we can reconstruct (except for the unimportant case of void shuffle) the random walk of $n$ steps taken by our grid Markov Chain. 
We note that this grid representation might not be enough to accurately model the behavior of a dealer. For example, shufflers often tend to drop chunks of consecutive cards from left or right pile regardless of the pile sizes. To address this issue one might want to introduce 
an extra parameter -- which pile the last card was taken from -- to our grid parameterization, which can be done by doubling the number of states in the Markov 
chain. To capture this and other potential extensions of the Markov chain model for a riffle shuffle we introduce the following general theoretical framework.
 
\begin{definition}[Sparse MC]
\label{def:sparse}
Consider a Markov chain defined by transition matrices $P=\{P_t\}_{t=1}^{n_1}$ over $n_2$ states that proceeds in $n_1$-step rounds, as follows. Starting from some state $X_0=s_0$ it follows a transition according to $P_1$, then $P_2$, etc, then $P_{n_1}$ to arrive at some state $X_1$. Starting from $X_1$ it repeats transitions according to  $P_1,\ldots,P_{n_1}$, in sequence, and so on, ad infinitum. The transition matrices are assumed {\em sparse} having $O(n_3)$ non-zero entries.
\end{definition}
To relate the above definition to the riffle shuffle, we should think of the state space as the set $\{(a,b)| 0 \le a+b \le n\}$, where $n=52$. So in particular, there are $n_2=O(n^2)$ states. There are $n_1=n+1$ transition matrices. $P_1$ takes us from an uncut deck of cards, corresponding to the state $(0,0)$, to a cut deck corresponding to a state in set $\{(a,b)| a+b = n\}$. Then each other transition matrix $P_t$, $t >1$, maps a state in  $\{(a,b): a+b=n-t+2\}$ to states in $\{(a,b): a+b=n-t+1\}$. All transition matrices have $O(n)$ non-zero entries. Note that this way of modeling the riffle shuffle, while forgetting the specific ordering of cards, maintains the essential information that we need to test a riffle shuffle model, and in particular saves exponentially in the size of the state space.

%
%$n_1$ steps, and then repeats these $n_1$. Each transition matrix $P_t$ is a {\em sparse} matrix having at most $O(n)$ non zero entries. The initial distribution (e.g. the initial cut in the riffle shuffle) is modeled as a transition 
%matrix $P_1$ from a single state $\onee$ to the distribution over $n$ states (e.g. in the riffle shuffle the cut choose some state from $\{(a,b): a+b=n-1\}$), each of the matrices $\{P_t\}_{t\ge 2}$ describes transition probabilities among states (e.g. in the riffle shuffle matrix $P_t$ describes transition probabilities from states $\{(a,b): a+b=n-t+1\}$ to states $\{(a,b): a+b=n-t\}$).
%\end{definition}

\vspace{-10pt}\paragraph{Testing sparse Markov chains.} We develop tools for goodness-of-fit testing of sparse Markov chain models. 

\medskip \noindent {\bf Simplification:} To avoid carrying around several parameters, we will henceforth take $n_1=n_3=n$ and $n_2= O(n^2)$, which is what we would need for the riffle shuffle. Our results, namely the use and analysis of our edge tester, extend to the general case. We will also assume that $P_{n_1}$ is the trivial matrix taking all states into a fixed state $s_0$, which is also what we would need for the riffle shuffle, namely $s_0=(0,0)$. Again, our results easily extend to the general case. 

\medskip \noindent With these simplifications in place, we can break an observed trajectory from a sparse Markov chain model into ``samples.'' One sample is a 
word $w=s_0\cdots s_{n}$, whose transitions $s_{t-1}\to s_t$ are performed according to transition 
 matrix $P_t$. 

\smallskip As described in Section \ref{sec:distance}, a natural measure of distance between two Markov chains $Q=\MCseqQ$ and $P=\MCseqP$ is the total variation 
distance between words of certain length sampled from these chains.
 %distributions $\word{Q}{n}$ and $\word{P}{n}$, as it precisely captures our ability to distinguish
%which Markov chain $P$ or $Q$ a single word $w$ of length $n$ was generated from. 
As we have a natural length $n$ to use here, we can take our distance between chains to be $\dist{P}{Q}\eqdef\dtv{\word{P}{n}}{\word{Q}{n}}$.

We note that $\frac{\distsq{P}{Q}}{2}=\frac{\dtvsq{\word{P}{n}}{\word{Q}{n}}}{2}
\le\hellingersq{\word{P}{n}}{\word{Q}{n}}$ and for Hellinger-squared distance 
we can derive a formula similar to \eqref{eq:hellinger_square_algebraic}:
$
1-\hellingersq{\word{P}{n}}{\word{Q}{n}}=\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev.
$ In particular, we could alternatively define our distance using the spectral approach we took in Section~\ref{sec:symmetric}. 
%We show in Appendix~\ref{app:riffle_model} that the two notions are tightly related, but we opt for the use of total variation distance as we find it more natural in this context.
To this end we can define a large matrix $Q^*$ for 
Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$. 
%In our running application to card shuffling, it captures the divergence in one iteration of two riffle shuffles with different para total variation distance of the difference in one step of the shuffle.


%\begin{multline*}
%1-\hellingersq{\word{P}{n}}{\word{Q}{n}}=\sum_{w=s_0\ldots s_{n}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}
%=\trans{\left[\sum_{w=s_0\ldots s_{n-1}s}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{s\in[n]}\circ\onev\\
%=\trans{\left[\sum_{\substack{w=s_0\ldots s_{n-1}\\s_{n-1}=r}}\sqrt{\Prlong[P]{w}\Prlong[Q]{w}}\right]}_{r\in[n]}\circ\srprod{P_n}{Q_n}\circ\onev
%=\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev.
%\end{multline*}


%\begin{itemize}
%\item Formulation as testing Markov Chains with $n$ steps on a $n\times n$ grid.
%\item General model: sparse Markov Chains with $n$ transition matrices $P_i$, each having a total number of $O(n)$ of non zero entries.
      %We model cut (initial distribution) as a transition $P_1$ from a single state $\onee$ to the distribution over $n$ initial states.    
%\end{itemize}
%
%Derivation of 
%$$\frac{\distsq{P}{Q}}{4}\le\hellingersq{P}{Q}=1-\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev$$
%\begin{remark}
%It is also possible to define $\dist{P}{Q}$ via the spectral radius approach as was done in Section \ref{sec:distance}. To this end we can define a large matrix $Q^*$ for 
%Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
%$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
%We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$.
%\end{remark}
%Alternative description as a long Markov Chain cycled from the state $t=n$ to states $t=0$ according to distribution $p_0$. 
%Relation between spectral radius $\rho(A)$ and $\dist{\MCseqP}{\MCseqQ}$.
%With this distance definition in hand it is a very reasonable question to ask:
%\begin{quote}
%Given a specific probabilistic model for shuffling (a sparse Markov chain $Q$), how many shuffles (samples) does one need to test whether $Q$ is an accurate model for shuffling?
%\end{quote}
With these definitions we are interested in the following testing problem:
%\begin{description}
%\item[Input:] $Q=\MCseqQ$, s.t. each $Q_t$ is sparse, i.e., it has only $O(n)$ non zero entries in total;
%$m$ samples of $w=s_0\cdots s_{n}$ from a sparse Makrov chain $P=\MCseqP$.
%\item[Output:] $P=Q$, or $P\neq Q$ if $\dist{P}{Q}\ge\eps$. 
%\end{description}

\begin{algorithm}[H]
\KwIn{$Q=\MCseqQ$, s.t. each $Q_t$ is sparse, i.e., it has only $O(n)$ non zero entries in total;
$m$ samples of $w=s_0\cdots s_{n}$ from a sparse Markov chain $P=\MCseqP$.}
\KwOut{$P=Q$, or $P\neq Q$ if $\dist{P}{Q}\ge\eps$.}
\end{algorithm}


==> riffle_model.tex <==
It is also possible to define $\dist{P}{Q}$ via the spectral radius approach as was done in Section \ref{sec:distance}. To this end we can define a large matrix $Q^*$ for 
Markov chain $Q$ that acts on $n(n+1)$ states ($n+1$ distinct copies $n_t$ of $n$ states for each $t\in\{0,\cdots, n\}$), such that $Q^*$ behaves exactly like matrix 
$Q_t$ on states $n_{t-1}$ transitioning them to sates $n_{t}$, and for $t=n$ states $n_t$ are transitioned to the initial state $s_1$ with $t=0$. 
We similarly define large matrix $P^*$ for the Markov chain $P$. Then it turns out that the spectral radius $\specr{\srprod{Q^*}{P^*}}^{n+1}=1-\hellingersq{\word{P}{n}}{\word{Q}{n}}$.


%A commonly used technique to shuffle decks of $n=52$ cards is the riffle shuffle:
%first, the dealer cuts the deck into two piles. Then, the piles are ``riffled'' together:
%the shuffler successively drops cards from the bottom of each pile to form a new pile. There
%are two variable aspects in this procedure. First, the numbers of cards in
%each pile after the initial cut can vary. Second, each time the dealer drops a card she needs to choose the pile from which the card is dropped.
%
%The standard and by far the most well studied mathematical model for riffle shuffle is due to Gilbert, Shannon, and Reeds (GSR-model for short): 
%first, the deck is cut into two packs according to a $(n,0.5)$-binomial random variable where $n$ is the number of cards in the deck; 
%next, cards are dropped one by one from the bottom of one or the other pile with probability proportional to the relative sizes of the
%piles (i.e., if the left pile contains $a$ cards and the right pile $b$ cards, the next card drops from the left pile with probability 
%$\frac{a}{a + b}$). A well known result in this model is due to Bayer and Diakonis~\cite{BayerDiaconis} who gave a sharp mathematical 
%analysis of the mixing time of the riffle shuffle Markov chain showing that ``seven shuffles are necessary and sufficient to approximately randomize $52$ cards'', which actually convinced Las Vegas 
%casinos to increase the number of shuffles in their shuffling procedures.
%
%% Emperical work
%There have also been some statistical studies validating the adequacy of the GSR model for riffle shuffles in practice.
%For example Diaconis and Reeds (see~\cite{DiaconisLectures88}) did empirical analysis of about a hundred riffle shuffles performed by each of them.
%They looked at a few different statistics including the count of consecutive cards dropped from each of the piles. These statistics revealed certain differences between the two
%shufflers, in particular, Diaconis' shuffles (a former professional magician) were much neater and closer to the shuffles of professional dealers in Las Vegas casinos, 
%while Reeds' shuffles were more like ``ordinary person'' shuffles. In another work (see~\cite{DiaconisTechReport02} open problem 5) Chakraborty and Diakonis 
%pointed out that some shuffling machines performing riffle shuffles do not conform to the GSR model. Instead they proposed 
%another model to capture this observed phenomenon (we call it {\em CD-model}), where, in contrast to the GSR model, cards are dropped with probability $\frac{a}{a+b}$ from the pile containing $b$ cards 
%and $\frac{b}{a+b}$ from the pile containing $a$ cards.
%
%Despite a large interest in card shuffling and all the existing work mentioned above, there has not been much theoretical statistical 
%analysis on the question of testing whether a particular shuffling model is accurate. 


==> shuffle_model.tex <==
A commonly used technique to shuffle decks of $n=52$ cards is the riffle shuffle:
first, the dealer cuts the deck into two piles. Then, the piles are ``riffled'' together:
the shuffler successively drops cards from the bottom of each pile to form a new pile. There
are two variable aspects in this procedure. First, the numbers of cards in
each pile after the initial cut can vary. Second, each time the dealer drops a card she needs to choose the pile from which the card is dropped.

The most well studied mathematical model for riffle shuffle is due to Gilbert, Shannon, and Reeds (GSR-model for short): 
first, the deck is cut into two packs according to a $(n,0.5)$-binomial random variable where $n$ is the number of cards in the deck; 
next, cards are dropped one by one from the bottom of one or the other pile with probability proportional to the relative sizes of the
piles (i.e., if the left pile contains $a$ cards and the right pile $b$ cards, the next card drops from the left pile with probability 
$\frac{a}{a + b}$). A well known result in this model is due to Bayer and Diaconis~\cite{BayerDiaconis} who gave a sharp mathematical 
analysis of the mixing time of the riffle shuffle Markov chain showing that ``seven shuffles are necessary and sufficient to approximately randomize $52$ cards,'' which actually convinced Las Vegas 
casinos to increase the number of shuffles in their shuffling procedures.

% Emperical work
There have been some statistical studies validating the accuracy of the GSR model for riffle shuffles in practice.
For example Diaconis and Reeds (see~\cite{DiaconisLectures88}) did empirical analysis of about a hundred riffle shuffles performed by each of them.
They looked at a few different statistics including the count of consecutive cards dropped from each of the piles. 
%These statistics revealed certain differences between the two
%shufflers: Diaconis' shuffles (a former professional magician) were much neater and closer to the shuffles of professional dealers in Las Vegas casinos, 
%while Reeds' shuffles were more like ``ordinary person'' shuffles. 
In other work (see~\cite{DiaconisTechReport02} open problem 5), Chakraborty and Diaconis 
pointed out that some shuffling machines performing riffle shuffles do not conform to the GSR model. Instead they proposed 
another model to capture this observed phenomenon (we call it {\em CD-model}), where, in contrast to the GSR model, cards are dropped with probability $\frac{a}{a+b}$ from the pile containing $b$ cards 
and $\frac{b}{a+b}$ from the pile containing $a$ cards.

Despite a large interest in card shuffling and all the existing work mentioned above, there has not been much theoretical statistical 
analysis on the question of testing whether a particular shuffling model is accurate. In this section we propose a new theoretical 
framework for the statistical analysis of riffle shuffles. We aim to address the following question:
\begin{quote}
How many trials are needed to test that shuffles are performed according to a specified probabilistic model?   
\end{quote}





==> sparse_lb.tex <==
In this section we will show that any algorithm that tests identity of a sparse Markov chain representing 
card riffle shuffling requires at least $\Omega\left({\frac{n}{\eps^2}}\right)$ independent trials, where 
each trial is a $n$-length word generated by a sparse Markov chain.
We recall Definition~\ref{def:sparse} of a sparse Markov chain adapting it slightly for the convenience of lower bound presentation.
Sparse Markov chains $P=\{P_t\}_{t=1}^{T}, Q=\{Q_t\}_{t=1}^{T}$: each independent run consists of $T=O(n)$ time steps; has $O(n)$ states for each time $t$;  Markov chain starts
from a single state at $t=0$ ; there are only $O(1)$ possible transitions $P_t(ij)\neq 0$ from each state 
$i$ to other states for all but the very first time step $t>0$.

\begin{theorem}
\label{thm:sparse-lower-bound}
There is an instance of Identity testing problem for a sparse Markov chain $Q$ that requires
at least $m\ge\Omega(\frac{n}{\eps^2})$ i.i.d. samples to check identity of $Q$ with $99$\% confidence\footnote{We assume
	$\eps=\omega(n^{-1/6})$ in the requirement $\dist{P}{Q}\ge\eps$, when $P\neq Q$.}.
%There exists a constant $c>0$, such that any algorithm which, given the description of a sparse Markov chain $Q$ with 
%$O(n)$ layers and each layer containing $O(n)$ states, and sample access to words from another sparse Markov chain $P$ 
%over the same set of states as $Q$, distinguishes between the cases $P \equiv Q$ and $\dist{P}{Q} \ge \eps$ with 
%probability at least $99/100$ requires at least $k \geq \frac{cn}{\eps^2}$ samples.
\end{theorem}
%Complete argument is provided in Appendix~\ref{app:sec_riffle_lb}. 

\begin{proof}
	The high-level proof idea is similar to that of Theorem~\ref{thm:symm-lower-bound}, but particular details and proofs are more involved. At an abstract level, we construct a sparse Markov chain $Q$, 
	with respect to which we are interested in testing identity, and a class of sparse Markov chains $\mathcal{P}$ such that 
	\begin{enumerate}
		%\item $\mathcal{Q}$ is a single Markov chain $Q$ which identity we are testing. 
		\item Every $P \in \mathcal{P}$ is at least $\eps$ far from $Q$, i.e., $\dtv{\word{P}{T}}{\word{Q}{T}}\ge \eps$ for any $P \in \mathcal{P}$.
		\item There is a constant $c > 0$, such that it is impossible to distinguish $m$ i.i.d. samples of $T$-length words generated by 
		a random Markov chain $\bar{P}\sim \mathcal{P}$ from the samples produced by $Q$ with probability 
		equal to or greater than $\frac{99}{100}$, for $m\le\frac{cn}{\eps^2}$.
	\end{enumerate}
	
	We denote the joint distribution of $m$ i.i.d. samples from $Q$ by $Q^{\otimes m}$ and that from $\bar{P}$ by $\bar{P}^{\otimes m}$.
	To prove the last point we show that $\dtv{Q^{\otimes m}}{\bar{P}^{\otimes m}}$ is small for some $m=\Om{\frac{n}{\eps^2}}$.
	We now describe our construction. To simplify presentation, we use multi-edges in the description of sparse Markov chains.
	We convert this instance into simple edge graph by the same duplicating trick we employed in 
	the lower bound construction of Theorem~\ref{thm:symm-lower-bound}.
	
	%We respectively denote the words of length $m$ obtained from $Q$ by $\word{Q}{m}$, and from a Markov chain $\bar{P}\sim\mathcal{P}$ by $\word{\bar{P}}{m}$.\\
	%We will assume $n$ is odd without loss of generality for the following lower bound construction.
	%\noindent 
	
	
	\begin{description}
		\item[Markov Chain $Q$:] $T=2n+1$ time steps; single state at $t=0$, states $[2n]$ at each $1\le t\le T$.
		All states are divided into two categories: {\em Frequently} visited ($F$) $\eqdef\{2i-1, i\in[n]\}$ and {\em Rare} ($R$) $\eqdef\{2i,i\in[n]\}$.
		Table below describes weighted multi-graph $Q=\{Q_t\}_{t=1}^{T}$: $x\in F,$ $y\in R$, $x,y\in [2n]$ denote respective generic frequent and rare states. 
		We adopt notational convention: $0\eqdef 2n$, $2n+1\eqdef 1$.   
		
		\begin{tabular}{r|c|c|c|c}
			&  $F\to F$        & $F\to R$       & $R\to F$       &     $R\to R$   \\ 
			%				&  $(2i\to 2j)$    & $(2i\to 2j+1)$ & $(2i+1\to 2j)$ & $(2i+1\to 2j+1)$ \\ 
			\hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=1:} }
			&  $(1\to x)\in E$                  & \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} 
			& \multicolumn{1}{|c}{\multirow{2}{*}{$\emptyset$}}                  \\ %\hline
			& $Q_{1}(1,x)=\frac{1}{n}$       &                                                   &                                                     &              \\ \hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=2k:} }
			& $(x\to x)\in E$             &  $(x\to x\pm 1)\in E$           &  $(y\to y\pm 1)\in E$           & \multicolumn{1}{|c}{\multirow{2}{*}{$\emptyset$}}     \\ %\hline
			& $Q_t(x,x)=1-\frac{2}{n}$ &  $Q_t(x,x\pm 1)=\frac{1}{n}$ &  $Q_t(y,y\pm 1)=\frac{1}{2}$ &                                                       \\ \hline
			\multicolumn{1}{ r| }{\multirow{2}{*}{t=2k+1:} }				
			&  $(x\to x)\in E$            &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} &  \multicolumn{1}{|c|}{\multirow{2}{*}{$\emptyset$}} 
			&  $(y\to y)_{1,2}\in E$                               \\ %\hline
			&  $Q_t(x,x)=1$            &                                                     &                                                     
			&  $Q_t(e_1)=Q_t(e_2)=\frac{1}{2}$                                  \\ %\hline
		\end{tabular}
		%\begin{align*}
		%t=1:& \quad\quad \forall 2i+1\in[2n]\quad \quad (1,2i+1)\in E\quad  \quad Q_{1}(1\to 2i+1)=\frac{1}{n}\\
		%t=2k:& \quad\quad \forall i\in[2n]\quad \quad (1i)\in E\quad  \quad Q_{1}(1i)=\frac{1}{2n}\\
		%t=2k+1:& \quad\quad \forall i\in[2n]\quad \quad (1i)\in E\quad  \quad Q_{1}(1i)=\frac{1}{2n}
		%%Q_{(ij)_1}=\frac{1}{2(n-1)} \quad\quad Q_{(ij)_2}=\frac{1}{2(n-1)}\quad\quad \text{ for any } i\neq j.
		%\end{align*}
		\item[Family $\mathcal{P}$:] every $P \in \mathcal{P}$ has the same set of states and edges as $Q$.
		Similar to the construction in Section~\ref{sec:symmetric_lb}, we only change weights of the multi-edge 
		pairs (independently and uniformly at random for each pair $(y\to y)_{1,2}$ and time $t$): 
		\[
		P_{t}(e_{1,2})=\frac{1\pm 4\eps}{2} \quad\quad\text{ or }\quad\quad
		P_{t}(e_{1,2})=\frac{1\mp 4\eps}{2}.
		\]
	\end{description}
	
	%The family $\mathcal{P}$ of Markov chains is constructed by making slight random perturbations to the multi-edge 
	%transitions in $Q$. In particular, every $P \in \mathcal{P}$ has the same set of states as $Q$. In each $P$, every 
	%transition is identical to those in $Q$ except the multi-edge transition probabilities from a rare state in an 
	%even-indexed layer to the corresponding rare state in the next layer. Instead of having a $1/2$ transition probability 
	%on each edge from $(2i,2t)$ to $(2i,2t+1)$, we will have as transition probabilities either $1/2(1 \pm 2\eps)$ or 
	%$1/2(1 \mp 2\eps)$ chosen uniformly at random. Hence this creates a class of sparse Markov chains which contains 
	%$2^{O(n^2)}$ sparse Markov chains.
	%
	%
	%\begin{itemize}
	%\item \textbf{The Markov Chain $Q$}\\
	%$Q$ will have $2n+1$ layers each with $n$ states along with an additional initial layer which has transitions with 
	%probability $2/n+1$ from state 1 to each of the odd indexed states in layer 2. Label the states in layer $t$ as 
	%$(1,t),(2,t)\ldots,(n,t)$. States $(2i-1,t)$ are frequent states and states $(2i,t)$ are rare states for each $t > 1$. 
	%From every frequent state in an even-indexed layer $(2i-1,2t)$, there exists a transition to frequent state $(2i-1,2t+1)$ 
	%with probability $(1-2/n)$ and a transition to rare state $(2i,2t+1)$ with probability $1/n$ and to rare state 
	%$(2i-2,2t+1)$ with probability $1/n$. If $i=1$ (or $i=n$), then for any even-indexed layer $2t$ there is a transition 
	%from $(1,2t)$ ($(n,2t)$) to the rare state $(2,2t+1)$ ($(n,2t+1)$) with probability $2/n$ instead. From every frequent 
	%state in an odd-indexed layer $(2i-1,2t-1)$ there is a transition to the frequent state $(2i-1,2t)$ with probability 1. 
	%From each rare state in an even-indexed layer $(2i-1,2t)$, there are two transitions to rare state $(2i-1,2t+1)$ with 
	%probability $1/2$ and $1/2$. These are the only multi-edge transitions in the construction of $Q$. From each rare state 
	%in an odd-indexed layer $(2i,2t+1)$, there are transitions with probability $1/2$ to frequent states $(2i+1,2t+2)$ and 
	%with probability $1/2$ to $(2i-1,2t+2)$. This completes a description of the construction of the sparse Markov chain $Q$.
	%
	%\item \textbf{Constructing the family $\mathcal{P}$}\\
	%The family $\mathcal{P}$ of Markov chains is contructed by making slight random perturbations to the multi-edge 
	%transitions in $Q$. In particular, every $P \in \mathcal{P}$ has the same set of states as $Q$. In each $P$, every 
	%transition is identical to those in $Q$ except the multi-edge transition probabilities from a rare state in an 
	%even-indexed layer to the corresponding rare state in the next layer. Instead of having a $1/2$ transition probability 
	%on each edge from $(2i,2t)$ to $(2i,2t+1)$, we will have as transition probabilities either $1/2(1 \pm 2\eps)$ or 
	%$1/2(1 \mp 2\eps)$ chosen uniformly at random. Hence this creates a class of sparse Markov chains which contains 
	%$2^{O(n^2)}$ sparse Markov chains.
	%\end{itemize}
	
	%\begin{remark}
	%To convert the above constructions involving multi-edges into ones with simple edges we do the following. Firstly, 
	%note that the only multi-edge transitions are from a rare state to another rare state. To make this instance a simple 
	%graph with at most one directed edge between any pair of vertices we apply a standard graph theoretic transformation: 
	%we make a copy $i'$ for each vertex $i$ involved in a double edge; for each pair of double edges $e_1=(ij)_1, e_2=(ij)_2$ 
	%construct $4$ edges $(ij),(ij'),(i'j),(i'j')$ with weights $w(ij)=w(i'j')=w(e_1)$ and $w(ij')=w(i'j)=w(e_2)$. This 
	%increases the total number of states in a layer by a factor of $3/2$.
	%\end{remark}
	
	%Now, we state a simple claim about the distance between two sparse Markov chains.
	%\begin{claim}
	%\label{clm:dist-monotone}
	%Consider two sparse Markov chains $P$ and $Q$, each with $n$ layers. For any $1 \le t \le n$, let
	%$$\hellingersq{P}{Q}_t = 1 - \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\onev.$$
	%Then, we have that, for any $1 \le t < n$,
	%$$\hellingersq{P}{Q}_t \le \hellingersq{P}{Q}_{t+1}.$$
	%\end{claim}
	%\begin{proof}
	%Let $\vect{v}^{\top} = \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}$. Then $\vect{v}^{\top} 
	%\circ \onev =  \onenorm{\vect{v}}$. Since $P_{t+1}$ and $Q_{t+1}$ are stochastic matrices, 
	%$\srprod{P_{t+1}}{Q_{t+1}}$ has non-negative entries and moreover from Perron-Frobenius theorem we have that 
	%$\srprod{P_{t+1}}{Q_{t+1}} \circ \onev \le \onev$ entry-wise. Hence $\vect{v}^{\top} \circ 
	%\srprod{P_{t+1}}{Q_{t+1}} \circ \onev \le \onenorm{\vect{v}}$ implying the claim.
	%\end{proof}
	
	The idea of this construction is that a typical trajectory of Markov chain $Q$ or $P\in\mathcal{P}$ 
	stays in frequent states almost all the time and very rarely visits one of the rare states.  However,
	a typical trajectory has constant probability of visiting a rare state.
	\begin{lemma}
		\label{clm:p-far-from-q shuffle}
		Any $P \in \mathcal{P}$ is at least $\eps$-far from $Q$, i.e., $\dist{P}{Q}= \dtv{\word{P}{T}}{\word{Q}{T}}\ge\eps$.
	\end{lemma}
	\begin{proof}
		Consider a $P \in \mathcal{P}$. First, we argue that probability of any word $w$
		with only a single visit to a rare state (at even $t=2k$) satisfies $\left| \Prx[Q]{w} - \Prx[P]{w}\right|  = 4\eps\cdot\Prx[Q]{w}.$
		%We will show $\dist{P}{Q}$ is large by arguing that the probability of any word 
		%with only one visit to a rare state at even time step $t=2k$ differs under $Q$ and under $P$ by at least $2\eps$ factor. 
		Indeed, let visit to the rare state $2i$ in $w$ happen at the time $t=2k$, then
		\[
		\begin{cases}
		\Prx[Q]{w} = \Prx[Q]{s_1 \ldots s_{2k}}\cdot \frac{1}{2} \cdot \Prx[Q]{s_{2k+1} \ldots s_{2n+1}|s_{2k+1}}\\
		\Prx[P]{w} = \Prx[P]{s_1 \ldots s_{2k}}\cdot \frac{1}{2}(1 \pm 4\eps) \cdot \Prx[P]{s_{2k+1} \ldots s_{2n+1}|s_{2k+1}}.
		\end{cases}
		\]
		Therefore, as $Q$ and $P$ have the same transitional probabilities of $s_t\to s_{t+1}$ for $t\neq 2k$, we get 
		$$\left| \Prx[Q]{w} - \Prx[P]{w}\right|  = 4\eps\cdot\Prx[Q]{w}.$$ 
		Now, the probability of visiting a rare state exactly once (at even $t$) in $Q$ is precisely 
		\[
		\sum_{\substack{w \text{ with}\\ \text{1 rare visit}}} \Prx[Q]{w} = n\cdot\frac{2}{n}\cdot\left(1-\frac{2}{n}\right)^{n-1}> 2\cdot e^{-2}>\frac{1}{4},
		\]
		where we used inequality $(1-\frac{1}{n})^{n-1}> e^{-1}$ to get the estimate in the right hand side.
		%The probability of 0 visits to rare states is $(1-2/n)^{n} \le e^{-4}$. Conditioned on there being a visit to a 
		%rare state, the probability of 0 additional visits to rare states in even-indexed layers is $(1-2/n)^{2n-2} \le 
		%4e^{-4}$ for $n \ge 4$. Hence the probability of exactly one rare state visit in an even-indexed layer is 
		%$\ge (1-e^{-4})(1-4e^{-4}) \ge 1/2$. 
		Hence, 
		\begin{align*}
		\dtv{\word{P}{T}}{\word{Q}{T}} \ge \sum_{\substack{w \text{ with}\\ \text{1 rare visit}}} 
		\left|\Prx[Q]{w} - \Prx[P]{w}  \right| =  \sum_{\substack{w \text{ with}\\ \text{1 rare visit}}}4\eps\cdot\Prx[Q]{w} 
		\ge 4\eps\cdot\frac{1}{4} = \eps.
		\end{align*}
		%From the relation between total variation and Hellinger squared distances and Claim \ref{clm:dist-monotone}, we 
		%have that, $\dist{P}{Q} \ge \hellingersq{P}{Q} \ge \hellingersq{P}{Q}_2$. Under our construction, $\oneet \circ 
		%\srprod{P_1}{Q_1} = \frac{1}{n}\onev^{\text{T}}$ and it can be seen that $\oneet \circ \srprod{P_1}{Q_1} \circ 
		%\srprod{P_2}{Q_2} \circ \onev \le 1-\eps$. Hence $\hellingersq{P}{Q}_2 \ge \eps$ thereby proving the claim.
	\end{proof}
	
	
	%We group transitions within a single word into two categories: Those which occur from a frequent state and those 
	%which occur from a rare state. Note that from a rare state, the transition has to happen to a frequent state. 
	We define collisions and $3$-way collisions similar to the proof of Theorem~\ref{thm:symm-lower-bound}. Namely,
	a collision is a transition that occurs in two samples (3-way collision -- in at least three samples) of $Q^{\otimes m}$ or $P^{\otimes m}$ from the 
	same state and at the same time. Moreover, as $P\sim\mathcal{P}$ and $Q$ are the same except for the double edges
	between rare states, we are only interested in the collisions along multi-edges between rare states. 
	%If the same transition repeats in two samples, we call it a collision. If it occurs in 3 distinct samples, we 
	%call it a 3-way collision. We make the following observations about $Q$ and $\mathcal{P}$.
	
	
	\begin{lemma}
		\label{clm:num-collisions shuffle}
		The expected number of collisions in samples $Q^{\otimes m}$ is $O\left(\frac{m^2}{n^2} \right) = O\left(\frac{1}{\eps^4} \right)$.
		%Consider a sample from $Q^{\otimes m}$. The expected number of collisions among transitions from a rare state 
		%to another rare state is $O\left(\frac{m^2}{n^2} \right) = O\left(\frac{1}{\eps^4} \right)$.
	\end{lemma}
	\begin{proof}
		Let $I_w(m_1,m_2,y,t)$ indicate the event that either of the transitions along edges $e_{1,2}=y\to y$ at time $t$, occurred in samples $m_1$ and $m_2$. 
		Note that at each fixed time all of the $n$ frequent states are equally likely to occur in a sample from $Q$. Therefore, the probability of visiting given
		rare state $y$ at time $t$ in a single run is at most $O(1/n^2)$. 
		%probability is uniformly spread over all $n$ frequent states and the probability of 
		%transitioning to a rare state from a frequent state is $2/n$.
		This implies 
		$\Prx[Q]{I_w(m_1,m_2,y,t) = 1} = O\left(\frac{1}{n^2}\cdot \frac{1}{n^2}\right) = 
		O(1/n^4)$.
		%because at each time probability is uniformly spread over all $O(n)$ frequent states and the probability of 
		%transitioning to a rare state from a frequent state is $2/n$. 
		Let $X$ denote the total number of collisions.
		\begin{align*}
		\Ex{X} &= \sum_{m_1 \neq m_2}\sum_{i\neq j} \Ex{I_w(m_1,m_2,y,t)} = O\left(m^2n^2 \frac{1}{n^4} \right) = 
		O\left(\frac{m^2}{n^2} \right)
		\end{align*}
	\end{proof}
	
	
	\begin{lemma}
		\label{clm:3-way collision shuffle}
		The probability of a 3-way collision in samples $Q^{\otimes m}$ is $o(1)$.
		%Consider $m=\frac{n}{\eps^2}$ samples from either $Q$. The probability of a 3-way collision 
		%among the $m$ samples is $o(1)$.
	\end{lemma}
	\begin{proof}
		Similar to the proof of Lemma~\ref{clm:num-collisions shuffle} we can give an upper bound on the expected number of 
		$3$-way collisions being $\Ocomplex{n^2m^3\cdot\frac{1}{n^6}\cdot }=\Ocomplex{\frac{m^3}{n^4}}$. Markov's inequality concludes 
		the proof.
	\end{proof}
	
	Now consider a typical set of $m$ words generated by $Q$ (or equivalently drawn from $Q^{\otimes m}$).
	%$\bar{P}\sim\mathcal{P}$. 
	As we know from Lemma~\ref{clm:3-way collision shuffle} it has no 3-way collisions and by Markov's inequality 
	and Lemma~\ref{clm:num-collisions shuffle} has at most $O(\frac{1}{\eps^2})$ collisions with probability greater 
	than $9/10$ (for sufficiently small $c>0$ and $m=\frac{cn}{\eps^2}$). As we show next a typical set of $m$ words drawn from 
	$Q$ has similar probability under the $\bar{P}\sim\mathcal{P}$ and $Q$ models.
	
	\begin{lemma}
		\label{clm:no-collision-analysis shuffle}
		At least $1/2$ of the sets $S = \{w_1,\ldots,w_m\}$ of samples from $Q^{\otimes m}$ satisfy 
		$$ \frac{1}{2}\cdot\prob[Q^{\otimes m}]{S}<\prob[\bar{P}^{\otimes m}]{S} < 2\cdot \prob[Q^{\otimes m}]{S}$$
	\end{lemma}
	\begin{proof}
		We consider the ratio of the respective probabilities $(*)\eqdef\frac{\prob[\bar{P}^{\otimes m}]{S}}{\prob[Q^{\otimes m}]{S}}$. As in 
		Lemma~\ref{clm:no-collision-analysis}, both probabilities in the numerator and denominator can be expressed in terms of 
		simple statistics for the set $S$, specifically the number of single step transitions between pairs of states. 
		Also similar to the Lemma~\ref{clm:no-collision-analysis}, the corresponding multiplicative terms for $\bar{P}^{\otimes m}$ 
		and $Q^{\otimes m}$ are identical except for the collisions along multi-edges between two rare states (at least two transitions between
		a pair of rare states). Moreover, we also differentiate type I and type II collisions between rare states: (type I) transitions between
		rare states $y\to y$ at time $t$ were made along different edges $e_1$ and $e_2$; (type II) two transitions were made along the same edge
		either $e_1$, or $e_2$. Per type I and II collisions the corresponding terms in $(*)$ are respectively
		$(1-4\eps)(1+4\eps)=1-16\eps^2$ and $1+16\eps^2$.
		
		We further continue following the proof of the Lemma~\ref{clm:no-collision-analysis}, and make sure that with high probability there are only $X=O(\frac{1}{\eps^4})$ collisions and
		no $3$-way collisions in $S$. We can make sure that the difference between numbers of type I and type II collisions is at most $O(\sqrt{X})=O(\frac{1}{\eps^2})$ 
		with probability at least $3/4$, as the choice of collision type in $w$ under $Q$ model is uniform between type I and type II and independent across different collisions.
		For small enough $m=\Omega(\frac{n}{\eps^2})$ we can make sure that at least $\frac{1}{2}$ fraction of words $w$ under $Q$ model have the number of collisions
		at most $\frac{c_1}{\eps^4}$ and also have the difference between number of type I and type II collisions at most $\frac{c_2}{\eps^2}$, for some small constants $c_1,c_2>0$.
		In this case we get the following bounds on $(*)$.
		\[
		2>\left(1+16\eps^2\right)^{\frac{c_2}{\eps^2}}>\frac{\prob[\bar{P}^{\otimes m}]{S}}{\prob[Q^{\otimes m}]{S}}>
		\left(1-256\eps^4\right)^{\frac{c_1}{2\eps^4}}\cdot \left(1-16\eps^2\right)^{\frac{c_2}{\eps^2}}>1/2
		\]
		
		
		%For each feasible set of samples $S$ under $Q$, i.e., $S$ such that $\prob[Q]{S}>0$
		%\[
		%\Prlong[Q]{S}=\left(\frac{1}{2(n-1)}\right)^{m-1}
		%\quad\quad 
		%\Prlong[\bar{P}\sim\mathcal{P}]{w}=\prod_{j>i}\sum_{\bar{P}_{(ij)_1}=\frac{1\pm\sqrt{8\eps}}{2(n-1)}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|} 
		%\]
		%
		%First, if $w$ has only one transition along edge $(ij)$, then the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{w}$ 
		%\[
		%\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1}{2}\left(\frac{1+\sqrt{8\eps}}{2(n-1)}+\frac{1-\sqrt{8\eps}}{2(n-1)}\right)=
		%\frac{1}{2(n-1)}.
		%\]
		%From Claim \ref{clm:3-way collision shuffle}, we know that probability of a $3$-way collision in $S$ is $o(1)$ under $Q$ model. We observe that for a $2$-way collision $(ij)$
		%(a collision which is not a $3$-way collision), the corresponding term in $\prob[\bar{P}\sim\mathcal{P}]{S}$  for the case of transition along two different 
		%edges $(ij)_1$ and $(ij)_2$ is
		%\[
		%\sum_{\bar{P}_{(ij)_1}} \bar{P}_{(ij)_1}^{|\{(ij)_1\in w\}|} \cdot\bar{P}_{(ij)_2}^{|\{(ij)_2\in w\}|}=\frac{1+\sqrt{8\eps}}{2(n-1)}\cdot\frac{1-\sqrt{8\eps}}{2(n-1)}=
		%\frac{(1-8\eps)}{4(n-1)^2}.
		%\] 
		%We call this type of collision {\em type I} collision. For the other case ({\em type II} collisions) of transition along the same edges the respective probability is 
		%$\frac{(1+8\eps^2)}{4n^2}$. By Claim~\ref{clm:num-collisions shuffle} and by Markov inequality the total number of collisions is $O(\frac{1}{\eps^4})$ with probability $\frac{3}{4}$. 
		%We can also make sure that out of these collisions number of type I and type II collisions is roughly the same. More precisely, the difference between numbers of 
		%type I and type II collisions is at most $O(\frac{1}{\eps^2})$ with probability of at least $\frac{3}{4}$. Indeed, the choice of edge collision type in $w$ is uniform 
		%between type I and type II, and is independent across all collision edges. Now, for small enough $m$ we can make sure that at least $\frac{1}{2}$ fraction of words $w$ 
		%has number of collisions at most $\frac{c_1}{\eps^4}$ and the difference between number of type I and II collisions is at most $\frac{c_2}{\eps^2}$, for some small 
		%constants $c_1,c_2>0$. Thus the corresponding density functions can be related as follows.
		%\[
		%2>\left(1+8\eps^2\right)^{\frac{c_2}{\eps^2}}>\frac{\prob[\bar{P}\sim\mathcal{P}]{w}}{\prob[Q]{w}}>
		%\left(1-64\eps^4\right)^{\frac{c_1}{2\eps^4}}\cdot \left(1-8\eps^2\right)^{\frac{c_2}{\eps^2}}>1/2
		%\]
	\end{proof}
	
	Lemma~\ref{clm:no-collision-analysis shuffle} shows that $\dtv{Q^{\otimes m}}{\bar{P}^{\otimes m}} \leq \frac{3}{4}$ for $m 
	\leq \frac{cn}{\eps^2}$ for some constant $c$, which implies that no algorithm can successfully distinguish $Q$ from the family 
	$\mathcal{P}$ with probability greater than $\frac{3}{4}$ for some $m=\Omega(\frac{n}{\eps^2})$.
\end{proof}

==> sparse_ub.tex <==
For the upper bound, one might consider an appropriately defined statistic on the number of visits to a particular state $s_{i,t}$ to distinguish between the two cases. Such statistics however can be mathematically difficult to deal with and we obtain worse bounds on the moments. In this paper, instead, we consider a different statistic. We look at all one-step transitions that can have positive probability in the Markov chain $Q$ or $P$, we call these one-step transitions as {\em edges}. 
We denote a generic edge from a state $s_{i,t-1}$ to a state $s_{j,t}$ by $e$; the set of all possible edges by $E$; the set of transitions in $E$ between 
states at time $t-1$ and time $t$ by $E(t)$ for each $t\in[n]$. For each edge $e$, let $q_e$ and $p_e$ be the probabilities that there was a transition along 
edge $e$ in one sample $s_1\cdots s_n$ from $Q$, or from $P$, respectively. Our statistic is defined on these edges. From a high level perspective, it consists of two steps: 

\paragraph{Pruning.} We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. We show that the Markov chain obtained post pruning and renormalization is still close to the original chain (Lemma \ref{cl:rejection_Q}). This step is necessary as rare instances of such transitions along {\em rare edges} could potentially shift the value of the statistic by a lot and we want to avoid that. Let $E^*$ be 
the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
rejected samples. Otherwise, we continue to the next step. In Lemma \ref{cl:error_prob_pruning} we show that returning $P \neq Q$ in this step doesn't affect the success probability by too much.
\paragraph{$\chi^2$-statistic on edges.} For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
  \[
      Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
  \]
We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold. This test is similar in spirit to that of \cite{AcharyaDK15} but requires much more involved analysis.
Indeed, in our stetting it is not clear which statistic to use: one can attempt to count frequencies of state visits in the MC, or employ other state dependent statistics.
After many trials and errors we figured out that doing the analysis across separate edges was the best approach.
Indeed, since we are dealing with non i.i.d. but dependent samples, obtaining a non-trivial variance bound for our edge statistic proves to be a challenging task. 
Similar to the classical i.i.d. setting, Poissonization helps to ease the analysis in our setting too. However, we rely on it in more subtle way: 
the effects of Poissonization at the top layer of $n$ states percolate nicely through to the bottom layers of the chain as shown in Lemma~\ref{cl:ind_poisson}. We show that $\Var{Z} = \Ocomplex{kn^3}$ 
in Lemmas~\ref{cl:var_z} and~\ref{cl:var_z_easy}. Another challenge for us was to relate the new definition of distance between two non stationary Markov chains with 
the parameters in the description of their kernels, as e.g. in our Lemma~\ref{cl:expectation_dist}.
%\begin{description}
 %\item[Pruning.] We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. Let $E^*$ be 
%the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
%rejected samples. Otherwise, we continue to the next step.
 %\item[$\chi^2$-statistic on edges.] For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
%{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
  %\[
      %Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
  %\]
  %We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold.
%\end{description}
Our $\chi^2$ test yields the following guarantee on the number of samples
\begin{theorem}
There is an algorithm that can tell whether $P=Q$, or $P\neq Q$, when $\dist{P}{Q}\ge\eps$,  
with probability at least $\frac{2}{3}$ using $O(\frac{n^{3/2}}{\eps^2})$ samples.
\label{th:main_shuffling}
\end{theorem}
Note that, while we state the above theorem in terms of the number of samples, we really mean that we observe a single trajectory from the sparse Markov chain which we have partitioned into segments of length $n$. In particular, the length of the required trajectory for the above statements is a factor of $n$ larger than the stated number of samples. Additionally note that to properly compare to our results from Section~\ref{sec:symmetric} we should note that the number of states here is $O(n^2)$.
All details are provided in Section~\ref{sec:riffle_ub_details}. We also have a complementary lower bound which is presented in Section \ref{sec:sparse_lb}. 


\subsection{More Details on the Tester for Sparse Markov Chains}
\label{sec:riffle_ub_details}
We consider all one-step transitions that can have positive probability in the Markov chain $Q$ or $P$, we call these one-step transitions as {\em edges}. 
We denote a generic edge from a state $s_{i,t-1}$ to a state $s_{j,t}$ by $e$; the set of all possible edges by $E$; the set of transitions in $E$ between 
states at time $t-1$ and time $t$ by $E(t)$ for each $t\in[n]$. 
%We also add new edges $E(0)$ to $E$, which indicate transitions to the original states at 
%time $t=0$ with positive probabilities in $q_0$ or $p_0$. 
For each edge $e$, let $q_e$ and $p_e$ be the probabilities that there was a transition along 
edge $e$ in one sample $s_1\cdots s_n$ from $Q$, or from $P$, respectively.
Our test, from a high level perspective, consists of two steps: 
\begin{description}
	\item[Pruning.] We remove all {\em rare edges}, i.e., edges that are traversed with probability less than $O(\frac{\eps^2}{n^2})$ in $Q$. Let $E^*$ be 
	the resulting pruned set of edges. We reject all samples from $P$ that go along any removed edge $e\notin E^*$. We return $P\neq Q$ if there are too many 
	rejected samples. Otherwise, we continue to the next step.
	\item[$\chi^2$-statistic on edges.] For each non rare edge $e\in E^*$ we count the number of transitions $n_e$ along $e$. We define $\chi^2$ 
	{\em edge statistic} $Z_e\eqdef\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$. Our main statistic is 
	\[
	Z\eqdef\sum_{e\in E^*}Z_e =\sum_{e\in E^*}\frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}.
	\]
	We accept or reject $P=Q$ depending on $Z$ being smaller or larger than a certain threshold.
\end{description}
In the remainder of this section we mostly focus on the latter step. Specifically, we analyze the $\chi^2$ edge statistic in the case when 
$q_e\ge\Omega(\frac{\eps^2}{n^2})$ for all $e\in E$ and $p_e=0$ for all $e\notin E$. At the end of the section we explain why after the pruning step these conditions 
are satisfied. 

%Poisson number of samples with expectation $m$.
\paragraph{Poisson Sampling.} Throughout the analysis of $\chi^2$ statistic, we use the standard Poissonization approach. 
Instead of drawing exactly $m$ samples from $P$, we first draw $m'\sim\Poisson{m}$, and then draw $m'$ samples from $P$. 
The benefit of this is that the number of times different elements in the support of the cut distribution occur in the sample become 
independent, giving simpler analysis. Moreover, the number of transitions observed along the edge 
$e\in E(t)$, $n_e$, for a fixed $t$ will be distributed as $\Poisson{m\cdot p_e}$, independently for all $e\in E(t)$ (see Lemma~\ref{cl:ind_poisson}). As 
$\Poisson{m}$ is tightly concentrated around $m$, this additional flexibility comes only at a sub-constant cost in 
the sample complexity with an inversely exponential in $m$, additive increase in the error probability. We note that 
as in equations $(1-2)$ from~\cite{AcharyaDK15} the expectation and variance of our $\chi^2$ statistic are as follows.
\[
\Ex{Z_e}=m\cdot\frac{(p_e-q_e)^2}{q_e} 
\quad\text{and}\quad 
\Var{Z_e}=2\frac{p_e^2}{q_e^2}+m\cdot\frac{p_e(p_e-q_e)^2}{q_e^2}.
\]

\begin{lemma}
	\label{cl:ind_poisson}
	The number of transitions $n_e$ along an edge $e$ is distributed as $\Poisson{m\cdot p_e}$ and all $n_e$ are independent for $e\in E(t)$, for any
	$t\in[n]$.
\end{lemma}
\begin{proof}
	The proof proceeds by induction on $t$ and is based on the following two standard observations on Poisson random variables:
	
	\textit{(Observation I)} for any discrete distribution $\distr$, $k\sim\Poisson{\lambda}$ i.i.d. samples from
	$\distr$ form a collection of jointly independent Poisson random variables for the occurrences of each element in 
	the support of $\distr$, i.e., distribution $\prod_i\Poisson{\lambda\cdot\Prx[x\sim\distr]{x=i}}$;
	
	\textit{(Observation II)} the sum of two independent Poisson random variables with distributions $\Poisson{\lambda_1}$ and $\Poisson{\lambda_2}$
	is a Poisson random variable with the distribution $\Poisson{\lambda_1+\lambda_2}$.
	
	For $t=1$ as we start with $\Poisson{m}$ samples,  Observation I gives us the desired result. For the induction step (from $t=k$ to $t=k+1$), we observe that counts of visits to each particular state $i$ at time $t$ are independent Poisson random variables by Observation II. Now, Observation I 
	applied to the states at time $t$ yields the desired result.
\end{proof}

The following procedure correctly distinguishes between the case $P=Q$, or $\dist{P}{Q}\ge\eps$, in the regime when $q_e\ge\Omega(\frac{\eps^2}{n^2})$ 
for all $e\in E(Q)$ and $p_e=0$ for all $e\notin E$.

\begin{algorithm}[H]
	\caption{$\chi^2$ Edge Test}
	\label{alg:chi_sq_edges}
	\KwIn{$\eps$; an explicit $k$-sparse Markov Chain $Q=\MCseqQ$; (Poisson) $m$ samples from a Markov Chain $P=\MCseqP$, where $n_e$ 
		denotes the number of transitions along the edge $e$.}
	\KwOut{Accept if $P=Q$, or reject if $\dist{P}{Q}\ge\eps$}
	\BlankLine
	$E\leftarrow\{e: q_e> 0\}$\;  
	$Z\leftarrow\sum\limits_{e\in E} \frac{(n_e-q_e\cdot m)^2-n_e}{q_e\cdot m}$\; 
	%\eIf{$Z\le\frac{\eps\cdot m}{4}$}
	\eIf{$Z\le 2\sqrt{k}n^{3/2}$}
	{
		\KwRet \textsc{Accept}\;  
	}
	{
		\KwRet \textsc{Reject}\;  
	}
\end{algorithm}

\begin{theorem} 
	Algorithm~\ref{alg:chi_sq_edges} is correct with probability at least $4/5$, if $m\ge\frac{C n^{3/2}}{\eps^2}$ for some $C=O(1)$, 
	$q_e\ge\frac{\eps^2}{kn^2}$ for all $e\in E$, and $p_e=0$ for all $e\notin E$.
	\label{th:sparse_ub}
\end{theorem}
\begin{proof} To get the desired result we analyze expectation and variance of $Z$. First, we relate the expected value of $Z$ with the distance $\dist{P}{Q}$ between $P$ and $Q$.
	
	\begin{lemma}
		\label{cl:expectation_dist}
		%%$\Ex{Z}\ge m\cdot\hellingersq{P}{Q}.$
		$\Ex{Z}\ge \frac{m}{4}\cdot\distsq{P}{Q}.$
	\end{lemma}
	\begin{proof}
		We recall that 
		\begin{multline}
		\label{eq:dist_P_Q_sum}
		\hellingersq{P}{Q}  =1-\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_t}{Q_t}\circ\cdots\srprod{P_n}{Q_n}\circ\onev\\
		= \oneet\circ\left(\frac{P_1+Q_1}{2}\right)\circ\cdots\circ\left(\frac{P_n+Q_n}{2}\right)\circ\onev-
		\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\srprod{P_n}{Q_n}\circ\onev\\
		=\sum_{t=1}^{n} \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\left(\frac{P_t+Q_t}{2}-\srprod{P_t}{Q_t}\right)\circ\left(\frac{P_{t+1}+Q_{t+1}}{2}\right)\cdots
		\left(\frac{P_{n}+Q_{n}}{2}\right)\circ\onev\\
		=\frac{1}{2}\sum_{t=1}^{n} \oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_{t-1}}{Q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev,
		\end{multline}
		where in the last line $\sqsrprod{P_t}{Q_t}=\left(\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2\right)_{ij}$. Indeed, the first equality holds true as
		$P_t\circ\onev=Q_t\circ\onev=\onev$ for any $t\in[n]$; the second equality is a telescopic sum; the last equality is simply the formula for the complete square. 
		Let $q_t$ and $p_t$ be the respective distribution vectors over the states $s_{i,t}$, $i\in[n]$ in $Q$ and $P$ Markov chains. We also define distributions $p_0=q_0=\onee$.
		
		By applying Cauchy-Schwarz inequality to the corresponding Bhattacharya coefficient of $P$ and $Q$ at a fixed state $i$ and time $t$  
		we obtain
		\begin{align*}
		\oneet\circ\srprod{P_1}{Q_1}\circ\cdots\circ\srprod{P_{t}}{Q_{t}}\circ\onevi=
		HS_i\left(\word{P}{t},\word{Q}{t}\right)  = \sum_{\substack{w=s_0\ldots s_t \\ \text{s.t. } s_t=i}}  \sqrt{\Prl[P]{w}\Prl[Q]{w}}\\
		\le\sqrt{\sum_{\substack{w=s_1\ldots s_t \\ \text{s.t. } s_t=i}}  \Prl[P]{w}\sum_{\substack{w=s_1\ldots s_t \\ \text{s.t. } s_t=i}}\Prl[Q]{w}} 
		=\sqrt{p_t(i)\cdot q_t(i)}.
		\end{align*}
		We plug in this estimate to \eqref{eq:dist_P_Q_sum} and obtain
		\[
		\frac{1}{4}\cdot\distsq{P}{Q}=\frac{1}{4}\dtvsq{P}{Q}\le \hellingersq{P}{Q}  \le \frac{1}{2}\sum_{t=1}^{n} \srprodt{p_{t-1}}{q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev,
		\]
		%where $p_{-1}=q_{-1}$ is a probability distribution with one element in the support and $P_0$ and $Q_0$ are the $1\times n$ matrices corresponding to $p_0$ and $q_0$ vectors. 
		We examine each term of the summation in the right hand side of the last equation
		\be
		\label{eq:dist_sqrtpq}
		\frac{1}{2}\srprodt{p_{t-1}}{q_{t-1}}\circ\sqsrprod{P_t}{Q_t}\circ\onev=\sum_{i}\frac{\sqrt{p_{t-1}(i)\cdot q_{t-1}(i)}}{2}\cdot\sum_{j:(ij)\in E(t)}
		\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2,
		\ee
		We show that corresponding terms in $\Ex{Z}=\sum\limits_{i,t}\sum\limits_{e:(ij)\in E(t)}\Ex{Z_e}$ give an upper bound on \eqref{eq:dist_sqrtpq} for each fixed state $i$.
		
		\begin{multline}
		\frac{1}{m}\sum_{e:(ij)\in E(t)}\Ex{Z_e}=\sum_{e:(ij)\in E(t)}\frac{(p_e-q_e)^2}{q_e}=\sum_{j:(ij)\in E(t)}
		\frac{\left(p_{t-1}(i)P_t(ij)-q_{t-1}(i)Q_t(ij)\right)^2}{q_{t-1}(i)Q_t(ij)}\\
		%=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\frac{P_t^2(ij)}{Q_t(ij)}-2p_{t-1}(i)\sum_{j:(ij)\in E(t)}P_t(ij)+q_{t-1}(i)\sum_{j:(ij)\in E(t)}Q_t(ij)\\
		=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\left(\sum_{j:(ij)\in E(t)}\frac{P_t^2(ij)}{Q_t(ij)}\right)-2p_{t-1}(i)+q_{t-1}(i)\\
		%=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\frac{\left(P_t(ij)-Q_t(ij)\right)^2}{Q_t(ij)}+
		%2P_t(ij)-Q_t(ij)\right)-2p_{t-1}(i)+q_{t-1}(i)\\
		=\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\frac{\left(P_t(ij)-Q_t(ij)\right)^2}{Q_t(ij)}+
		\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\\
		%= \frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2\left(\frac{\sqrt{P_t(ij)}+\sqrt{Q_t(ij)}}{\sqrt{Q_t(ij)}}\right)^2+
		%\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\\
		\ge \frac{p_{t-1}^2(i)}{q_{t-1}(i)}\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2+\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)},
		\label{eq:inequality_sqrtpq}
		\end{multline}
		where the third and forth equalities hold true as $\sum_{j:(ij)\in E(t)}P_t(ij)=\sum_{j:(ij)\in E(t)}Q_t(ij)=1$, and to get the last inequality one can simply use identity 
		$\frac{(a-b)^2}{b}=(\sqrt{a}-\sqrt{b})^2\left(\frac{\sqrt{a}+\sqrt{b}}{\sqrt{b}}\right)^2$. Now, we claim that the expression in RHS of \eqref{eq:inequality_sqrtpq} is 
		at least RHS of \eqref{eq:dist_sqrtpq} for a given $i$, i.e., we need to show that
		\be
		\label{eq:inequality_four_deg_poly}
		\left(\frac{p_{t-1}^2(i)}{q_{t-1}(i)}-\frac{\sqrt{p_{t-1}(i)q_{t-1}(i)}}{2}\right)\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-
		\sqrt{Q_t(ij)}\right)^2+\frac{\left(p_{t-1}(i)-q_{t-1}(i)\right)^2}{q_{t-1}(i)}\ge 0.
		\ee
		The inequality is obviously true, if $\frac{p_{t-1}^2(i)}{q_{t-1}(i)}\ge\frac{\sqrt{p_{t-1}(i)q_{t-1}(i)}}{2}$.
		Otherwise, without loss of generality, we can substitute the term 
		\[
		\sum_{j:(ij)\in E(t)}\left(\sqrt{P_t(ij)}-\sqrt{Q_t(ij)}\right)^2
		\] 
		with an upper bound of $2$. Furthermore, by denoting $x=\sqrt{\frac{p_{t-1}(i)}{q_{t-1}(i)}}$ the inequality \eqref{eq:inequality_four_deg_poly} can be rewritten as
		$q_{t-1}(i)\cdot\left(2x^4-x+(x^2-1)^2\right)\ge 0$, and, indeed, one can verify that this fourth degree polynomial is always positive.
	\end{proof}
	
	Now we estimate the variance of random variable $Z$
	
	\begin{lemma}
		$\Ex{Z}\ge \left(\frac{12\sqrt{2k}}{C}+\frac{2\sqrt{2}+\sqrt{k}}{\sqrt{C}}\right)\cdot\sqrt{\Var{Z}}$, when $m\ge \frac{C\cdot n^{3/2}}{\eps^2}$ and $\dist{P}{Q}\ge \eps$.
		\label{cl:var_z}
	\end{lemma}
	\begin{proof}
		We recall that $Z=\sum_{e\in E}Z_e$ and by Lemma~\ref{cl:ind_poisson} all $Z_e$ for a fixed $t$ and $e\in E(t)$ are independent.
		For any random variables $X_1,\dots, X_n$ it is true that 
		\[
		\Var{X_1+\cdots+X_n}\le\left(\sqrt{\Var{X_1}}+\cdots+\sqrt{\Var{X_n}}\right)^2.
		\]
		We use this estimate for $X_t=\sum_{e\in E(t)}Z_e$ to obtain
		\[
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\Var{Z_e}}=\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}+m\cdot\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\]
		We further simplify the above expression by using the fact that $\sqrt{x+y}\le \sqrt{x}+\sqrt{y}$.
		\be
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}}+\sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\label{eq:var_sqrt_ub}
		\ee
		
		On the other hand, by Lemma~\ref{cl:expectation_dist}
		\be
		\label{eq:expectation_def_eps}
		\Ex{Z}\ge \frac{1}{2}\Ex{Z} + \frac{m}{8}\distsq{P}{Q} =  m\cdot\left(\frac{1}{2}\sum_{e\in E}\frac{(p_e-q_e)^2}{q_e}+\frac{\eps^2}{8}\right).
		\ee
		In the following we use \eqref{eq:expectation_def_eps} to give separate upper bounds on each of the two summation terms in the 
		RHS of \eqref{eq:var_sqrt_ub}. 
		
		\paragraph{First term of \eqref{eq:var_sqrt_ub}.} To estimate the first term, we split $E$ into two sets 
		\[
		E_1\eqdef\{e\in E: p_e\le 2q_e\} \quad\text{and}\quad E_2\eqdef\{e\in E: p_e> 2q_e\}
		\]
		We define accordingly the sets $E_1(t)$ and $E_2(t)$ for each $t\in[n]$. Again we have
		\beq
		\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{p_e^2}{q_e^2}}\le \sum_{t=1}^n\sqrt{\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}} + \sum_{t=1}^n\sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}}.
		\eeq
		\textbf{Estimate for $\mathbf{E_1}$.} 
		We have $2\frac{p_e^2}{q_e^2}\le 8$ for any edge $e\in E_1$. Therefore, by the sparsity condition $\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}\le 8n\cdot k$, where $k=O(1)$.
		Thus, 
		%\nick{determine $c_1$}
		\be
		\sum_{t=1}^n\sqrt{\sum_{e\in E_1(t)}2\frac{p_e^2}{q_e^2}}\le \sqrt{8k}\cdot n^{3/2}\le \frac{\sqrt{8k}}{C} \cdot m\cdot \eps^2 \le \frac{4\sqrt{8k}}{C}\cdot\Ex{Z} 
		\label{eq:e1}
		\ee
		\textbf{Estimate for $\mathbf{E_2}$.} We have $\frac{(p_e-q_e)^2}{q_e}\ge \frac{p_e^2}{4q_e}$ for any $e\in E_2$. Therefore,
		%\nick{$c_2\cdot m\frac{\eps^2}{4n^{3/2}}=1$}
		\begin{multline}
		\frac{\sqrt{32k}}{C}\cdot\Ex{Z}\ge \frac{\sqrt{32k}m}{C}\cdot\sum_{t=1}^n\left(\frac{1}{16}\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e}+\frac{\eps^2}{8n}\right)
		\ge \frac{\sqrt{32k}m}{C}\sqrt{\frac{4\eps^2}{16\cdot 8n}}\sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e}}\\
		\ge \frac{\sqrt{32k}m}{C}\sqrt{\frac{\eps^2}{32n}}\cdot\sqrt{\frac{\eps^2}{kn^2}}\sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}}
		\ge \sum_{t=1}^n \sqrt{\sum_{e\in E_2(t)}2\frac{p_e^2}{q_e^2}},
		\label{eq:e2}
		\end{multline}
		where the first inequality holds by \eqref{eq:expectation_def_eps}; the second inequality is simply AM-GM inequality; and to get the third
		inequality we used the bound $q_e\ge\frac{\eps^2}{kn^2}$.
		
		\paragraph{Second term  of \eqref{eq:var_sqrt_ub}.} We split $E$ into another two sets $E_3,E_4$ (similarly define $E_3(t)$ and $E_4(t)$): 
		\[
		E_3\eqdef\{e\in E: p_e\le 2\sqrt{n}q_e\} \quad\text{and}\quad E_4\eqdef\{e\in E: p_e> 2\sqrt{n}q_e\}
		\]
		\[
		\text{Again}\quad \sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}+
		\sum_{t=1}^n\sqrt{\sum_{e\in E_4(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		\]
		\textbf{Estimate for $\mathbf{E_3}$.} We have 
		\begin{multline}
		2\sqrt{\frac{2}{C}}\cdot\Ex{Z}\ge \sqrt{\frac{2}{C}}m\cdot\sum_{t=1}^n\left(\sum_{e\in E_3(t)}\frac{(p_e-q_e)^2}{q_e}+\frac{\eps^2}{4n}\right)\ge
		\sqrt{\frac{2}{C}}m\sqrt{\frac{\eps^2}{n}}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{(p_e-q_e)^2}{q_e}}\\
		\ge m\sqrt{\frac{2\eps^2}{Cn}}\cdot \sqrt{\frac{1}{2n^{1/2}}}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}}
		= \sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E_3(t)}\frac{p_e(p_e-q_e)^2}{q_e^2}},
		\label{eq:e3}
		\end{multline}
		where the first inequality holds by \eqref{eq:expectation_def_eps}, the second inequality is AM-GM inequality, to get the third inequality
		we use definition of $E_3$ that $\frac{p_e}{q_e}\le 2\sqrt{n}$.\newline
		\textbf{Estimate for $\mathbf{E_4}$.} We have $p_e-q_e\ge \left(1-\frac{1}{2\sqrt{n}}\right)p_e$ for any $e\in E_4$. Therefore,
		\begin{multline}
		\frac{\sqrt{k}}{\sqrt{2C}\left(1-\frac{1}{2\sqrt{n}}\right)}\cdot\Ex{Z}\ge \frac{m\sqrt{k}}{\sqrt{2C}}\sum_{e\in E_4}\frac{p_e(p_e-q_e)}{q_e}\ge
		\sqrt{m}\sqrt{\frac{km\cdot2\eps^2 }{2C\cdot kn^{3/2}}}\sum_{e\in E_4}\frac{p_e^{1/2}(p_e-q_e)}{q_e}\\
		\ge\sqrt{m}\sum_{t=1}^n\sqrt{\sum_{e\in E_4(t)}\frac{p_e^{1/2}(p_e-q_e)}{q_e}},
		\label{eq:e4}
		\end{multline}
		where the first inequality follows from\eqref{eq:expectation_def_eps}, to get the second inequality we estimate $\sqrt{p_e}\ge \sqrt{2n^{1/2}q_e}\ge\sqrt{\frac{2\eps^2}{kn^{3/2}}},$
		to get the last inequality we simply use that $\sqrt{x}+\sqrt{y}\ge\sqrt{x+y}$. 
		
		Finally, combining estimates \eqref{eq:e1},\eqref{eq:e2},\eqref{eq:e3},\eqref{eq:e4} we obtain the desired bound on the variance.
	\end{proof}
	
	\begin{lemma}
		If $P=Q$, then $\Var{Z}\le\sqrt{k}n^{3/2}$.
		\label{cl:var_z_easy}
	\end{lemma}
	\begin{proof}
		Using similar estimate as in the proof of Lemma~\ref{cl:var_z} we get
		\[
		\sqrt{\Var{Z}}\le\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}\Var{Z_e}}=\sum_{t=1}^n\sqrt{\sum_{e\in E(t)}2\frac{q_e^2}{q_e^2}}\le n\cdot\sqrt{kn}.
		\]
	\end{proof}
	
	To conclude the proof of Theorem~\ref{th:sparse_ub} it remains to notice that in case $P=Q$ the error probability (Algorithm~\ref{alg:chi_sq_edges} returns ``reject'') is at most
	\[
	\Prx{Z> 2\sqrt{k}n^{3/2}}\le\Prx{Z> 2\sqrt{\Var{Z}}}\le \frac{1}{5},
	\]
	where the first inequality follows from Lemma~\ref{cl:var_z_easy}, the last is Cantelli's inequality, since $\Ex{Z}=0$.
	On the other hand, when $\dist{P}{Q}\ge \eps$, then $\Ex{Z}\ge m\cdot\frac{\eps^2}{4}$. If Algorithm~\ref{alg:chi_sq_edges} makes an error by returning ``accept'', 
	then $Z\le 2\sqrt{k}n^{3/2}\le \frac{2\sqrt{k}}{C}\Ex{Z}$. Thus $Z-\Ex{Z}\le (\frac{2\sqrt{k}}{C}-1)\Ex{Z}$. Now if $C$ is such that
	$1-\frac{2\sqrt{k}}{C}\ge 2\cdot\left(\frac{12\sqrt{2k}}{C}+\frac{2\sqrt{2}+\sqrt{k}}{\sqrt{C}}\right)$ (any constant 
	$C\ge\max\left(\sqrt{k}(42\sqrt{2}+4),(8\sqrt{2}+4\sqrt{k})^2\right)$ would work), then $Z-\Ex{Z}\le -2\sqrt{\Var{Z}}$ by Lemma~\ref{cl:var_z}. Furthermore,
	by Cantelli's inequality 
	\[
	\Prx{Z\le 2\sqrt{k}n^{3/2}}\le \Prx{Z-\Ex{Z}\le -2\sqrt{\Var{Z}}}\le \frac{1}{5},
	\]
	i.e., probability of Algorithm~\ref{alg:chi_sq_edges}'s error in the case $P\neq Q$ is at most $\frac{1}{5}$.  
\end{proof}


\paragraph{Analysis of pruning step.} Here we slightly modify Markov Chains $Q$ and $P$ so that the probability of traversing any edge in $Q$ is $\Omega(\frac{\eps^2}{n^2})$ and that 
$P$ only uses these edges. To this end, we sequentially remove edges from $Q$ that have too low probability of traversal in $Q$. Effectively, in the pruning process we are sampling from $Q$, but rejecting all the 
samples that use a ``rare'' edge. We choose the threshold for the ``rare'' edges in such a way that we would reject at most $\eps^2$ fraction of samples from $Q$. Recall that the Markov chain obtained by pruning $Q$ is denoted as $Q^*$.
After pruning of $Q$, we do the corresponding empirical rejection sampling for $P$ (see Algorithm~\ref{alg:pruning}) which is equivalent to obtaining samples from the modified Markov chain $P^*$. If there are too many rejected samples, 
we conclude that $\dist{P}{P^*}>\dist{Q}{Q^*}$ with high probability, and thus $P\neq Q$. Otherwise we proceed to Algorithm~\ref{alg:chi_sq_edges} for the modified $Q$ and pruned samples 
from $P$. 

\begin{algorithm}%[H]
	\caption{Pruning Test. In the pruned Markov Chain $Q^*$ all edges with $q_e>0$ satisfy $q_e\ge\frac{\eps^2}{kn^2};$ samples from Markov Chain $P^*$ can only go along these edges.}
	\label{alg:pruning}
	\SetKwData{Recompute}{Recompute}\SetKwData{Samples}{PrunedSamples}\SetKwData{Count}{RejectCount}
	\SetKwFunction{Delete}{Delete}
	\KwIn{$\eps$; an explicit $k$-sparse Markov Chain $Q=\MCseqQ$; $m$ samples from a Markov Chain $P=\MCseqP$}
	\KwOut{$m\cdot(1-2\eps^2)$ i.i.d. samples from pruned $P^*$ and pruned $Q^*$ s.t., each $q_e=\Omega(\frac{\eps^2}{n^2})$; reject $P$ if there are not enough samples.}
	\BlankLine
	Let $E^*=\{e: q_e>0\}$\;
	\While{$\exists~e\in E^*:q_{e}<\frac{\eps^2}{k\cdot n^2}$}{
		$E^*\leftarrow E^*\setminus e$\tcc*{$e=(ij)$, $e\in E(t)$}
		\Delete($e,Q$)\tcc*{set $Q_t(ij)=0$, re-normalize row $i$ in $Q_t$}
		\lForEach{edge $e\in E^*$}{\Recompute{$q_e$}}
	}
	\For{$w=s_1\cdots s_n \sim P$}{
		\lIf{$\forall~t~ (s_ts_{t+1})\in E^*$}{Add $w$ to \Samples}
		\lElse{increase \Count}
	}
	\eIf{\Count$>2m\eps^2$}
	{
		\KwRet \textsc{Reject}\;  
	}
	{
		\KwRet \Samples\;  
	}
\end{algorithm}


Let $Q^*$ be a modified Markov Chain $Q$ that sample $w\sim Q$ and reject any $w$ with $e\notin E^*$.
\begin{lemma}
	$\dist{Q}{Q^*}\le 2\eps^2$
	\label{cl:rejection_Q}
\end{lemma}   
\begin{proof}
	By definition of the set of pruned edges $E^*$, by removing each new edge we lose at most $\frac{\eps^2}{kn^2}$ fraction of samples.
	As there are only at most $kn^2$ edges in $Q$, the probability of avoiding removed edges is at least
	$(1-\frac{\eps^2}{kn^2})^{kn^2}\ge 1-\eps^2$. Thus at most $\eps^2$ fraction of words $\word{Q}{n}$ are rejected in $\word{Q^*}{n}$, which implies that
	$2\eps^2\le\dtv{\word{Q}{n}}{\word{Q^*}{n}}=\dist{Q}{Q^*}$.
\end{proof}

We need to argue about probability of error in Algorithm~\ref{alg:pruning}. First, in the case $P=Q$ Algorithm~\ref{alg:pruning} could incorrectly return ``reject''.
Our next Lemma~\ref{cl:error_prob_pruning} provides the necessary bound. On the other hand, when $P\neq Q$ and  Algorithm~\ref{alg:pruning} does not return ``reject'', we 
want Algorithm~\ref{alg:chi_sq_edges} to be able to distinguish $P^*$ and $Q^*$. To this end, Lemma~\ref{cl:error_prob_pruning} shows that $\dist{P^*}{Q^*}=\Omega(\eps)$ 
with high probability.  


%Therefore, in the case $P=Q$ we have $\dist{P}{P^*}\le 2\eps^2$. In this case we show that Algorithm~\ref{alg:pruning} does not reject $P$
%with high probability. On the other hand, if $P\neq Q$ and Algorithm~\ref{alg:pruning} does not reject $P$, 
%we want to make sure that Algorithm~\ref{alg:chi_sq_edges} will distinguish $P^*$ and $Q^*$. To this end, we need to provide a lower bound on 
%$\dist{P^*}{Q^*}\ge\eps-\dist{P}{P^*}-\dist{Q}{Q^*}$. As $\dist{Q}{Q^*}\le 2\eps^2$, for a lower bound of $\dist{P^*}{Q^*}\ge\frac{\eps}{4}$ 
%it would suffice to show that $\dist{P^*}{P}\le\frac{\eps}{2}$.
\begin{lemma}~
	\label{cl:error_prob_pruning}
	
	(1) If $P=Q$, then Algorithm~\ref{alg:pruning}'s error of rejecting $P$ is at most $0.1$.
	
	(2) If $\dist{P}{Q}\ge \eps$, then either $\dist{P^*}{Q^*}=\Omega(\eps)$, or Algorithm~\ref{alg:pruning} correctly rejects $P$ with probability at least $0.9$.
\end{lemma}
\begin{proof}
	Let $X_\ell$ be Bernoulli random variables for $\ell\in[m]$ denoting ($X_\ell=1$) whether $\ell$-th sample from $P$ was rejected, or accepted to $P^*$ ($X_\ell=0$).  
	Then the number of rejected samples $X=\sum_{\ell=1}^m X_\ell$. Variables $X_\ell$ are i.i.d. Let $x=\Prx{X=1}$.
	
	1. If $P=Q$, then probability of rejecting a sample from $P$ is not more than $\eps^2$, i.e., $x\le \eps^2$. $\Ex{X}=m\cdot x, \Var{X}=m\cdot(x-x^2)$. Then
	\[
	\Prx{X\ge 2m\eps^2}\le\Prx{X\ge \Ex{X}+3\sqrt{\Var{X}}}\le\frac{1}{10},
	\]
	where the first inequality holds because $2m\eps^2> m\cdot \eps^2 + 3\sqrt{m\eps^2}>\Ex{X}+3\sqrt{\Var{X}}$; the second is Cantelli's inequality.
	
	2. We first observe that $\dist{P^*}{Q^*}\ge\eps-\dist{Q}{Q^*}-\dist{P}{P^*}$. We want to argue that if $\dist{P}{P^*}\ge 6\eps^2$, then
	Algorithm~\ref{alg:pruning} rejects $P$ with probability at least $9/10$. Indeed, then probability $x$ of rejecting a sample from $P$ must be at least 
	$\frac{1}{2}\dist{P}{P^*}\ge 3\eps^2$, then $\Ex{X}\ge 3m\eps^2$ and
	\[
	\Prx{X\le 2m\eps^2}\le\Prx{X-\Ex{X}\le -\frac{\Ex{X}}{3}}\le\Prx{X-\Ex{X}\le -3\sqrt{\Var{X}}}\le\frac{1}{10}.
	\]
	Thus we get $\dist{P^*}{Q^*}\ge\eps-\dist{Q}{Q^*}-\dist{P}{P^*}\ge\eps-2\eps^2-6\eps^2\ge\frac{\eps}{2}$ if $\eps$ is small enough constant. 
\end{proof}

\begin{theorem}
	Together, Algorithm~\ref{alg:pruning} and Algorithm~\ref{alg:chi_sq_edges} tell whether $P=Q$, 
	or $P\neq Q$, when $\dist{P}{Q}\ge\eps$,  with probability at least $\frac{2}{3}$ using $O(\frac{n^{3/2}}{\eps^2})$ samples.
	%\label{th:main_shuffling}
\end{theorem}
\begin{proof}
	In case $P=Q$, Algorithm~\ref{alg:pruning} produces $P^*=Q^*$ and $m(1-2\eps^2)$ samples from $P^*$ with probability at least $0.9$.
	Furthermore, Algorithm~\ref{alg:chi_sq_edges} converts these $m(1-2\eps^2)$ samples into Poisson $m'=\Omega(m)$ samples and accepts
	$P=Q$ with $4/5$ probability. Overall, we have $4/5\cdot 0.9>2/3$ probability of correctly accepting $P=Q$.
	
	When $\dist{P}{Q}\ge\eps$, Algorithm~\ref{alg:pruning} either correctly rejects $P^*$, or produces $P^*$ and $Q^*$ s.t. $\dist{P^*}{Q^*}\ge\frac{\eps}{2}$ with probability at least $0.9$. In the latter case Algorithm~\ref{alg:chi_sq_edges} correctly rejects $P^*$ with probability at least $4/5$. Overall, we get the probability of correctly rejecting $P$ to be at least $4/5\cdot 0.9>2/3$.
\end{proof}

==> tight_upper_bound.tex <==
\section{A Linear in $n$ Upper Bound}

\input{MC_to_adversarial}
\input{adversarial}
